Monotone Submodular Multiway Partition

In submodular multiway partition (SUB-MP), the input is a non-negative submodular function $f:2^V \rightarrow \mathbb{R}_{\ge 0}$ given by an evaluation oracle along with $k$ terminals $t_1, t_2, \ldots, t_k\in V$. The goal is to find a partition $V_1, V_2, \ldots, V_k$ of $V$ with $t_i\in V_i$ for every $i\in [k]$ in order to minimize $\sum_{i=1}^k f(V_i)$. In this work, we focus on SUB-MP when the input function is monotone (termed MONO-SUB-MP). MONO-SUB-MP formulates partitioning problems over several interesting structures -- e.g., matrices, matroids, graphs, and hypergraphs. MONO-SUB-MP is NP-hard since the graph multiway cut problem can be cast as a special case. We investigate the approximability of MONO-SUB-MP: we show that it admits a $4/3$-approximation and does not admit a $(10/9-\epsilon)$-approximation for every constant $\epsilon>0$. Next, we study a special case of MONO-SUB-MP where the monotone submodular function of interest is the coverage function of an input graph, termed GRAPH-COVERAGE-MP. GRAPH-COVERAGE-MP is equivalent to the classic multiway cut problem for the purposes of exact optimization. We show that GRAPH-COVERAGE-MP admits a $1.125$-approximation and does not admit a $(1.00074-\epsilon)$-approximation for every constant $\epsilon>0$ assuming the Unique Games Conjecture. These results separate GRAPH-COVERAGE-MP from graph multiway cut in terms of approximability.

==> algorithm.tex <==

    
\subsection{Approximation Algorithm}
In this section, we describe our algorithm for \monosubmp and analyze its approximation factor. 
For $\vx \in [0, 1]^n$ and $\theta \in [0, 1]$, we define $\vx^{\theta}\in \{0,1\}^n$ as 
\[
(\vx^\theta)_j := 
\begin{cases} 
1 & \text{ if } \vx_j \geq \theta, \\ 
0 & \text{ otherwise. }  
\end{cases}
\]
We also define $f\left(\vx^\theta\right) := f\left(\{v_j \colon (\vx^\theta)_j = 1\}\right)$. We define the Lov\'{a}sz extension $\hat{f}:[0,1]^n\rightarrow \R$ of $f$ as follows: For all $\vx \in [0, 1]^n$, $\hat{f}(\vx) := \E_{\theta \in [0, 1]}\left[f(\vx^\theta)\right] = \int_0^1 f\left(\vx^\theta\right) d\theta$. We define $\vx_i = \left(x(v_1, i), \ldots, x(v_n, i)\right)$ and consider the convex program %\submprel 
below:
\begin{align}
    \text{minimize } \sum_{i = 1}^k \hat{f}\left(\vx_i\right) & \tag{Sub-MP-Rel} \label{CP:submp} \\
    %\text{subject to: } 
    \sum_{i = 1}^k x(v, i) = 1 & \quad \forall v \in V \notag\\
    x(t_i, i) = 1 & \quad \forall i \in [k] \notag\\
    x(v, i) \geq 0 & \quad \forall v \in V, i \in [k]. \notag
\end{align}
The convex program is identical to the convex programming relaxation of \submp 
introduced by Chekuri and Ene and it can be solved in polynomial time \cite{CE}. 
%It is a relaxation for \submp and 
%The convex program can be solved can be solved in polynomial time. 
We present a rounding algorithm for \monosubmp based on this relaxation. Our rounding algorithm is similar to the $\theta$-rounding algorithms of Chekuri and Ene for \submp and \symsubmp \cite{CE}, but the interval from which we choose $\theta$ is different. 
%Using the same interval as that of Chekuri and Ene for \submp or \symsubmp does not achieve a $4/3$-approximation (see Remark \ref{??}).  
Our choice for the interval of $\theta$ is designed to exploit monotonicity in order to achieve a better approximation factor. 
Below, we present the rounding algorithm for \monosubmp:
\begin{algorithm}[H] % H causes weird spacing right now
\caption{Mono-Sub-MP Rounding}\label{alg:mono}
\begin{algorithmic}
    \State Let $\vx$ be an optimal solution to \ref{CP:submp} %SUBMP-REL
    \State Choose $\theta \in [\frac{1}{4}, 1]$ uniformly at random
    \For{$i \in [k]$}
        \State $A(i, \theta) \gets \{v \in V \colon x(v, i) \geq \theta \}$
    \EndFor
    \State $U(\theta) \gets V - \bigcup_{i = 1}^k A(i, \theta)$
    \For{$v \in V$}
        \State $I_v \gets \{i \in [k] \colon v \in A(i, \theta) \}$
        \If{$|I_v| > 1$}
            \State delete $v$ from all but one of the sets $\{A(i, \theta)\}_{i \in I_v}$
        \EndIf
    \EndFor
    \State \Return $\left(A_1, \ldots, A_{k - 1}, A_k \right) = \left(A(1, \theta), \ldots, A(k - 1, \theta), A(k, \theta) \cup U(\theta) \right)$
\end{algorithmic}
\end{algorithm}

We observe that the rounding algorithm guarantees that each $v \in V$ is assigned to exactly one of the returned sets. Additionally, for each $i \in [k]$, we have that $t_i \in A(i, \theta)$ since $\vx(t_i,i)=1$. Hence, the algorithm returns a feasible multiway partition of $V$. Moreover, the algorithm can be implemented to run in polynomial time. It remains to bound the approximation factor. 


==> approximation-factor.tex <==

\subsubsection{Approximation Factor Analysis}
The following is the main theorem of this section. It bounds the approximation factor of Algorithm \ref{alg:mono} relative to the optimum value of \ref{CP:submp}. 

\begin{restatable}{theorem}{thmMonoSubMPRelCP} \label{thm:mono-sumbp-4/3}
 Let $\opt_{frac}$ be the optimal value of \ref{CP:submp} and $S_1, \ldots, S_k$ be the solution returned by Algorithm \ref{alg:mono}. Then, 
\[
    \E\left[\sum_{i=1}^k f(S_i)\right]\le \frac{4}{3}\opt_{frac}. 
\]

%Algorithm \ref{alg:mono} achieves an approximation factor of $4/3$ for \monosubmp.
\end{restatable}

The rest of this section is devoted to proving Theorem \ref{thm:mono-sumbp-4/3}. 
Our approximation factor analysis uses certain ingredients of Chekuri and Ene, but differs from their analysis to exploit monotonicity. We will point out the differences as we proceed with the analysis. 

We start with a lemma about the truncated mass of a discrete probability distribution. A vector $x\in \R^k_{\ge 0}$ with $\sum_{i\in [k]}x_i=1$ can be viewed as a probability distribution over the set $\{1,2,\ldots, k\}$ with $x_i$ being the probability of picking item $i$. For $\delta\in [0,1]$, the quantity $\sum_{i=1}^k \min\{\delta, x_i\}$ is the truncated probability mass. We show that if $\delta\ge 1/4$, then the truncated probability mass is at least $1-\max_{i\in [k]}x_i$. The choice of $\delta\in [1/4,1]$ in the rounding algorthm emanates from this lemma. This lemma does not appear in Chekuri and Ene \cite{CE} and is our contribution. 

\begin{lemma} \label{claim:1/4-ineq}
    Let $\vx \in \mathbb{R}^k_{\ge 0}$ such that $\sum_{i = 1}^k x_i = 1$ and $\delta \ge 1/4$. Then, 
    \[\sum_{i = 1}^k \min\left\{\delta, x_i\right\} \geq 1 - \max_{i \in [k]} x_i.\]
\end{lemma}
\begin{proof}
    % Proof of claim 3.1
    The LHS can be rewritten as follows: 
    \begin{align*}
        \sum_{i = 1}^{k} \min\left\{\delta, x_i\right\} &= \sum_{i = 1}^{k} x_i - \sum_{i \in [k]: x_i > \delta} (x_i - \delta)  
        = 1 - \sum_{i \in [k] : x_i > \delta} (x_i - \delta)
    \end{align*}
    % Hence, it suffices to show that $\sum_{i\in [k]: x_i>\delta}(x_i-\delta) \le \max_{i\in [k]}x_i$. 
    \iffalse
    \begin{align*}
        \sum_{i = 1}^k \min(\delta, x_i) \geq 1 - \max_{i = 1}^k x_i 
        &\iff 1 - \sum_{i : x_i > \delta} (x_i - \delta) \geq 1 - \max_{i = 1}^k x_i \\ 
        &\iff \sum_{i : x_i > \delta} (x_i - \delta) \leq \max_{i = 1}^k x_i
    \end{align*}
    \fi
    % \knote{
    Let $L:=\{i\in [k]: x_i>\delta\}$ and let $j\in [k]$ such that $x_j=\max_{i\in [k]}x_i$. 
    It suffices to show that $x_j \ge \sum_{i\in L}(x_i-\delta)$. 
    For the sake of contradiction, suppose that $x_j <\sum_{i\in L}(x_i-\delta)$. We case based on the size of $L-\{j\}$ and arrive at a contradiction in all cases.
    
    \noindent \textbf{Case 1.} Suppose $L-\{j\}=\emptyset$. If $j\in L$, then $L=\{j\}$, and hence, 
    \[
    x_j < \sum_{i\in L}(x_i-\delta) = x_j - \delta,
    \]
    a contradiction. If $j\not\in L$, then $L=\emptyset$, and hence,
    \[
    0\le x_j < \sum_{i\in L}(x_i-\delta) = 0,
    \]
    a contradiction. 
    
    \noindent \textbf{Case 2.} Suppose $|L-\{j\}|=1$. Let $L-\{j\}=\{\ell\}$. Then, by definition of $j, \ell,$ and $L$, we have that $L=\{\ell, j\}$. Consequently, we have that 
    \[
    x_j < \sum_{i\in L}(x_i-\delta) = x_j + x_{\ell} - 2\delta.
    \]
    Hence, we have that $x_{\ell}> 2\delta \ge 1/2$ since $\delta \ge 1/4$. Also, by definition of $j$, we have that $x_j\ge x_{\ell}$. Hence, we have that $x_j\ge x_{\ell}>1/2$ and hence, $\sum_{i=1}^k x_i \ge x_j + x_k >1$, a contradiction.

    \noindent \textbf{Case 3.} Suppose $|L-\{j\}|\ge 2$. 
    Then, by definition of $j$, we have that $j\in L$ and hence, $|L|\ge 3$ and $x_j\ge \delta$. Thus, we have that 
    \[
    \delta \le x_j <\sum_{i\in L}(x_i-\delta) \le \left(\sum_{i\in L}x_i\right) - 3\delta.
    \]
    The last inequality above is because $|L|\ge 3$. From the above inequalities, we have that $\sum_{i=1}^k x_i \ge \sum_{i\in L}x_i > 4\delta \ge 1$, a contradiction. 
\end{proof}
    % }

    
    % Let $j$ be the index for which $x_j$ is maximum. Then we claim, 

\iffalse
    \begin{claim} \label{claim:sub-ineq}
        $\sum_{i : x_i > \delta, i \neq j} (x_i - \delta) \leq \delta \Rightarrow \sum_{i : x_i > \delta} (x_i - \delta) \leq x_j$
    \end{claim}
    \begin{proof}
        We shall proceed via cases. 
        \begin{case} 
        $\{i : x_i > \delta, i \neq j\} = \phi$.
        \end{case}
        Then, $\{i : x_i > \delta\} = \{j\}$ or $\phi$. So, $\sum_{i : x_i > \delta} (x_i - \delta)$ is $x_j - \delta$ or $0$. In either case, $\sum_{i : x_i > \delta} (x_i - \delta) \leq x_j$.
        \begin{case}
            $\{i : x_i > \delta, i \neq j\} \neq \phi$
        \end{case}
        Then, $j \in \{i : x_i > \delta\}$. So, we add $x_j$ and subtract $\delta$ from both sides of left hand side of the claim to get, 
        \begin{align*}
            \sum_{i : x_i > \delta, i \neq j} (x_i - \delta) \leq \delta &\Rightarrow \sum_{i : x_i > \delta, i \neq j} (x_i - \delta) + x_j - \delta \leq \delta + x_j - \delta \\ 
            &\Rightarrow \sum_{i : x_i > \delta} (x_i - \delta) \leq x_j 
        \end{align*}
    \end{proof}
    Now that we have claim \ref{claim:sub-ineq}, showing $\sum_{i : x_i > \delta, i \neq j} (x_i - \delta) \leq \delta$ suffices to show claim \ref{claim:1/4-ineq}. 

    \begin{claim} \label{claim:final-ineq}
        $\sum_{i : x_i > \delta, i \neq j} (x_i - \delta) \leq \delta$
    \end{claim}
    \begin{proof}
        We again proceed via cases. \setcounter{case}{0}
        % Find a proper way to reset counter of cases to 0.
        \begin{case}
            $\{i : x_i > \delta, i \neq j\} = \phi$
        \end{case}
        Then, $\sum_{i : x_i > \delta, i \neq j} (x_i - \delta) = 0 \leq \delta$. Hence the inequality holds.
        \begin{case}
            $|\{i : x_i > \delta, i \neq j\}| = 1$
        \end{case}
        Let $\{i : x_i > \delta, i \neq j\} = \{l\}$. If we have 
        \begin{align*}
            \sum_{i : x_i > \delta, i \neq j} (x_i - \delta) > \delta &\Rightarrow x_l - \delta > \delta
            \Rightarrow x_l > 2\delta
        \end{align*}
        Since $\delta \geq \frac{1}{4}$, we get $x_l > \frac{1}{2}$. We also have $x_j \geq x_l > \frac{1}{2}$. Hence, $\sum_{i=1}^{k} x_i \geq x_l + x_j > 1$ which gives us a contradiction showing the claim.
        \begin{case}
            $|\{i : x_i > \delta, i \neq j\}| \geq 2$
        \end{case}
        Let $ \sum_{i : x_i > \delta, i \neq j} (x_i - \delta) > \delta$. We get, 
        \begin{align*}
            \delta < \sum_{i : x_i > \delta, i \neq j} (x_i - \delta) \leq \sum_{i : x_i > \delta, i \neq j} x_i - 2\delta \\
            \Rightarrow \sum_{i : x_i > \delta, i \neq j} x_i > 3\delta
        \end{align*}
        Adding $x_j$ to both sides, and with $x_j \geq \delta$ (since $\{i : x_i > \delta, i \neq j\} \neq \phi$) we get 
        \begin{align*}
            \sum_{i : x_i > \delta, i \neq j} x_i + x_j = \sum_{i=1}^{k}x_i > 3\delta + x_j \geq 4\delta
        \end{align*}
        Using $\delta \geq \frac{1}{4}$, and $\sum_{i = 1}^{k} x_i = 1$ implies $1 > 1$ which is a contradiction. 
        This finishes the proof of claim \ref{claim:final-ineq}
    \end{proof}
    
    Hence, the proof of claim \ref{claim:final-ineq} finishes the proof of claim \ref{claim:1/4-ineq}
    \knote{Can remove Claim \ref{claim:final-ineq}.}
% \end{proof}
\fi

\begin{remark}\label{remark:tight-for-1/4-ineq}
    The conclusion of Lemma \ref{claim:1/4-ineq} fails for $\delta <1/4$. We give an example to illustrate this: let $k=2$ and let $x_1=1/2, x_2 = 1/2$. Now, consider $\delta <1/4$. Then, the LHS of the lemma is $\sum_{i=1}^k \min\{\delta, x_i\}=\min\{\delta, x_1\} + \min\{\delta, x_2\} = 2\delta$. On the other hand, the RHS of the lemma is $1-\max_{i\in [k]}x_i = 1- \max\{x_1, x_2\}=1/2$. Thus, the LHS is at least the RHS only for $\delta\ge 1/4$ and fails for $\delta<1/4$. 
    %$2\delta \ge 1/2$ fails to hold if $\delta < 1/4$. 
\end{remark}

We now setup some notation to analyze the approximation factor of our algorithm. This notation is similar to that of Chekuri and Ene \cite{CE}. 
\paragraph{Notation.}
Let $\vx$ be a feasible solution to \submprel. For each $v_j\in V$, we define $\alpha_j = \max_{i = 1}^k x(v_j, i)$. We assume that the elements $v_1, v_2, \ldots, v_n$ of the ground set $V$ are ordered such that $0 \leq \alpha_1 \leq \alpha_2 \leq \ldots \leq \alpha_n \leq 1$. For convenience, we define $\alpha_0 := 0$ and $\alpha_{n + 1} := 1$. For each $j \in [n]$, we let $\ell_j := \argmax_{i = 1}^k x(v_j, i)$. For each $i \in [k]$, we define $A(i, \theta) = \{v \in V \colon x(v, i) \geq \theta\}$. Additionally, for each $j \in [n]$, we let $V_j := \{v_1, \ldots, v_j\}$, and for convenience, we define $V_0 := \emptyset$. Finally, we let $A_j(i, \theta) := A(i, \theta) \cap V_j$.

With the above notation, we show the following technical lemma based on monotonicity and submodularity of $f$ and by using Lemma \ref{claim:1/4-ineq}. Since we rely on monotonicity and Lemma \ref{claim:1/4-ineq}, the following lemma does not follow from the results in Chekuri and Ene \cite{CE}. 
\begin{lemma} \label{lem:telescope-sum}
    For every $\delta \in [\frac{1}{4}, 1]$ and $j \in [n]$, we have that
    \[
        \sum_{i = 1}^k \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \geq (1 - \alpha_j) \left(f(V_j) - f(V_{j - 1}) \right).
    \]
    % \knote{Remember to punctuate math modes. Put a period at the end of the above math mode.}
\end{lemma}
\begin{proof}
    % Let us fix $j \in [n]$ and $i \in [k]$ 
    Let $\delta\in [1/4, 1]$ and $j\in [n]$. We show the following two claims that will help in proving the lemma.
    \begin{claim} \label{claim:telescope-trunc}
    For every $i\in [k]$,
        \[\int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta 
        = \int_0^{\min\{\delta, x(v_j, i)\}} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta.\]
    \end{claim}
    \begin{proof}
        Let $i\in [k]$.
        We may assume that $\min\{\delta, \ x(v_j, i)\}=x(v_j, i)$ (otherwise, the claim holds trivially). 
        % Then, for all $\theta \in (x(v_j, i), \delta]$, we get $x(v_j, i) < \theta$. So, $v_j \notin A(i, \theta)$. Thus, $A_j(i, \theta) = A(i, \theta) \cap V_j = A(i, \theta) \cap V_{j-1} = A_{j-1}(i, \theta)$. 
        For every $\theta \in (x(v_j, i), \delta]$, we get $x(v_j, i) < \theta$ and hence, $v_j \notin A(i, \theta)$. Thus, for every $\theta \in (x(v_j, i), \delta]$, we have that $A_j(i, \theta) = A(i, \theta) \cap V_j = A(i, \theta) \cap V_{j-1} = A_{j-1}(i, \theta)$. Consequently, 
        % Hence, 
        \begin{align*}
            \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta
            &= \int_0^{x(v_j, i)} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta\\ 
            & \quad \quad + \int_{x(v_j, i)}^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \\ 
            &= \int_0^{x(v_j, i)} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta.
        \end{align*}
    \end{proof}
    \begin{claim} \label{claim:sub-telescope}
        For every $i\in [k]$, 
        \[\int_0^{\min\{\delta, x(v_j, i)\}} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta 
        \geq
        \min\{\delta, x(v_j, i)\} \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) d\theta.
        \]
    \end{claim}
    \begin{proof}
        Let $\theta \in [0, \min(\delta, x(v_j, i))]$. Then, $x(v_j, i) \geq \theta$ and thus, $A_j(i, \theta) = A_{j-1}(i, \theta) \cup \{v_j\}$. Additionally, $V_j = V_{j-1} \cup \{v_j\}$, $A_{j-1}(i, \theta) \subseteq V_{j-1}$, and $v_j \notin V_{j-1}$. Hence, we have that 
        \begin{align*}
            f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right) &= f\left(A_{j-1}(i, \theta) \cup \{v_j\}\right) - f\left(A_{j - 1}(i, \theta)\right) \\
            &\geq f\left(V_{j-1} \cup \{v_j\}\right) - f\left(V_{j-1}\right) \quad \quad \text{(by submodularity of $f$)}\\
            &= f\left(V_j\right) - f\left(V_{j-1}\right). 
        \end{align*}
        Thus, 
        \begin{align*}
            \int_0^{\min\{\delta, x(v_j, i)\}} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta 
            &\geq
            \int_0^{\min\{\delta, x(v_j, i)\}} \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) d\theta\\
            &= \min\{\delta, x(v_j, i)\} \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right).
        \end{align*}
        % \knote{Punctuate math mode above.}
    \end{proof}
    Now, we use the above claims to rewrite the LHS of Lemma \ref{lem:telescope-sum} as follows:  
    \begin{align}
        &\sum_{i = 1}^k \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \notag\\
        &\quad \quad \quad \quad =
        \sum_{i = 1}^k \int_0^{\min\{\delta, x(v_j, i)\}} \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \quad \quad \text{(by Claim \ref{claim:telescope-trunc})} \notag\\ 
        &\quad \quad \quad \quad \geq
        %\sum_{i = 1}^k \int_0^{\min(\delta, x(v_j, i))} \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) d\theta \\ &= 
        \sum_{i = 1}^k \min\{\delta, x(v_j, i)\} \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) \quad \quad \text{(by Claim \ref{claim:sub-telescope})} \notag\\ 
        &\quad \quad \quad \quad = \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) \left( \sum_{i = 1}^k \min\{\delta, x(v_j, i)\} \right). \label{ineq:fA_j-difference}
    \end{align}
    Finally, we know that $x(v_j, i)\ge 0$ for every $i \in [k]$ and $\sum_{i=1}^{k} x(v_j, i) = 1$ since $x$ is a feasible solution to the convex program. Hence, using Lemma \ref{claim:1/4-ineq}, we get
    \begin{align}
    \sum_{i=1}^k \min\{\delta, x(v_j, i)\} &\ge 1- \max_{i\in [k]}x(v_j, i) = 1-\alpha_j. \label{ineq:truncated-mass}
    \end{align}
    Further, by monotonicity of $f$, we have that $f(V_j) - f(V_{j-1})\ge 0$. Hence, 
    \begin{align}
    \left(f\left(V_j\right) - f\left(V_{j-1}\right)\right) \left( \sum_{i = 1}^k \min\{\delta, x(v_j, i)\} \right) 
    \geq (1 - \alpha_j)  \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right). \label{ineq:fV_j-difference}
    \end{align}
    
    % \begin{align*}
    %     \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) \left( \sum_{i = 1}^k \min(\delta, x(v_j, i)) \right) &\geq 
    %     \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right) \left( 1 - \max_{i=1}^{k} x(v_j, i) \right) \\
    %     &= (1 - \alpha_j)  \left( f\left(V_j\right) - f\left(V_{j-1}\right)\right)
    % \end{align*}
    Thus, using inequalities (\ref{ineq:fA_j-difference}) and (\ref{ineq:fV_j-difference}), we get that 
    \begin{align*}
        \sum_{i = 1}^k \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \geq (1 - \alpha_j) \left(f(V_j) - f(V_{j - 1}) \right).
    \end{align*}
    % This finishes the proof of lemma \ref{lem:telescope-sum}. \knote{Remove last sentence. The QED symbol takes care of the sentence.} \knote{Punctuate math mode throughout the above proof. Add all periods. }
\end{proof}

We need the following Proposition from Chekuri and Ene \cite{CE}.
\begin{proposition} \cite{CE} \label{prop:U-int-telescope}
    Let $f$ be an arbitrary non-negative submodular function, $r \in [0,1]$, and let $h$ be the largest value of $j$ such that $\alpha_j \leq r$. We have
    \iffalse
    \begin{align*}
        \int_0^r f\left(A(\theta)\right) d\theta = \sum_{j=1}^{h} \alpha_j \left(f(V - V_{j-1}) - f(V - V_j)\right) + rf(V - V_h),
    \end{align*}
    and 
    \fi
    \begin{align*}
        \int_0^r f\left(U(\theta)\right) d\theta = \sum_{j=1}^{h} \alpha_j \left(f(V_{j-1}) - f(V_j)\right) + rf(V_h).
    \end{align*}
\end{proposition}

Lemma \ref{lem:telescope-sum} and Proposition \ref{prop:U-int-telescope} lead to the following corollary. 
\begin{corollary}
\label{cor:at_least_U}
    For every $\delta \in [\frac{1}{4}, 1]$, 
    \[
        \sum_{j = 1}^n \left( \sum_{i = 1}^k \int_0^\delta \left(f(A_j(i, \theta) - f(A_{j - 1}(i, \theta) \right) d\theta \right) \geq \int_0^1 f(U(\theta)) d\theta - f(\emptyset).
    \]
\end{corollary}
\begin{proof}
    We use $r = 1$ and $h = n$ in Proposition \ref{prop:U-int-telescope} to get, 
    \begin{align} \label{eq:u-theta}
        \int_0^1 f\left(U(\theta)\right) d\theta = \sum_{j=1}^{n} \alpha_j \left(f(V_{j-1}) - f(V_j)\right) + f(V_n).
    \end{align}
    Now, by Lemma \ref{lem:telescope-sum}, we get 
    \begin{align*}
        \sum_{j=1}^{n} \left(\sum_{i = 1}^k \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \right) 
        &\geq 
        \sum_{j=1}^{n} (1 - \alpha_j) \left(f(V_j) - f(V_{j - 1}) \right) \\
        &= \sum_{j=1}^{n} \left(f(V_j) - f(V_{j - 1}) \right) + 
         \sum_{j=1}^{n} \alpha_j\left(f(V_{j-1}) - f(V_{j}) \right) \\
         &= f(V_n) - f(V_0) + \sum_{j=1}^{n} \alpha_j\left(f(V_{j-1}) - f(V_{j}) \right). 
    \end{align*}
    Finally, using $V_0 = \emptyset$ and equation (\ref{eq:u-theta}), we get, 
    \begin{align*}
        \sum_{j=1}^{n} \left(\sum_{i = 1}^k \int_0^\delta \left( f\left(A_j(i, \theta)\right) - f\left(A_{j - 1}(i, \theta)\right)\right) d\theta \right) 
        &\geq
        \int_0^1 f(U(\theta)) d\theta - f(\emptyset).
    \end{align*}
\end{proof}

We have the following theorem as a consequence of Corollary \ref{cor:at_least_U}. We observe that this theorem upper bounds the expected function value of the set of unassigned elements. 
\begin{theorem}
\label{thm:sum_of_A_at_least_U}
    For all $\delta \in [\frac{1}{4}, 1]$, 
    \[
        \sum_{i = 1}^k \int_0^\delta f(A(i, \theta)) d\theta \geq (k \delta - 1)f(\emptyset) + \int_0^1 f(U(\theta)) d\theta.
    \]
\end{theorem}
\begin{proof}
We have that 
    \begin{align*}
        \sum_{i = 1}^k \int_0^\delta f(A(i, \theta)) d\theta 
        &= \sum_{i = 1}^k \int_0^\delta f(A_n(i, \theta)) d\theta \\
        &= \sum_{i = 1}^k \int_0^\delta f(A_0(i, \theta)) d\theta + \sum_{j = 1}^n \left( \sum_{i = 1}^k \int_0^\delta f(A_j(i, \theta)) - \sum_{i = 1}^k \int_0^\delta f(A_{j - 1}(i, \theta)) \right) \\
        &= \sum_{i = 1}^k \int_0^\delta f(A_0(i, \theta)) d\theta + \sum_{j = 1}^n \left( \sum_{i = 1}^k \int_0^\delta \left(f(A_j(i, \theta)) - f(A_{j - 1}(i, \theta))\right) d\theta \right) \\
        &\geq \sum_{i = 1}^k \int_0^\delta f(A_0(i, \theta))d\theta + \int_0^1 f(U(\theta)) d\theta - f(\emptyset) \quad \quad \quad \text{(by Corollary \ref{cor:at_least_U})} \\
        &= (k\delta - 1)f(\emptyset) + \int_0^1 f(U(\theta)) d\theta.
    \end{align*}
\end{proof}

\begin{remark}\label{remark:tight-for-assigned-vs-unassigned-charging}
    We note that Theorem \ref{thm:sum_of_A_at_least_U} fails to hold for $\delta<1/4$. We give an example to illustrate this: let $V:=\{t_1, t_2, u\}$, $T:=\{t_1, t_2\}$ (i.e., $n=3$ and $k=2$) and let $f(X):=1$ for every non-empty $X$ and $f(\emptyset)=0$. Setting $x(u, 1)=x(u, 2)=1/2$, $x(t_1, 1) = 1$, $x(t_2, 2)=1$ with the rest of the $x$ values being $0$ gives an optimum solution to the convex program \submprel. Now consider $\delta \le 1/4$. Then, we have that 
    $f(A(1, \theta))=1= f(A(2, \theta))$ for $\theta \in [0, 1/2]$, and hence, the LHS of the theorem is 
    $\sum_{i=1}^k \int_{0}^{\delta}f(A(i, \theta))d\theta = \int_{0}^{\delta} f(A(1, \theta))d\theta + \int_{0}^{\delta}f(A(1, \theta))d\theta= \delta + \delta = 2\delta$. On the other hand, we have that $f(U(\theta))=0$ for every $\theta \in [0,1/2)$ and $f(U(\theta))=1$ for every $\theta \in [1/2,1]$ and   hence, the RHS of the theorem is 
    $\int_{0}^1 f(U(\theta))d\theta = \int_{1/2}^1 f(U(\theta))d\theta = 1/2$. Thus, $2\delta \ge 1/2$ fails to hold if $\delta <1/4$. We note that this tight example for Theorem \ref{thm:sum_of_A_at_least_U} arises from the tight example for Lemma \ref{claim:1/4-ineq} mentioned in Remark \ref{remark:tight-for-1/4-ineq}. 
\end{remark}


We use Theorem \ref{thm:sum_of_A_at_least_U} and submodularity and monotonicity of $f$ to bound the approximation factor of the algorithm relative to the optimum value of the convex program. We restate and prove Theorem \ref{thm:mono-sumbp-4/3} below. 
\thmMonoSubMPRelCP*
\begin{proof}
    %We show that the algorithm Mono-Sub-MP Rounding gives a $\frac{4}{3}$-approximation for Mono-Sub-MP. 
    We note that $\opt_{frac} = \sum_{i = 1}^k \hat{f}(\vx_i) = \int_0^1 \sum_{i = 1}^k f(A(i, \theta)) d\theta$. By Theorem \ref{thm:sum_of_A_at_least_U}, 
    \[
        \sum_{i = 1}^k \int_0^\frac{1}{4} f(A(i, \theta)) d\theta \geq \left(\frac{1}{4}k - 1\right)f(\emptyset) + \int_0^1 f(U(\theta)) d\theta \geq \int_0^1 f(U(\theta)) d\theta. 
    \]
    The last inequality above is because $f(\emptyset)=0$. 
    Rewriting the above inequality gives 
    \begin{align}
        0 &\geq -\sum_{i = 1}^k \int_0^\frac{1}{4} f(A(i, \theta)) d\theta + \int_0^1 f(U(\theta)) d\theta \geq -\sum_{i = 1}^k \int_0^\frac{1}{4} f(A(i, \theta)) d\theta + \int_{\frac{1}{4}}^1f(U(\theta)) d\theta. \label{ineq:minus_A_plus_U}
    \end{align}
Hence, the expected cost of the partition returned by Algorithm \ref{alg:mono} is
    \begin{align*}
        \E_{\theta \in [\frac{1}{4}, 1]}\left[ \sum_{i = 1}^k f(A_i) \right] 
        &\leq \E_{\theta \in [\frac{1}{4}, 1]} \left[ \sum_{i = 1}^{k - 1} f(A(i, \theta)) + f(A(k, \theta) \cup U(\theta))\right] \quad \quad \text{(since $f$ is monotone)} \\
        &\leq \E_{\theta \in [\frac{1}{4}, 1]}\left[ \sum_{i = 1}^k f(A(i, \theta)) + f(U(\theta)) \right] \quad \quad \text{(since $f$ is non-negative and submodular)} \\
        &= \frac{4}{3} \int_{\frac{1}{4}}^1 \left(\sum_{i = 1}^k f(A(i, \theta)) + f(U(\theta))\right) d\theta \\
        &= \frac{4}{3} \left(\opt_{frac} - \sum_{i = 1}^k \int_{0}^{\frac{1}{4}} f(A(i, \theta)) d\theta + \int_{\frac{1}{4}}^1 f(U(\theta)) d\theta \right) \\
        &\leq \frac{4}{3}\opt_{frac}. \quad \quad \text{(by inequality (\ref{ineq:minus_A_plus_U}))}
    \end{align*}
\end{proof}

\begin{remark}
    We emphasize that monotonicity of the function is used only in the proofs of Theorem \ref{thm:mono-sumbp-4/3} and Lemma \ref{lem:telescope-sum}. 
\end{remark}
\begin{remark}
    Our approximation factor analysis for Algorithm \ref{alg:mono} is tight. We give an example to show that Algorithm \ref{alg:mono} does not achieve $(4/3-\epsilon)$-approximation for any constant $\epsilon>0$. Let $V:= \{t_1, t_2, u_1 \cdots, t_{2k-1}, t_{2k}, u_k\}$, $T:= \{t_1, t_2, \cdots, t_{2k}\}$. Let $E_i := \{t_{2i-1}, t_{2i}, u_i\}$ and $f(X) := |\{j : X \cap E_j \neq \emptyset\}|$.
    The partition $V_{2i} = \{t_{2i}, u_{i}\}$, $V_{2i-1} = \{t_{2i-1}\}$ is optimal for this instance of \monosubmp, with $\sum_{i=1}^{2k} f(V_i) = \sum_{i=1}^{k} \left(f(V_{2i}) + f(V_{2i-1})\right) = 2k$. 
    Now, setting $x(u_i, i) = x(u_i, i+1) = \frac{1}{2}$ with the rest of the $x$ values being $0$ gives an optimum solution to the convex program \submprel. For $\theta \in (\frac{1}{2}, 1]$, $A(i, \theta) = \{t_i\}$, $U(\theta) = \{u_1, \cdots, u_k\}$. Hence, the algorithm returns $V_i = \{t_i\}$ for $i \in [2k-1]$, $V_{2k} = \{u_1, \cdots, u_k, t_{2k}\}$. This gives $\sum_{i=1}^{2k} f(V_i) = 3k-1$. Further, for $\theta \in [\frac{1}{4}, \frac{1}{2}]$, $A(2i, \theta) = \{t_{2i}, u_i\}$ and $A(2i-1) = \{t_{2i-1}, u_i\}$. Hence, the algorithm returns $V_{2i} = \{t_i, u_i\}$, $V_{2i-1} = \{t_{2i-1}\}$, and $\sum_{i=1}^{2k} f(V_i) = 2k$. Hence, $\E_{\theta \in [\frac{1}{4}, 1]}[\sum_{i=1}^{2k} f(V_i)] = \frac{1}{3}(2k) + \frac{2}{3}(3k-1) = \frac{8k-2}{3}$. Hence, approximation factor for this example is $\frac{8k-2}{6k} = \frac{4}{3} - \frac{1}{3k}$. Setting $k$ large enough gives us the desired result.
    We mention that this example is obtained by taking multiple copies of the tight example for Theorem \ref{thm:sum_of_A_at_least_U} mentioned in Remark \ref{remark:tight-for-assigned-vs-unassigned-charging}.

    
\end{remark}

\begin{remark}
For threshold rounding where the threshold $\theta$ is picked uniformly at random from the interval $[1/2, 1]$ (i.e., Chekuri and Ene's rounding algorithm for \submp), the best possible approximation factor is at least $3/2$. The example in the previous remark illustrates this. 
%Moreover, for threshold rounding where the threshold $\theta$ is picked uniformly at random from the interval $[0, 1]$ and the sets are subsequently uncrossed via monotonicity (i.e., akin to Chekuri and Ene's rounding algorithm for \symsubmp), the best possible approximation factor is at least $2$: 
\end{remark}

\iffalse
\begin{remark} \label{rmk:0-1-rounding}
    Single threshold rounding with uniformly random $\theta \in [0, 1]$ gives a $2$-approximation. We first observe that 
    \begin{align}
        \E_{\theta \in [0, 1]} \left[f\left(U(\theta)\right)\right] &= \int_0^1 f\left(U(\theta)\right) d\theta \notag \\
        &\leq \sum_{i = 1}^k \int_0^{\frac{1}{4}} f\left(A(i, \theta)\right) d\theta \quad \quad \text{(by Theorem \ref{thm:sum_of_A_at_least_U})} \notag \\
        & \leq \sum_{i = 1}^k \int_0^1 f\left(A(i, \theta)\right) d\theta \quad \quad \text{(by non-negativity of $f$)}. 
        \label{ineq:U_bounded_by_OPT}
    \end{align}
    Then, the expected cost of the rounded solution is at most
    \begin{align*}
        \E_{\theta \in [0, 1]} \left[\sum_{i = 1}^k f\left(A(i, \theta)\right) + f(U(\theta)\right] &= \E_{\theta \in [0, 1]} \left[\sum_{i = 1}^k f\left(A(i, \theta)\right) \right] + \E_{\theta \in [0, 1]} \left[ f(U(\theta)\right] \\
        &\leq 2 \sum_{i = 1}^k \int_0^1 f\left(A(i, \theta)\right) d\theta \quad \quad \text{(by inequality (\ref{ineq:U_bounded_by_OPT}))} \\
        &= 2OPT_{frac}. 
    \end{align*}
\end{remark}

\begin{remark}
    The analysis in Remark \ref{rmk:0-1-rounding} is tight if we do not consider uncrossing of the sets $A(i, \theta)$. We consider a star graph with $k$ edges of negligible weight and an additional self loop of weight $W$ such that the degree $1$ vertices are terminals. Then the central vertex of the star has an optimal assignment $x_u = \left(\frac{1}{k}, \cdots, \frac{1}{k}\right)$. Hence, for $\theta \in \left[0, \frac{1}{k}\right]$ we get $A(i, \theta) = \{i, u\}$, with $f(A(i, \theta)) = W$. We also get, for $\theta \in \left(\frac{1}{k}, 1\right]$, $A(i, \theta) = \{i\}$ and $U(\theta) = \{u\}$. Hence $\E_{\theta \in [0, 1]}[\sum_{i=1}^{k-1} f(A(i, \theta)) + f(A(k, \theta) \cup U(\theta))] = 2\left(1 - \frac{1}{k}\right) \cdot W$, whereas the cost of the optimal solution is $W$ giving a $2\left(1 - \frac{1}{k}\right)$ approximation. We observe that the analysis does not change if instead of a self loop we have an edge with weight $W$ and stars with $\frac{k}{2}$ additional edges of negligible weight on each end of this edge.
\end{remark}
\fi

%\subsection{Notes}
\iffalse
\knote{
Essentially, we want the least $\delta$ such that the following holds for every normalized monotone submodular function $f$: 
\begin{align}
\sum_{i=1}^k \int_{0}^{\delta}f\left(A\left(i, \theta\right)\right)d\theta \ge \int_{\delta}^{1}f\left(U\left(\theta\right)\right)d\theta. \label{ineq:sufficient-delta}
\end{align}
If we have such a value of $\delta$, then the approximation factor becomes $1/(1-\delta)$. 
We have shown that the above holds for $\delta = 1/4$. But there is still a slack in inequality \eqref{ineq:minus_A_plus_U} which makes me wonder if inequality \ref{ineq:sufficient-delta} also holds for smaller $\delta$, say $\delta=1/5$ or $\delta = 1/10$? 

Did we have a tight example for Theorem \ref{thm:sum_of_A_at_least_U}? I.e., an example for which the conclusion of the theorem fails for $\delta <1/4$? Does that example also show tightness if we only want inequality \eqref{ineq:sufficient-delta}? Yes, it does show tightness even if we only want inequality \eqref{ineq:sufficient-delta}. 
}
\fi

\iffalse
\knote{What if we consider an alternate rounding algorithm: pick $\theta\in [0, 1]$ uniformly at random and set $A(i):=\{u\in V: x(u, t_i)\ge\theta\}$ for every $i\in [k]$, uncross to ensure that $A(i)$s are disjoint, and assign unassigned elements to $A(1)$?}


\donote{What is the integrality gap of the convex program? Show some lower bound.}

\knote{Consider \gcovmp and rounding by picking $\theta\in [0,1]$ uniformly. Then, we should have the following claim: $1+Pr(u, v\text{ is cut})\le (5/4)(1+||x_u-x_v||_1)$. 
This claim is equivalent to showing that the expected coverage of an edge is at most $5/4$ times the LP-coverage of the edge. 
Prove this claim independently/adapt the proof of CKR to fit this directly. 
Does the proof give any ideas to improve the approximation factor for \monosubmp to $5/4$? Perhaps, the proof gives a counterpart of Lemma 2.1 for $\delta\ge 0$?}

\knote{I think rounding by picking $\theta\in [0,1]$ uniformly should also give a $5/4$-approximation for \covmp --- easy to see for \gcovmp by previous remark; same proof ideas should go through for hypergraphs as well. Verify.} \knote{Same proof ideas do not seem to go through for hypergraphs.}
\knote{If the above is true and if $4/3$ is tight for \monosubmp, then the hard instances are not going to come from coverage function. In particular, what is the integrality gap of the convex program for \covmp?}

\knote{What is the approximation factor of CKR rounding for Hypergraph-Multiway-Partition? Chekuri-Ene say that it is at most $3/2$ but they analyze a different rounding. Can we figure out the edge-by-edge analysis? This analysis would be a helpful step towards understanding the same rounding for \covmp. If we can show that this rounding achieves a $5/4$-approximation for \covmp, then it would imply that we cannot construct integrality gap examples for the convex program via the the graph coverage function.}
\fi

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
%In this work, we investigated the approximability of \monosubmp. 
%We exploited monotonicity to design rounding algorithms for the convex relaxation that achieves better approximation guarantees than 
In this work, we improved on both the approximation factor and the inapproximability of \monosubmp. Further, our results for \gcovmp shows a separation of the problem from \mwc in terms of approximability. Our results lead to several interesting directions for future research. Firstly, can we obtain approximation guarantees for \matroidmp, \matrixmp, and \covmp that are better than the guarantee of $4/3$ for \monosubmp? Secondly, can we extend the known results for \mwc to \gcovmp? We mention two fundamental results for \mwc that do not seem to extend to \gcovmp. 
C\u{a}linescu, Karloff, and Rabani \cite{CKR00} formulated a linear programming relaxation for \mwc that is referred to in the literature as the CKR-relaxation. A similar LP-relaxation can also be formulated for \gcovmp (it has the same constraints but different objective)---see \ref{LP:gcovmp}. Firstly, the integrality gap of the CKR-relaxation for $k=3$ terminals has been determined exactly  \cite{kkrsty, CCT06}. However, we are unable to determine the integrality gap of \ref{LP:gcovmp} for $k=3$ terminals. This is because 
it is unclear if the worst-case integrality gap instance for \ref{LP:gcovmp} will be \emph{axis-aligned} (as is the case for the CKR-relaxation). 
%we are unable to prove the \emph{axis-aligned property} of the worst-case gap instance of the CKR-relaxation. 
%which was the key to reducing the problem to an axis-aligned simplex partitioning problem and reducing the search space. 
Secondly, the inapproximability factor of \mwc is known to coincide with the integrality gap of the CKR-relaxation \cite{MNRS08}. We are unable to show a similar connection between the inapproximability factor of \gcovmp and the integrality gap of \ref{LP:gcovmp}. This is because we do not have a metric associated with edge costs in the coverage setting. The issue underlying our inability to extend both results seem related. Extending either of these results from \mwc to \gcovmp would reveal further similarities/differences between the two problems.

==> graph-coverage-MP-backup.tex <==
\section{Graph Coverage Multiway Partition}
\label{sec:graph-coverage-mp}
% \knote{Define the problem. Is it NP-hard? No PTAS? Explain these aspects. }
% \knote{State the approximation result.}

We recall the \gcovmp problem. We are given a graph $G = (V, E, w)$ where $V$ is the set of vertices, $E$ is the set of edges, and $w : E \to \R_+$ is the edge weight function \knote{I prefer to use edge cost function $c:E\to \R_+$ - general convention is to use cost for minimization problems and weights for maximization problems---e.g., min-cost spanning tree and max-weight matching}, and a set of terminal vertices $T = \{t_i : i \in [k]\}$. The goal is to find
\begin{align*}
    \min \left\{\sum_{i=1}^k f(S_i) : S_1, \cdots, S_k \text{ is a partition of $V$ }, t_i \in S_i \forall i \in [k]\right\},
\end{align*}
where $f : 2^V \to \R_+$ is the graph coverage function given by, 
\begin{align*}
    f(S) := \sum_{e = (u, v) \in E : \{u, v\}\cap S\neq \emptyset} w_e.
\end{align*}
\knote{We observe} Observe that in the objective function an edge $e = (u, v)$ is counted once if both its endpoints lie inside the same partition, and is counted twice if they lie in different partitions. 
Let $S_1, \ldots, S_k$ be a partition of $V$. Let $\delta(S_1, \ldots, S_k):=\{e\in E: e\in delta(S_i)\cap \delta(S_j)\text{ for distinct }i, j\in [k]\}$. Then, for a partition $S_1, \ldots, S_k$ of $V$, the objective can be rewritten as, 
\begin{align*}
    \sum_{i=1}^k f(S_i) &= 2\sum_{e \in \delta(S_1, \cdots, S_k)} w_e + \sum_{e \notin \delta(S_1, \cdots, S_k)}w_e 
    = \sum_{e \in \delta(S_1, \cdots, S_k)} w_e + \sum_{e \in E} w_e.
\end{align*}
Hence, the objective function of \gcovmp is a shifted version of the \mwc objective function. Since solving \mwc is NP-hard, it follows that \gcovmp is also a NP-hard problem. It was shown in \cite{cmplx-mwc} that \mwc does not admit a PTAS. Their reduction can be adapted to also conclude that \gcovmp is also APX-hard (see Theoerm \ref{thm:apx-hardness}). 
%We show that this can be extended to \gcovmp using an approach similar to \cite{cmplx-mwc}.
We focus on the approximability of \gcovmp. The following proposition is easy. 
\begin{proposition}
If we have an $\alpha$-approximation for \mwc, then we have a $(1+\alpha)/2$-approximation for \gcovmp. 
\end{proposition}
\donote{Include the proof.}

\knote{Consider rounding by picking $\theta\in [0,1]$ uniformly. Then, we should have the following claim: $1+Pr(u, v\text{ is cut})\le (5/4)(1+||x_u-x_v||_1)$. 
This claim is equivalent to showing that the expected coverage of an edge is at most $5/4$ times the LP-coverage of the edge. 
Prove this claim independently/adapt the proof of CKR to fit this directly. 
Does the proof give any ideas to improve the approximation factor for \monosubmp to $5/4$? Perhaps, the proof gives a counterpart of Lemma 2.1 for $\delta\ge 0$?}

\knote{I think rounding by picking $\theta\in [0,1]$ uniformly should also give a $5/4$-approximation for \covmp --- easy to see for \gcovmp by previous remark; same proof ideas should go through for hypergraphs as well. Verify. 

If the above is true and if $4/3$ is tight for \monosubmp, then the hard instances are not going to come from coverage function. In particular, what is the integrality gap of the convex program for \covmp?}

\subsection{APX-hardness}
In this section, we show that \gcovmp is APX-hard for every $k\ge 3$. 
\begin{theorem}\label{thm:apx-hardness}
    For any \knote{every} \knote{Writing convention: avoid using `any' while writing math. It can mean `some' and `every' based on context and this can lead to ambiguity. } $k \geq 3$, \gcovmp with $k$ terminals is APX-hard.
\end{theorem}
\begin{proof}
    We will show this via a linear reduction from \maxcut (an APX-complete problem). Consider the gadget graph shown in fig. \ref{fig:gadget_graph} \knote{Figure \ref{fig:gadget_graph}} with $9$ vertices and $3$ terminals. Now, given an instance $G$ of \maxcut, we define an instance $F$ of \gcovmp for $k=3$ as follows, 
    \begin{enumerate}
        \item Add the set of vertices of $G$ to $F$ along $3$ terminals $s_1, s_2, s_3$. \knote{Unclear} 
        \item For each $(u, v) \in E(G)$, add a gadget graph where $x = u, y = v$ and the $4$ unlabelled vertices in gadget are new dummy vertices. 
    \end{enumerate}

       
\begin{figure}[h]
    \centering
    \input{gadget-snp-hard}
    \caption{Gadget graph with terminals $s_1, s_2, s_3$ and two specified vertices $x, y$. Twelve edges incident on terminals have weight $4$ and the remaining $6$ unlabelled edges have weight $1$.}
    \label{fig:gadget_graph}
\end{figure}

    For a linear reduction, we need the following properties to hold, 
    \begin{enumerate}[label=Property \arabic*.,itemindent=*]
        \item $OPT_{3-terminal-\gcovmp} \leq \alpha \cdot OPT_{\maxcut}$ for some constant $\alpha$. \label{prop:red1}
        \item Let $y$ be cost of feasible solution to $F$ and $x$ be the cut of corresponding \maxcut obtained from $G$ by cutting $(u, v)$ iff copies of $u, v$ are assigned to different terminals in graph coverage instance, then 
        $|x - OPT_{\maxcut}| \leq \beta \cdot |y - OPT_{3-terminal-\gcovmp}|$ for some constant $\beta$. \label{prop:red2}
    \end{enumerate}

    First we shall show \ref{prop:red1}
    % \begin{lemma}
    %     \label{lem:reduction-const}
    %     (\cite{cmplx-mwc})
    %     Given a \maxcut instance $G$ and corresponding 3-way-\mwc instance $F$ any solution of \maxcut with cost $K$ can be converted to a solution of 3-way-\mwc with cost $28|E(G)|-K$ and vice-versa.
    % \end{lemma}
    We need a lemma from \cite{cmplx-mwc} to get started.
    \begin{lemma}\label{lem:reduction-cov} $G$ has a cut of size $K$ or greater if and only if $F$ has a $3$-terminal cut of weight $B = 28|E(G)|-K$ or less.
    \end{lemma}

    \begin{corollary} \label{cor:rel-mwc-cut}
        $OPT_{3-way-\mwc} = 28|E(G)| - OPT_{\maxcut}$.
    \end{corollary}
    \begin{proof}
        Let $K$ be cost of optimal cut for $G$. Let there exist a 3-way-cut with cost $B < 28|E(G)| - K$. Then, from lemma \ref{lem:reduction-cov}, there exists a cut with cost $K' > 28|E(G)| - B > K$, giving a contradiction. Moreover, from lemma \ref{lem:reduction-cov} there exists a solution to $3$-way-\mwc with cost atmost $28|E(G)| - K$. 
    \end{proof}
    

    Using corollary \ref{cor:rel-mwc-cut}, we get, $OPT_{3-way-\mwc} = 28|E(G)| - OPT_{\maxcut}$. Now, in graph $F$ we have that the total weight of all edges is $|E(G)| \cdot w(E(Gadget))$, i.e., $w(E(F)) = 54|E(G)|$.
    \begin{align} \label{eq:cut-term}
        OPT_{3-terminal-\gcovmp} &= OPT_{3-way-\mwc} + w(E(F)) \notag\\ 
        &= 54|E(G)| + 28|E(G)| - OPT_{\maxcut} \notag\\
        &= 82|E(G)| - OPT_{\maxcut}.
    \end{align}
         
    
    Since $OPT_{\maxcut} \geq \frac{|E(G)|}{2},$
    \begin{align*}
        OPT_{3-terminal-\gcovmp} &\leq 82(2 \cdot OPT_{\maxcut}) - OPT_{\maxcut} = 163 \cdot OPT_{\maxcut}.
    \end{align*} 
    Now we shall show \ref{prop:red2}
    Given a solution with cost $y$ to $3$-terminal-\gcovmp, the corresponding $3$-way-\mwc cost is $y - w(E(F)) = y - 56|E(G)|$. Now using lemma \ref{lem:reduction-cov}, we get a solution to \maxcut instance corresponding to $G$ with cost $x$ such that
    \begin{align*}
        &x \geq 28|E(G)| - (y - 56|E(G)|)\\
        \implies &x \geq 82|E(G)| - y.
    \end{align*}
    Hence we get, 
    \begin{align*}
        |x - OPT_{\maxcut}| &= OPT_{\maxcut} - x  \\
        &\leq OPT_{\maxcut} - 82|E(G)| + y \\ 
        &= y - OPT_{3-terminal-\gcovmp} \quad \quad \text{(from equation (\ref{eq:cut-term}))}\\
        &= |y - OPT_{3-terminal-\gcovmp}|.
    \end{align*}
\end{proof}



\subsection{Algorithm}
\donote{Do the edits suggested in this section.}
Next, we will prove theorem \ref{thm:graph-coverage-upper-bound} \knote{Theorem \ref{thm:graph-coverage-upper-bound}}. We will apply the simplex partitioning algorithm for graph multiway cut given by \cite{smplx-mwc}, with a slightly different analysis to show the required approximation factor. Consider the following relaxation of \gcovmp (denoted \gcovrel): 
\begin{align*}
    \min \quad &\frac{1}{2} \sum_{e \in E}w_e \lVert x_u - x_v \rVert_1 + \sum_{e \in E} w_e \\ 
    &x_u \in \Delta_k \quad \quad \forall u \in V \\ 
    &x_{t_i} = e_i \quad \quad \forall i \in [k]
\end{align*}
where $\Delta_k$ denotes the $k$-simplex, i.e. $x \in \Delta_k$ iff $x \in \R^k, \sum_i x_i = 1, x \geq 0$ \knote{$\Delta_k:=\{x\in \R^k: \sum_{i=1}^k x_i = 1, x\ge 0\}$} and $e_i$ denotes the unit vector in $\R^k$ with $1$ at the $i$-th index. 
\knote{I would prefer to write the objective as $(1/2)\sum_{e=uv\in E}w_e\sum_{i=1}^k \max\{x_u^i, x_v^i\}$. Also, leave the analysis below as it is, but create a new copy and do the analysis wrt this objective function directly.}
Below is the algorithm for \gcovmp:
% \knote{State the LP for \gcovmp.}
\begin{algorithm}[H] 
\caption{\gcovmp Simplex Partitioning}\label{alg:gcov}
\begin{algorithmic}
    \State Let $\vx$ be an optimal solution to \gcovrel
    \State Choose i.i.d random variables $Z_i \sim \exp(1)$ for $i \in [k]$
    \State $\forall u \in V$ : $l(u) = \argmin\{\frac{Z_i}{(x_u)_i} : i \in [k]\}$
    \State \Return The assignment $l : V \to [k]$
    
\end{algorithmic}
\end{algorithm}

\subsection{Approximation Factor Analysis}
Let us denote $x_u = (u_1, \cdots, u_k)$ for all $u \in V$. Let $\epsilon_{uv} := \frac{1}{2} \lVert x_u - x_v \rVert_1$.
\begin{lemma} \label{lem:u-v-sum}
    $\sum_{j=1}^k \max\{0, v_j - u_j\} = \epsilon_{uv}$.
\end{lemma}
\begin{proof}
    Since $x_u, x_v \in \Delta_k$, $\sum_{j=1}^{k} u_j = \sum_{j=1}^{k} v_j = 1$. Hence we get, 
    \begin{align} \label{eq:u-v}
        \sum_{j=1}^{k} (u_j - v_j) = 0.
    \end{align}
    Further we have,
    \begin{align*}
        \sum_{j=1}^{k} |v_j - u_j| &= \sum_{j : v_j \geq u_j} (v_j - u_j) + \sum_{j : v_j < u_j} (u_j - v_j)\\ 
        &= 2\sum_{j:v_j \geq u_j} (v_j - u_j) + \sum_{j=1}^{k} (u_j - v_j) \\ 
        &= 2 \sum_{j=1}^{k} \max\{0, v_j - u_j\}. \quad \quad \text{(from equation (\ref{eq:u-v}))}
    \end{align*}
    Hence, 
    \begin{align*}
        \epsilon_{uv} = \frac{1}{2} \lVert x_u - x_v \rVert_1 = \sum_{j=1}^{k} \max\{0, v_j - u_j\}.
    \end{align*}
\end{proof}

\begin{lemma}
    For $(u, v) \in E$, $Pr(l(u) \neq l(v)) \leq \frac{2\epsilon_{uv}}{1 + \epsilon_{uv}}$.
\end{lemma}
\begin{proof}
    Let $A_i$ denote the event that $l(u) = l(v) = i$. Then we get, 
    \begin{align*}
        Pr[A_i] &= Pr\left[\frac{z_i}{u_i} \leq \min\left\{\frac{z_1}{u_1}, \cdots, \frac{z_{i-1}}{u_{i-1}}, \frac{z_{i+1}}{u_{i+1}}, \cdots \right\}, \frac{z_i}{v_i} \leq \min\left\{\frac{z_1}{v_1}, \cdots, \frac{z_{i-1}}{v_{i-1}}, \frac{z_{i+1}}{v_{i+1}}, \cdots \right\} \right] \\ 
        &\geq Pr\left[\frac{z_i}{\min\{u_i, v_i\}} \leq \min\left\{\frac{z_1}{\max\{u_1, v_1\}}, \cdots, \frac{z_{i-1}}{\max\{u_{i-1}, v_{i-1}\}}, \frac{z_{i+1}}{\max\{u_{i+1}, v_{i+1}\}}, \cdots\right\}\right] \\ 
        &= \frac{\min\{u_i, v_i\}}{\left(\sum_{j \neq i} \max\{u_j, v_j\}\right) + \min\{u_i, v_i\} }\\
        &= \frac{u_i - \max\{0, u_i - v_i\}}{\left(\sum_{j \neq i} \left(u_j + \max\{0, v_j - u_j\}\right)\right) + u_i - \max\{0, u_i - v_i\} } \\ 
        &\geq \frac{u_i - \max\{0, u_i - v_i\}}{\sum_{j=1}^k \left(u_j + \max\{0, v_j - u_j\}\right) } \\ 
        &= \frac{u_i - \max\{0, u_i - v_i\}}{1 + \epsilon_{uv}}. \quad \quad \text{(from lemma \ref{lem:u-v-sum})}
    \end{align*}
    Since $A_i$ for $i \in [k]$ are mutually exclusive events,
    \begin{align*}
        Pr[l(u) = l(v)] &= \sum_{i=1}^{k} Pr[A_i]. 
    \end{align*}
    Hence, 
    \begin{align*}
        Pr[l(u) \neq l(v)] &= 1 - \sum_{i=1}^k Pr[A_i] \\ 
        &\leq 1 - \left(\sum_{i=1}^{k} \frac{u_i - \max\{0, u_i - v_i\}}{1 + \epsilon_{uv}}\right) \\
        &= 1 - \left(\frac{1 - \epsilon_{uv}}{1+\epsilon_{uv}}\right)
        = \frac{2\epsilon_{uv}}{1+\epsilon_{uv}}.
    \end{align*}
\end{proof} 

\begin{theorem}
    Algorithm \ref{alg:gcov} achieves an approximation of $\frac{9}{8}$ for \gcovmp.
\end{theorem}
\begin{proof}
    The expected cost of the solution given by algorithm \ref{alg:gcov} is given by, 
    \begin{align} \label{eq:exp-cost}
        \E_{Z}[cost] &= \sum_{e = (u, v) \in E} w_e \cdot (1 + Pr[l(u) \neq l(v)]) \quad \quad\text{(by linearity of expectation)} \notag\\ 
        &= \sum_{e = (u, v) \in E} w_e \cdot \left(1 + \frac{2\epsilon_{uv}}{1 + \epsilon_{uv}}\right) \notag\\ 
        &= \sum_{e = (u, v) \in E} w_e \cdot \left(\frac{1+3\epsilon_{uv}}{1 + \epsilon_{uv}}\right).
    \end{align}
    Moreover, we know that \gcovrel is a relaxation for \gcovmp. Hence, 
    \begin{align} \label{eq:opt-gcov}
        OPT_{\gcovmp} 
        &\ge \frac{1}{2}\sum_{e=(u,v) \in E} w_e \lVert x_u - x_v \rVert_1 + \sum_{e \in E} w_e \notag\\ 
        &= \sum_{e=(u,v) \in E} w_e \cdot (1 + \epsilon_{uv}).
    \end{align}
    Now, bounding the approximation factor using inequalities (\ref{eq:exp-cost}) and (\ref{eq:opt-gcov}) we get that
    \begin{align*}
        \frac{\E_{Z}[cost]}{OPT_{\gcovmp}} &\leq \frac{\sum_{e = (u, v) \in E} w_e \cdot \left(\frac{1 + 3\epsilon_{uv}}{1 + \epsilon_{uv}}\right)}{\sum_{e = (u,v) \in E} w_e \cdot (1 + \epsilon_{uv})} \\ 
        &\leq \max_{e = (u, v) \in E} \left\{\frac{1 + 3\epsilon_{uv}}{(1 + \epsilon_{uv})^2}\right\}.
    \end{align*}
    Since $\epsilon_{uv} = \frac{1}{2} \lVert x_u - x_v \rVert_1$ and $x_u, x_v \in \Delta_k$, $\epsilon_{uv} \leq \frac{1}{2}(\lVert x_u \rVert_1 + \lVert x_v \rVert_1) = 1$. Hence, $\epsilon_{uv} \in [0, 1]$ for all $(u, v) \in E$.\\
    Now, optimising $g(x) = \frac{1+3x}{(1+x)^2}$ for $x \in [0, 1]$ gives maximum value at $x = \frac{1}{3}$, with $g(\frac{1}{3}) = \frac{9}{8}$. Hence, 
    \begin{align*}
        \frac{\E_{Z}[cost]}{OPT_{\gcovmp}} \leq \frac{9}{8}.
    \end{align*}
    
\end{proof}

\knote{Discuss tightness of the analysis. Is there an example showing that the algorithm cannot achieve better than $9/8$? Even if we do not have a tight example, it is good to show some lower bound (via an example to illustrate that the algorithm cannot be better than some factor). }

\subsection{Lower Bound on Integrality Gap of the LP}
\knote{Get some integrality gap by using the instances for \mwc. What is the gap based on CKR's instance? What is the gap based on Karger et al's instance for $k=3$?}

\knote{What is the gap from Freund-Karloff instance? }

\knote{What is the gap from Cheung-Cunningham-Tang instance? }

\knote{What is the largest possible integrality gap that we can obtain by some weighting of the discretized simplex edges for $k=3$? Follow the CCT approach to solving LPs for finite discretizations and see if there is a trend in the integrality gap.}

Next we discuss a few examples to give a lower bound on the integrality gap of the LP for graph coverage. 

First, we shall analyse the integrality gap for an example shown in \cite{cualinescu1998improved}. Consider the graph $G = (V, E, w)$, $V = \{S \subseteq \{1, 2, 3\} | 1 \leq |S| \leq 2\}$, $E = \{\{S, T\} | S \neq T, | S \cap T| = 1\}$ and the set of terminals $T = \{\{1\}, \{2\}, \{3\}\}$. $w : E \to \R$ is defined as, 
\begin{align*}
  w(S, T)
  =
  \left\{
  \begin{aligned}
    1, &\qquad& |S| = |T| = 2, \\
    2,  &&  |S| = 1 \text{ or } |T| = 1.
  \end{aligned}
  \right.
\end{align*}

As shown in \cite{cualinescu1998improved}, the optimal solution to the LP places the non-terminal $\{i, j\}$ midway between terminals $\{i\}$ and $\{j\}$. This will give the fractional optimum as, 
\begin{align*}
    LP-OPT = \frac{1}{2}\left(\sum_{uv \in E} w_e \left(\sum_{i=1}^{k}\max\{x_u^i, x_v^i\}\right)\right) = 22.5
\end{align*}
Moreover, was shown in \cite{cualinescu1998improved} that the integral optimum for the objective of \mwc is $8$. Since the \gcovmp objective is shifted by $w(E)$, we get that $OPT = 23$. Hence, the integrality gap is lower bounded by, 
\begin{align*}
    \frac{OPT}{LP-OPT} &= \frac{46}{45}
\end{align*}

Next, we discuss the above example generalised to $4$ terminals. Consider the graph $G = (V, E, w)$, $V = \{S \subseteq \{1, 2, 3, 4\} | 1 \leq |S| \leq 2\}$, $E = \{\{S, T\} | S \neq T, | S \cap T| = 1\}$ and the set of terminals $T = \{\{1\}, \{2\}, \{3\}, \{4\}\}$. $w : E \to \R$ is defined as, 
\begin{align*}
  w(S, T)
  =
  \left\{
  \begin{aligned}
    1, &\qquad& |S| = |T| = 2, \\
    2,  &&  |S| = 1 \text{ or } |T| = 1.
  \end{aligned}
  \right.
\end{align*}
As shown in \cite{cualinescu1998improved}, the optimal solution to the LP yet again places the non-terminal $\{i, j\}$ midway between terminals $\{i\}$ and $\{j\}$. This gives us, 
\begin{align*}
    LP-OPT = \frac{1}{2}\left(\sum_{uv \in E} w_e \left(\sum_{i=1}^{k}\max\{x_u^i, x_v^i\}\right)\right) = 60
\end{align*}
Next, by exhaustive search, \cite{cualinescu1998improved} shows that the optimal solution to \mwc has cost $26$. Since our objective is shifted by $w(E) = 36$, we get that $OPT = 62$. Hence, the gap for this instance is, 
\begin{align*}
    \frac{OPT}{LP-OPT} &= \frac{31}{30}
\end{align*}

% Next, we examine a gap instance with $3$ terminals mentioned in \cite{kkrsty}. Let $\Delta_k = \{x \in \R^k : \sum_{i=1}^k x_i = 1, x \geq 0\}$. Consider $G_N = (V, E, w)$, where $N \in \N$. $V = \{x \in \Delta_k | x_1, x_2, x_3 \in \{\frac{k}{3N}, k \in \N\}\}$ and $E = \{\{x, y\}|\frac{1}{2}\|x-y\|_1 = \frac{1}{3N}\}$. We define the set of terminals as $\{1, 2, 3\}$ where terminal $i$ is the point in simplex with $i$-th coordinate as $1$. For any pair of distinct terminals $i, j$ and a number $d \in [0, 1]$, let $l$ be the terminal in $\{1, 2, 3\} - \{i, j\}$. Let $a$ be the point on segment $il$ at distance $d$ from $i$, and let $b$ be the point on segment $jl$ at distance $d$ from $j$. Then $p(i, j , d)$ is the union of the three segments $ia, ab$ and $bj$.

% For each distinct $i, j \in \{1, 2, 3\}$, we have $N$ copies of the path $p(i, j, 0)$, and paths $p(i, j, \frac{m}{3N})$ for $m = 1, \cdots, 2N$. We define $w_e$ as the number of paths passing through $e$. As shown in \cite{cualinescu1998improved}, the LP-cost for this embedding,  


\knote{For the integrality gap of the LP, can we reduce to understanding the discretized simplex graph? I.e., does it boil down to understanding some notion of ``coverage density'' (similar to the connection between cut density and multiway cut)?}

\knote{Richard: For \covmp, there is an instance with integrality gap at least $26/25$. Need to fill this in. }
\knote{Symmetry gap to integrality gap - does EVW's reduction give }

\subsection{Notes}
\knote{Does the UGC-hardness coincide with the integrality gap of the LP? See Manokaran, Naor, Raghavendra, Steurer.}




==> lower-bound.tex <==
\subsection{Inapproximability}\label{sec:monosubmp-inapprox}
%\donote{State the lower bound result. Prove it in subsections below.}
In this section, we prove Theorem \ref{thm:mono-sub-mp-lower-bound}. 
%\thmMonoSubMPLowerBound*
Our approach will be similar to the approaches in \cite{Vondrak, EVW}---we define a notion of \emph{symmetry gap} below; in 
%Section \ref{subsec:sym_gap_to_query-complexity}, 
Theorem \ref{thm:sym-gap-to-oracle-lower-bound}, 
we show that symmetry gap gives a lower bound on the approximation factor of algorithms with polynomial number of function evaluation queries; 
finally, in Theorem \ref{thm:large-symmetry-gap}, 
%and in Section \ref{subsec:large-symmetry-gap}, 
we construct an instance of \monosubmp that exhibits a symmetry gap of $10/9$. 
We mention that Dobzinksi and Vondr\'{a}k \cite{DV12} showed a general approach to convert query complexity based inapproximability results via the symmetry gap to computation based inapproximability results. 


%We begin by defining symmetry gap. 
\begin{definition}(Symmetry Gap) 
\label{def:instance}
\iffalse
    Let $\phi_n, \phi_t \colon [k] \rightarrow \mathbb{R}$ be given functions. 
    We set $V = [k] \times [k]$, $R_i = \{(i, j) \colon j \in [k]\}$ and $C_j = \{(i, j) \colon i \in [k]\}$, and define 
    $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ as the function  
        \[
            f_{\phi_n, \phi_t}(S) = \sum_{i = 1}^k \left(\phi_n(S \cap R_i)\indicator{(i, i)\not\in S} + \phi_t(S \cap R_i)\indicator{(i, i)\in S} + \phi_n(S \cap C_i)\indicator{(i, i)\not\in S} + \phi_t(S \cap C_i)\indicator{(i, i)\in S}\right). 
        \] 
    We define the following: 
\fi
Let $V=[k]\times [k]$ and $f: 2^V\rightarrow \R$ be a set function defined over the set $V$. 
    \begin{enumerate}
    \item For a subset $A\subseteq V$, we denote $A^T:=\{(j,i): (i,j)\in A\}$. 
    \item The set function $f$ is a row-column-type function if there exists a function $g:2^{V}\rightarrow \R_{\ge 0}$ such that $f(A)=\sum_{i=1}^k (g(A\cap R_i) + g(A\cap C_i))$ for every $A\subseteq V$, where $R_i:=\{(i, j): j\in [k]\}$ and $C_i:=\{(j,i): j\in [k]\}$ for every $i\in [k]$.
    
    %\item The set function $f$ is \emph{transpose-invariant} if $f(A)=f(A^T)$ for every $A\subseteq V$. Generalizing, we say that a function $F:[0,1]^V\rightarrow R$ is \emph{transpose-invariant} if $F(\vx)=F(\vx^T)$ for every $\vx \in [0,1]^{[k]\times [k]}$, where $\vx^T$ is the transpose of the matrix $\vx$. 
    
    \item A partition $V_1, V_2, \ldots, V_k$ of $V$ is \emph{symmetric} if  
        %$(i, j) \in V_\ell$ if and only if $(j, i) \in V_\ell$ for all $(i, j) \in V$ and $\ell \in [k]$. 
        $V_{\ell}=V_{\ell}^T$ for every $\ell \in [k]$. 
        Generalizing, we say that $\vx \in [0, 1]^{V \times [k]}$ is \emph{symmetric} if $x(*, \ell) = x(*, \ell)^T$ for every $\ell \in [k]$. 
    \item Let 
    \begin{align*}
    \opt(f) &:= \min \left\{\sum_{i = 1}^k f(V_i) \colon V_1, \ldots, V_k \text{ is a partition of } V \text{ with } (i, i) \in V_i\ \forall i \in [k]\right\},\\
    \symopt(f) &:= \min \left\{\sum_{i = 1}^k f(V_i) \colon V_1, \ldots, V_k \text{ is a symmetric partition of } V \text{ with } (i, i) \in V_i\ \forall i \in [k]\right\}, and \\
    \symgap\left(f\right) &:= \frac{\symopt(f)}{\opt(f)}. 
    \end{align*}
    \end{enumerate}
\end{definition}

Next, we prove that the approximation factor of an algorithm that makes polynomial number of function evaluation queries should be at least the symmetry gap. 

\begin{restatable}{theorem}{thmSymGapToOracleLowerBound}\label{thm:sym-gap-to-oracle-lower-bound}
    Suppose that there exists a row-column-type non-negative monotone submodular function $f\colon 2^V \rightarrow \mathbb{R}$ over the set $V=[k]\times [k]$ such that $\symgap(f)\ge \alpha$. 
    %Let $V=[k]\times [k]$ and $f\colon 2^V \rightarrow \mathbb{R}$ be a row-column-type %transpose-invariant 
    %non-negative monotone submodular function over the set $V$ such that $\symgap(f)\ge \alpha$. 
    Then, for every constant $\eps>0$, every algorithm for \monosubmp with an approximation factor of $\alpha-\epsilon$ makes $2^{\Omega(n)}$ function evaluation queries, where $n$ is the size of the ground set. 
\end{restatable}

Finally, we show that there exists a row-column-type non-negative monotone submodular function with large symmetry gap. 
\begin{restatable}{theorem}{thmLargeSymmetryGap}\label{thm:large-symmetry-gap}
    Let $V^{(k)} = [k] \times [k]$. Then, there exists a sequence $\left(f^{(k)} \colon 2^{V^{(k)}} \rightarrow \mathbb{R}_{\geq 0}\right)_{k \in \mathbb{N}}$ of row-column-type non-negative monotone submodular functions parameterized by $k$ such that 
    \[
        \lim_{k \rightarrow \infty} \symgap\left(f^{(k)}\right) = 10/9.
    \]
\end{restatable}

Theorem \ref{thm:mono-sub-mp-lower-bound} follows from Theorems \ref{thm:sym-gap-to-oracle-lower-bound} and \ref{thm:large-symmetry-gap}. We prove Theorem \ref{thm:sym-gap-to-oracle-lower-bound} in Section \ref{subsec:sym_gap_to_query-complexity} and Theorem \ref{thm:large-symmetry-gap} in Section \ref{subsec:large-symmetry-gap}. Our proof approach for Theorem \ref{thm:sym-gap-to-oracle-lower-bound} is similar to the proof approaches in \cite{Vondrak, EVW}---the result does not follow directly from the results in \cite{Vondrak, EVW} since we are interested in \monosubmp (which was not the focus of those two works), so we have to work out the details. We encourage first-time readers to skip Section \ref{thm:sym-gap-to-oracle-lower-bound}. Our main contribution is Theorem \ref{thm:large-symmetry-gap}, i.e., constructing an instance of \monosubmp with large symmetry gap. 

%\knote{Can we convert oracle hardness results to NP-hardness results as shown in \cite{EVW} and this paper: ``From Query Complexity to Computational Complexity'', Dobzinski and Vondrak?}

\input{sym-gap-to-query-lower-bound-2}

\subsubsection{Symmetry Gap}
\label{subsec:large-symmetry-gap}
%\rnote{Might need to assume $k \geq 4$. (might need $k \geq \frac{k}{2} + 2$ for Corollary \ref{cor:final_structure})}
In this section, we construct an instance of \monosubmp with large symmetry gap, i.e., prove Theorem \ref{thm:large-symmetry-gap}. We begin by defining the function of interest. 

%We prove Theorem \ref{thm:large-symmetry-gap} in 
%\thmLargeSymmetryGap*

\begin{definition}
\label{def:def:f_for_10/9}
    Let $V = [k] \times [k]$ for $k\ge 4$. For each $i, j\in [k]$, let 
    \begin{align*}
        R_i &= \{(i, j) \colon j \in [k]\},\\
        \overrightarrow{R}_i &= \{(i, j) \colon j \in \{i + 1, i + 2, \ldots, k\} \}, \\
        \overleftarrow{R}_i &= \{(i, j) \colon j \in [i - 1]\}, \text{ and}\\
        C_j &= \{(i, j) \colon i \in [k]\}. 
    \end{align*}
    We define the following functions:
    \begin{enumerate}
        \item 
        $\phi_n \colon \mathbb{R} \rightarrow \mathbb{R}_{\geq 0}$ is defined as $\phi_n(a) = \min\left\{a, \frac{7}{8}k\right\}$;

        \item 
        $\phi_t \colon \mathbb{R} \rightarrow \mathbb{R}_{\geq 0}$ is defined as $\phi_t(a) = \min\left\{\frac{3}{8}ka, \frac{3}{8}k + a - 1, \frac{7}{8}k\right\}$;

        \item 
        $g \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ is defined as
        \[
            g(S) = \begin{cases} \phi_t\left(|S|\right) & \text{if } \left\{(\ell, \ell) \colon \ell \in [k] \right\} \cap S \neq \emptyset, \\ \phi_n\left(|S|\right) & \text{otherwise}; \end{cases}
        \]
        \item 
        $f \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ is defined as 
        \[
            f(S) = \sum_{i = 1}^k \left(g(R_i \cap S) + g(C_i \cap S) \right). 
        \]
    \end{enumerate}
    We say that $P_1, \ldots, P_k$ is a symmetric multiway partition of $V$ if $P_1, \ldots, P_k$ is symmetric partition of $V$ satisfying $(\ell, \ell) \in P_\ell$ for each $\ell \in [k]$. 
\end{definition}

In Lemma \ref{lem:function-is-monotone-submodular}, we show that the function $f$ defined above is row-column-type, non-negative, monotone, and submodular. 
In Lemma \ref{lem:opt-upper-bound}, we show that $\opt(f)\le (9k^2-k)/4$. 
In Lemma \ref{lem:sym-opt-lower-bound}, we show that $\opt(f)\ge (10k^2-14k-1)/4$. 
These three lemmas together imply Theorem \ref{thm:large-symmetry-gap}. We now prove these lemmas. 

\begin{lemma}\label{lem:function-is-monotone-submodular}
    Let $V = [k] \times [k]$ and $f \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ be defined as in Definition \ref{def:def:f_for_10/9}. Then, $f$ is a row-column-type non-negative monotone submodular function. 
\end{lemma}
\begin{proof}
    From the definition of $f$, we have that $f$ is row-column-type and non-negative. Moreover, $f$ is monotone since $\phi_n$ and $\phi_t$ are monotone and $\phi_t(a) \geq \phi_n(a)$ for all $a \in \{0, \ldots, k\}$. Now we prove that $f$ is submodular. We first prove the following observations in which $a$ and $c$ are assumed to take integer values:
    \begin{enumerate}
        \item For all $a \leq c$, $\phi_n(a + 1) - \phi_n(a) \geq \phi_n(c + 1) - \phi_n(c)$.

        \item For all $a \leq c$, $\phi_t(a + 1) - \phi_t(a) \geq \phi_t(c + 1) - \phi_t(c)$. 

        \item For all $0 \leq a \leq a + 1 \leq c$, $\phi_n(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_t(c)$.

        \item For all $0 \leq a \leq c$, $\phi_t(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_n(c)$.
    \end{enumerate}
    The first two observations follow from the concavity of $\phi_n$ and $\phi_t$, respectively. 
    
    To prove that if $0 \leq a$ and $a + 1 \leq c$, then $\phi_n(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_t(c)$, we examine two cases: $a \leq \frac{7}{8}k - 1$ and $ a \geq \frac{7}{8}k$. If $a \leq \frac{7}{8}k$, then $\phi_n(a + 1) - \phi_n(a) = 1$. Additionally, because $0 \leq a$ and $a + 1 \leq c$, $c \geq 1$, it follows that $1 \geq \phi_t(c + 1) - \phi_t(c)$. If $a \geq \frac{7}{8}k$, then $\phi_n(a + 1) - \phi_n(a) = 0 = \phi_t(c + 1) - \phi_t(c)$ since $c \geq a + 1$. 

    To prove that if $0 \leq a \leq c$, $\phi_t(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_n(c)$, we examine two cases: $c \leq \frac{7}{8}k$ and $c \geq \frac{7}{8}k + 1$. If $c \leq \frac{7}{8}k$, then $\phi_n(c) - \phi_n(a) = c - a$ while $\phi_t(c + 1) - \phi_t(a + 1) \leq c - a$ since $a + 1 \geq 1$. If $c \geq \frac{7}{8}k$, then $\phi_n(c) - \phi_n(a) = \max\left\{\frac{7}{8}k - a, 0\right\}$, and since $a + 1 \geq 1$, we have that $\phi_t(c + 1) - \phi_t(a + 1) = \max \left\{\frac{k}{2} - a + 1, 0\right\}$. Hence, $\phi_n(c) - \phi_n(a) \geq \phi_t(c + 1) - \phi_t(a + 1)$. Rearranging, we obtain that $\phi_t(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_n(c)$. 

    We now prove submodularity armed with the above observations. 
    We will show that for all $X \subseteq Y \subseteq V$ and $(i, j) \in V \setminus Y$, we have that $f\left(X + (i, j)\right) - f\left(X\right) \geq f\left(Y + (i, j)\right) - f\left(Y\right)$. Let $X \subseteq Y \subseteq V$ and $(i, j) \in V \setminus Y$. We observe that $f\left(X + (i, j)\right) - f\left(X\right) = g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) + g\left(C_j \cap X + (i, j)\right) - g\left(C_j \cap X\right)$. Similarly, $f\left(Y + (i, j)\right) - f\left(Y\right) = g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right) + g\left(C_j \cap Y + (i, j)\right) - g\left(C_j \cap Y\right)$. 

    First, we will consider the case in which $i \neq j$. In particular, we show that $g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) \geq g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right)$. We let $|R_i \cap X| = a$ and $|R_i \cap Y| = c$. If $(i, i) \notin Y$, then $g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) = \phi_n(a + 1) - \phi_n(a) \geq \phi_n(c + 1) - \phi_n(c) = g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right)$. If $(i, i) \in X$, then $g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) = \phi_t(a + 1) - \phi_t(a) \geq \phi_t(c + 1) - \phi_t(c) = g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right)$. Finally, if $(i, i) \in Y \setminus X$, then $c \geq a + 1$ and $a \geq 0$, so $g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) = \phi_n(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_t(c) = g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right)$. We have shown that $g\left(R_i \cap X + (i, j)\right) - g\left(R_i \cap X\right) \geq g\left(R_i \cap Y + (i, j)\right) - g\left(R_i \cap Y\right)$ in all cases. Similar reasoning shows that $g\left(C_j \cap X + (i, j)\right) - g\left(C_j \cap X\right) \geq g\left(C_j \cap Y + (i, j)\right) - g\left(C_j \cap Y\right)$. Thus, if $i \neq j$, then $f\left(X + (i, j)\right) - f\left(X\right) \geq f\left(Y + (i, j)\right) - f\left(Y\right)$. 

    Now, we consider the case in which $i = j$. Again, we let $|R_i \cap X| = a$ and $|R_i \cap Y| = c$. Then $g\left(R_i \cap X + (i, i)\right) - g\left(R_i \cap X\right) = \phi_t(a + 1) - \phi_n(a) \geq \phi_t(c + 1) - \phi_n(c) = g\left(R_i \cap Y + (i, i)\right) - g\left(R_i \cap Y\right)$. Similar reasoning shows that $g\left(C_j \cap X + (i, i)\right) - g\left(C_j \cap X\right) \geq g\left(C_j \cap Y + (i, i)\right) - g\left(C_j \cap Y\right)$. Hence, $f\left(X + (i, i)\right) - f\left(X\right) \geq f\left(Y + (i, i)\right) - f\left(Y\right)$. 
\end{proof}

Next, we show that the function $f$ of interest to this section has small $\opt$. 
\begin{lemma}\label{lem:opt-upper-bound}
    Let $V = [k] \times [k]$ and $f \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ be defined as in Definition \ref{def:def:f_for_10/9}. Then $\opt\left(f\right) \leq \frac{9k^2 - 4k}{4}$. 
\end{lemma}
\begin{proof}
    We upper bound the optimum value by exhibiting a cheap feasible solution. Consider the partition $V_1, \ldots, V_k$ of $V$ defined by $V_i := R_i$ for all $i\in [k]$. We observe that $V_1, \ldots, V_k$ is a feasible multiway partition of $V$ with $(i,i)\in V_i$ for every $i\in [k]$. Hence, we have that
    \begin{align*}
        \opt(f)
        \le \sum_{\ell = 1}^k f(V_\ell) 
        &= \sum_{\ell = 1}^k \sum_{i = 1}^k \left(g(R_i \cap V_\ell) + g(C_i \cap V_\ell) \right) \\
        &= \sum_{\ell = 1}^k \sum_{i = 1}^k \left(g(R_i \cap R_\ell) + g(C_i \cap R_\ell)\right) \\
        &= \sum_{\ell = 1}^k \left( \phit{R_\ell \cap R_\ell} + \phit{\{(\ell, \ell)\}} + \sum_{i \neq \ell} \phin{\{(\ell, i)\}} \right) \\
        &= \sum_{\ell = 1}^k \left( \frac{7}{8}k + \frac{3}{8}k + k - 1 \right) \\
        &= k\left(\frac{18}{8}k - 1\right) \\
        &= \frac{9k^2 - 4k}{4}.
    \end{align*}
    %Hence, $\opt\left(f\right) \leq \frac{9k^2 - 4k}{4}$. 
\end{proof}

Finally, we show that the function $f$ of interest to this section has large $\symopt$. The proof of the following lemma is non-trivial and we devote Section \ref{sec:sym-opt-lower-bound} to prove it. 
\begin{lemma}\label{lem:sym-opt-lower-bound}
Let $V = [k] \times [k]$ and $f \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ be defined as in Definition \ref{def:def:f_for_10/9}. Let $Q_1, \ldots, Q_k$ be a symmetric multiway partition of $V$. Then, $\sum_{\ell = 1}^k f(Q_\ell) \geq \frac{10k^2 - 22k - 1}{4}$ % \rnote{I think this should be $\frac{10k^2 - 22k - 1}{4}$}. 
\end{lemma}
%We devote Section \ref{sec:sym-opt-lower-bound} to prove Lemma \ref{lem:sym-opt-lower-bound}.  
\iffalse
\begin{proof}
    \donote{}
    
\end{proof}
\fi

\subsubsection{Proof of Lemma \ref{lem:sym-opt-lower-bound}}\label{sec:sym-opt-lower-bound}
In order to prove Lemma \ref{lem:sym-opt-lower-bound}, we first show a lower bound on the objective value of certain structured symmetric multiway partitions (see Lemma \ref{lem:structured-sym-opt-lower-bound}). Next, we show that every symmetric multiway partition can be converted to a structured symmetric multiway partition with a small additive loss (see Lemma \ref{lem:sym_part_structure}). See Figure \ref{fig:sym-part-structure} for an illustration of the structured symmetric multiway partition of interest that will be of interest to this section. 
For notational convenience, we define the objective value of a symmetric multiway partition $P_1, \ldots, P_k$ of $V$ as follows: 
\begin{align*}
    \obj{P_1, \ldots, P_k} &= \frac{1}{2} \sum_{\ell = 1}^k f(P_\ell).
\end{align*}
We observe that 
\begin{align*}
\obj{P_1, \ldots, P_k}
        &= \sum_{i = 1}^k \left(\phi_t\left(|R_i \cap P_i|\right) + \sum_{\ell \in [k] \setminus \{i\}} \phi_n\left(|R_i \cap P_\ell)\right)\right). 
\end{align*}

\begin{figure}[ht]
\centering
\begin{tikzpicture}
    \definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
    
    % Define grid size
    \def\gridsize{9}
    \def\spacing{0.9} % Distance between points

    % Draw the grid of vertices
    \foreach \x in {1,...,\gridsize} {
        \foreach \y in {1,...,\gridsize} {
            % Draw regular black vertices
            \filldraw[black] (\x*\spacing, \y*\spacing) circle (2pt);
        }
    }
    % coloring L's
    
    \foreach \i/\c in {0/red, 1/orange, 2/yellow, 3/green, 4/blue}{
    \fill[\c, opacity=0.4] (\i*\spacing + 0.5*\spacing, \gridsize*\spacing-0.5*\spacing - \i*\spacing) rectangle (\gridsize*\spacing+0.5*\spacing, \gridsize*\spacing+0.5*\spacing - \i*\spacing);

    \fill[\c, opacity=0.4] (0.5*\spacing + \i*\spacing, 0.5*\spacing) rectangle (1*\spacing+0.5*\spacing + \i*\spacing, \gridsize*\spacing+0.5*\spacing - \spacing - \i*\spacing);
    }

    % remaining vertices
    
    \foreach \i/\c in {5/brightube, 6/gray, 7/brown, 8/black}{
        \foreach \j in {5, 6, 7, 8}{
                \ifthenelse{\i=\j}{\fill[\c, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);}{\fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);}
        }
    }
\end{tikzpicture}
\caption{A figure illustrating the structure that will be obtained in Lemma \ref{lem:sym_part_structure}. Each color corresponds to a part in the symmetric multiway partition. In particular, $i^*=5$ in this symmetric multiway partition.}
\label{fig:sym-part-structure}
\end{figure}

\begin{lemma}\label{lem:structured-sym-opt-lower-bound}
Let $V = [k] \times [k]$ and $f \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ be defined as in Definition \ref{def:def:f_for_10/9}. Let $Q_1, \ldots, Q_k$ be a symmetric multiway partition of $V$ for which there exists $i^* \in [k]$ such that $\overrightarrow{R}_i \subseteq Q_i$ for all $i \in [i^*]$ and $\overrightarrow{R}_i \subseteq Q_1$ for all $i \in [k] \setminus [i^*]$. Then, $\sum_{\ell = 1}^k f(Q_\ell) \geq \frac{10k^2 - 6k - 1}{4}$. 
\end{lemma}
\begin{proof}
    We have that 
    \begin{align}
        \obj{Q_1, \ldots, Q_k} = \sum_{i = 1}^k \left(\phit{R_i \cap Q_i} + \sum_{\ell \in [k] - i} \phin{R_i \cap Q_\ell}\right). \label{eq:obj-expression}
    \end{align}
    Let $i \in [i^*]$. Then, we have that $R_i\cap Q_i=\overrightarrow{R}_i\cup\{(i,i)\}$. Moreover, we have $R_i\cap Q_{\ell}=\{(i, \ell)\}$ for every $\ell\in [i-1]$ and $R_i\cap Q_{\ell}=\emptyset$ for every $\ell\in \{i,\ldots, k\}$. Hence, for every $i\in [i^*]$, we have that 
    \begin{align}
        \phit{R_i \cap Q_i} + \sum_{\ell \in [k] - i} \phin{R_i \cap Q_\ell} &= \phi_t(k + 1 - i) + (i - 1)\phi_n(1) \notag\\
        &= \phi_t(k + 1 - i) + (i - 1). \label{eq:smaller-than-i*}
    \end{align}
    Let $i \in \{i^* + 1, \ldots, k\}$. Then, we have that $R_i\cap Q_i=\{(i,i)\}$. Moreover, we have that $R_i\cap Q_{1}=\overrightarrow{R}_i$, $R_i\cap Q_{\ell}=\{(i, \ell)\}$ for every $\ell\in \{2, \ldots, i^*\}$ and $R_i\cap Q_{\ell}=\emptyset$ for every $ell\in \{i^*+1, \ldots, k\}$. Hence, for every $i\in \{i^*+1, \ldots, k\}$, we have that 
    \begin{align}
        \phit{R_i \cap Q_i} + \sum_{\ell \in [k] - i} \phin{R_i \cap Q_\ell} &= \phi_t(1) + \phi_n\left(k - i^*\right) + \left(i^* - 1\right)\phi_n(1) \notag\\
        &= \frac{3}{8}k + \phi_n\left(k - i^*\right) + \left(i^* - 1\right). \label{eq:larger-than-i*}
    \end{align}
    We consider three cases based on the value of $i^*$ and show the lower bound in all three cases. %(i) $i^* \leq \frac{1}{8}k$, $\frac{1}{8}k < i^* \leq \frac{k}{2}$, and $\frac{k}{2} < i^*$. 
    
    \noindent\textbf{Case 1.} Suppose that $i^* \leq \frac{1}{8}k$. Then, we have $\phi_t(k + 1 - i) = \frac{7}{8}k$ for each $i \in [i^*]$ and $\phi_n(k - i^*) = \frac{7}{8}k$. Hence, by \eqref{eq:obj-expression}, \eqref{eq:smaller-than-i*}, and \eqref{eq:larger-than-i*}, we have that 
    \begin{align}
        \obj{Q_1, \ldots, Q_k} &= \sum_{i = 1}^{i^*} \left(\frac{7}{8}k + i - 1\right) + \left(k - i^*\right)\left(\frac{3}{8}k + \frac{7}{8}k + i^* - 1\right) \notag\\
        &= ki^* - k - \left(i^*\right)^2 + i^* + \frac{1}{8}\left(4(i^*)^2-3ki^*-4i^* + 10k^2\right). \label{eq:obj-small-i*}
    \end{align}
    Taking the derivative with respect to $i^*$, we have 
    \[
        \frac{\partial\obj{Q_1, \ldots, Q_k}}{\partial i^*} = -i^* + \frac{5}{8}k + \frac{1}{2} \geq \frac{k}{2} + \frac{1}{2} \geq 0,
    \]
    where the first inequality is because $i^*\le \frac{1}{8}k$. 
    Hence, for $i^* \leq \frac{1}{8}k$, the minimum value of $\obj{Q_1, \ldots, Q_k}$ is is attained at $i^* = 1$. Substituting $i^*=1$ in \eqref{eq:obj-small-i*}, we obtain that 
    \[
        \obj{Q_1, \ldots, Q_k} \geq k - k - 1 + 1 + \frac{1}{8}\left(4 - 3k - 4 + 10k^2\right) = \frac{10k^2 - 3k}{8}.
    \]

    \noindent\textbf{Case 2.} Suppose that $\frac{1}{8}k < i^* \leq \frac{k}{2}$. Then, $\phi_t(k + 1 - i) = \frac{7}{8}k$ and $\phi_n(k - i^*) = k - i^*$. Hence, by \eqref{eq:obj-expression}, \eqref{eq:smaller-than-i*}, and \eqref{eq:larger-than-i*}, we have that 
    \begin{align}
        \obj{Q_1, \ldots, Q_k} &= \sum_{i = 1}^{i^*} \left(\frac{7}{8}k + i - 1\right) + \left(k - i^*\right)\left(\frac{3}{8}k + k - i^* + i^* - 1\right) \notag\\
        &= \sum_{i = 1}^{i^*} \left(\frac{7}{8}k + i - 1\right) + \left(k - i^*\right)\left(\frac{11}{8}k - 1\right) \notag\\
        &= \frac{1}{2}\left((i^*)^2 - i^*\right) + \frac{1}{8}\left(11k^2 - 4ki^*\right) - k + i^*. \label{eq:medium-i*}
    \end{align}
    Taking the derivative with respect to $i^*$, we have 
    \[
        \frac{\partial\obj{Q_1, \ldots, Q_k}}{\partial i^*} = i^* + \frac{1}{2} - \frac{k}{2}. 
    \]
    We observe that $\frac{\partial^2\obj{Q_1, \ldots, Q_k}}{\partial (i^*)^2} = 1$, so $\obj{Q_1, \ldots, Q_k}$ is a convex function of $i^*$. Hence, for $\frac{1}{8}k < i^* \leq \frac{k}{2}$, the minimum value for $\obj{Q_1, \ldots, Q_k}$ is attained at $i^* = \frac{k}{2} - \frac{1}{2}$. Thus, evaluating the expression \eqref{eq:medium-i*} at $i^* = \frac{k}{2} - \frac{1}{2}$, we obtain that
    \[
        \obj{Q_1, \ldots, Q_k} \geq \frac{10k^2 - 6k - 1}{8}.
    \]

    \noindent\textbf{Case 3.} Suppose that $\frac{k}{2} < i^*$. Then, 
    \begin{align*}
    \phi_t(k + 1 - i) &= \begin{cases} \frac{7}{8}k & i \leq \frac{k}{2} \\ \frac{11}{8}k - i & i > \frac{k}{2}\end{cases} \text{ and}\\
    \phi_n(k - i^*) &= k - i^*.
    \end{align*}
    Hence, by \eqref{eq:obj-expression}, \eqref{eq:smaller-than-i*}, and \eqref{eq:larger-than-i*}, we have that 
    \begin{align*}
        \obj{Q_1, \ldots, Q_k} &= \sum_{i = 1}^{\frac{k}{2}} \left(\frac{7}{8}k + i - 1\right) + \sum_{i = \frac{k}{2} + 1}^{i^*} \left(\frac{11}{8}k - i + i - 1 \right) + \left(k - i^*\right)\left(\frac{3}{8}k + k - i^* + i^* - 1\right) \\
        &= \sum_{i = 1}^{\frac{k}{2}} \left(\frac{7}{8}k + i - 1\right) + \left(i^* - \frac{k}{2}\right)\left(\frac{11}{8}k - 1\right) + \left(k - i^*\right)\left(\frac{11}{8}k - 1\right) \\
        &= \sum_{i = 1}^{\frac{k}{2}} \left(\frac{7}{8}k + i - 1\right) + \left(\frac{k}{2}\right)\left(\frac{11}{8}k - 1\right) \\
        &= \frac{10k^2 -6k}{8}. 
    \end{align*}
    \iffalse
    Hence, in all cases, $\obj{Q_1, \ldots, Q_k} \geq \frac{10k^2 - 6k - 1}{8}$. This demonstrates that 
    \[
        \sum_{\ell = 1}^k f(Q_\ell) = 2\obj{Q_1, \ldots, Q_k} \geq \frac{10k^2 - 6k - 1}{4}.
    \]
    \fi
\end{proof}

The following lemma shows that every symmetric multiway partition can be converted to a structured symmetric multiway partition with a small additive loss in the objective. 
\begin{restatable}{lemma}{lemSymPartStructure}
\label{lem:sym_part_structure}
    Let $V = [k] \times [k]$. Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$. Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ with the following properties:
    \begin{enumerate}
        \item 
        $\sum_{\ell = 1}^k f(Q_\ell) \leq \sum_{\ell = 1}^k f(P_\ell) + 2k$ and 

        \item 
        There exists $i^* \in [k]$ such that $\overrightarrow{R}_i \subseteq Q_i$ for all $i \in [i^*]$ and $\overrightarrow{R}_i \subseteq Q_1$ for all $i \in [k] \setminus [i^*]$.
    \end{enumerate}
\end{restatable}
Lemmas \ref{lem:structured-sym-opt-lower-bound} and \ref{lem:sym_part_structure} together complete the proof of Lemma \ref{lem:sym-opt-lower-bound}. The rest of this section is devoted to proving Lemma \ref{lem:sym_part_structure}. For the rest of this section, let $V:=[k]\times [k]$.
We will denote a symmetric multiway partition of $V$ satisfying the second condition of Lemma \ref{lem:sym_part_structure} as a \emph{structured symmetric partition} (see Figure \ref{fig:sym-part-structure} for an example). 
To prove Lemma \ref{lem:sym_part_structure}, we will prove several claims about how symmetric multiway partitions of $V = [k] \times [k]$ can be transformed into a structured symmetric multiway partitions without increasing the cost of the partition by more than $2k$.
% For notational convenience, we define the objective value of a symmetric multiway partition $P_1, \ldots, P_k$ of $V$ as follows: 
% \begin{align*}
%     \obj{P_1, \ldots, P_k} &= \frac{1}{2} \sum_{\ell = 1}^k f(P_\ell).
% \end{align*}
% We observe that 
% \begin{align*}
% \obj{P_1, \ldots, P_k}
%         &= \sum_{i = 1}^k \left(\phi_t\left(|R_i \cap P_i|\right) + \sum_{\ell \in [k] \setminus \{i\}} \phi_n\left(|R_i \cap P_\ell)\right)\right). 
% \end{align*}

The requirement for structured symmetric multiway partition for $i=1$ is that $R_1\subseteq Q_1$. 
We begin with Claim \ref{claim:move-first-row} below which shows that this property can be achieved for $i=1$ with an additive loss in the objective value. We emphasize that Claim \ref{claim:move-first-row} will be the only transformation that incurs a loss in the objective value. The rest of the transformations will transform \emph{partially} structured symmetric partition into a fully structured symmetric partition (as desired in Lemma \ref{lem:sym_part_structure}) without any loss in the objective value. 
\begin{claim}\label{claim:move-first-row}
Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$. Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that 
\begin{enumerate}
    \item $R_1\subseteq Q_1$ and
    \item $\obj{Q_1,\ldots, Q_k} \le \obj{P_1, \ldots, P_k} + k$. 
\end{enumerate}
\end{claim}
\begin{proof}
    We define $Q_1, \ldots, Q_k$ as $Q_1 := P_1 \cup R_1$, and $Q_\ell := P_\ell \setminus R_1$ for each $\ell \in \{2, 3, \ldots, k\}$. The resulting partition $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$ with $R_1\subseteq Q_1$. It remains to bound the objective value of $Q_1, \ldots, Q_k$. 
    For each $i \in \{2, 3,\ldots, k\}$ and $\ell \in [k]$, we have $R_i \cap Q_\ell$ = $R_i \cap P_\ell$. Hence, we have that 
    \begin{align*}
        \obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} &= \phi_t\left(|R_1 \cap Q_1|\right) + \sum_{\ell = 2}^k \phi_n\left(|R_1 \cap Q_\ell|\right) \\
        & \quad \quad \quad \quad - \phi_t\left(|R_1 \cap P_1|\right) - \sum_{\ell = 2}^k \phi_n\left(|R_1 \cap P_\ell|\right) \\
        &\leq k + 0 - 0 - 0=k. 
    \end{align*}
\end{proof}

The rest of the proof of Lemma \ref{lem:sym_part_structure} involves transforming a partially structured symmetric partition into a structured symmetric partition without any loss in the objective value. For this, we introduce the notion of unhappy elements. 
    
\begin{definition}[unhappy elements]
\label{def:unhappy}
    Let $P_1, \ldots, P_k$ be a partition of $V$. An element $(i, j) \in V$ is \emph{unhappy under $P_1, \ldots, P_k$} if $(i, j) \in P_\ell$ where $\ell \notin \{i, j\}$. Moreover, let 
    \[
    U(P_1, \ldots, P_k) := \{(i, j) \in [k]\times [k] \colon  (i, j) \text{ is unhappy under } P_1, \ldots, P_k\}. 
    \]
\end{definition}

We now show that unhappy elements can be moved to the first part of a partially structured partition without increasing the objective value. 
%We note that $U(P_1, \ldots, P_k)\subseteq P_1$ implies that $R_1\subseteq P_1$ \rnote{I don't think this is true since e.g. $(1, 2) \in P_2$ would not be unhappy}, so the following claim can be viewed as a strengthening of Claim \ref{claim:move-first-row}. 
\begin{claim}
\label{claim:move-unhappy}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ such that $R_1 \subseteq P_1$. 
    Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that 
    %For $U:=U(P_1, \ldots, P_k)$, let $Q_1 := P_1 \cup U$, and $Q_{\ell} := P_{\ell} \setminus U$ for each $\ell\in \{2,3,\ldots, k\}$. Then, 
    \begin{enumerate}
        \item $R_1 \subseteq Q_1$, 
        \item $U(Q_1, \ldots, Q_k)\subseteq Q_1$, and 
        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
    \end{enumerate}
\end{claim}
\begin{proof}
For $U:=U(P_1, \ldots, P_k)$, let $Q_1 := P_1 \cup U$, and $Q_{\ell} := P_{\ell} \setminus U$ for each $\ell\in \{2,3,\ldots, k\}$. Then, $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$     The first two properties follow by definition of $Q_1, \ldots, Q_k$. It suffices to bound the objective value. 
We have that 
    \begin{align*}
        \obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} 
        &= \sum_{i = 1}^k \sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right).
        %&= \sum_{\ell = 1}^k \left(g(R_1 \cap Q_\ell) - g(R_1 \cap P_\ell)\right) 
         %\quad \quad \quad \quad 
         %+ \sum_{i = 2}^k \sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right). 
    \end{align*}
In order to complete the proof, we show that  $\sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right)\le 0$ for each $i\in [k]$. 

First, we consider $i = 1$. 
    \begin{align*}
        \sum_{\ell = 1}^k \left(g(R_1 \cap Q_\ell) - g(R_1 \cap P_\ell)\right) = \phit{R_1 \cap Q_1} - \phit{R_1 \cap P_1} + \sum_{\ell \neq 1} \left(\phin{R_1 \cap Q_\ell} - \phin{R_1 \cap P_\ell}\right) = 0,
    \end{align*}
    since $R_1 \subseteq P_1$ and $R_1 \subseteq Q_1$ implies that $|R_1 \cap Q_1| = |R_1 \cap P_1| = k$ and $|R_1 \cap Q_\ell| = |R_1 \cap P_\ell| = 0$ for each $\ell \in \{2, 3, \ldots, k\}$. 

Next, %we show that $\sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right) \leq 0$ for each $i\in \{2, \ldots, k\}$. Let 
let $i \in \{2, \ldots, k\}$. We need to show that $\sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right) \leq 0$. 
    We begin by showing that 
    \begin{align}
        |R_i\cap P_{\ell}|\le |R_i\cap Q_1| \text{ for each } \ell\in [k]\setminus \{1, i\}. \label{ineq:set-sizes}
    \end{align}
    We have that $R_i \cap P_i \cap U = \emptyset$, so $R_i \cap P_i = R_i \cap Q_i$. Moreover, $\sum_{\ell' = 1}^k \left(|R_i \cap Q_{\ell'}| - |R_i \cap P_{\ell'}|\right)=0$. Hence, we have that 
    \[
        \sum_{\ell' \neq i} \left(|R_i \cap Q_{\ell'}| - |R_i \cap P_{\ell'}|\right) = \sum_{\ell' = 1}^k \left(|R_i \cap Q_{\ell'}| - |R_i \cap P_{\ell'}|\right) = 0. 
    \]
    Therefore,
    \[
        |R_i \cap Q_1| - |R_i \cap P_1| + \sum_{\ell' \notin \{1, i\}} \left(|R_i \cap Q_{\ell'}| - |R_i \cap P_{\ell'}|\right) = 0. 
    \]
    Hence,  
    \[
        |R_i \cap Q_1| - |R_i \cap P_1| = \sum_{\ell' \notin \{1, i\}} \left(|R_i \cap P_{\ell'}| - |R_i \cap Q_{\ell'}|\right). 
    \]
    Since $R_i \cap Q_{\ell'} \subseteq R_i \cap P_{\ell'}$ for each $\ell' \in [k] \setminus \{1, i\}$, we have that 
    %$|R_i \cap P_{\ell'}| \geq |R_i \cap Q_{\ell'}|$ or 
    $|R_i \cap P_{\ell'}| - |R_i \cap Q_{\ell'}| \geq 0$ for each $\ell' \in [k] \setminus \{1, i\}$.
    Then, for each $\ell \in [k] \setminus \{1, i\}$,
    \[
        |R_i \cap P_\ell| - |R_i \cap Q_\ell| \leq \sum_{\ell' \notin \{1, i\}} \left(|R_i \cap P_{\ell'}| - |R_i \cap Q_{\ell'}|\right) = |R_i \cap Q_1| - |R_i \cap P_1|.
    \] 
    Hence, for each $\ell \in [k] \setminus \{1, i\}$,
    \begin{align*}
        |R_i \cap P_\ell| &\leq |R_i \cap Q_1| - |R_i \cap P_1| + |R_i \cap Q_\ell| \\
        &\leq |R_i \cap Q_1| - |R_i \cap P_1| + 1 \quad \text{(since $R_i \cap Q_\ell \subseteq \{(i, \ell)\}$)} \\
        &\leq |R_i \cap Q_1| - 1 + 1 \quad \text{(since $R_1 \subseteq P_1$, $(1, i) \in P_1$, so $(i, 1) \in P_1$)} \\
        &\leq |R_i \cap Q_1|.
    \end{align*}
    This completes the proof of inequality \eqref{ineq:set-sizes}. 

    Next, we observe that 
    \begin{align*}
        \sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right) & = \phi_t\left(|R_i \cap Q_i|\right) - \phi_t\left(|R_i \cap P_i|\right) + \sum_{\ell \neq i} \left(\phi_n\left(|R_i \cap Q_\ell|\right) - \phi_n\left(|R_i \cap P_\ell|\right) \right) \\
        &= \sum_{\ell \neq i} \left(\phi_n\left(|R_i \cap Q_\ell|\right) - \phi_n\left(|R_i \cap P_\ell|\right) \right) \quad \quad \text{(since $R_i \cap P_i \cap U = \emptyset$)} \\ 
        &= \phi_n\left(|R_i \cap Q_1|\right) - \phi_n\left(|R_i \cap P_1|\right) + \sum_{\ell \notin \{1, i\}} \left(\phi_n\left(|R_i \cap Q_\ell|\right) - \phi_n\left(|R_i \cap P_\ell|\right)\right).
    \end{align*} 
    % \knote{Tag the relevant inequalities and cite them as needed.}
    We consider two cases based on $|R_i \cap Q_1|$. 
    
    \noindent \textbf{Case 1.} Suppose $|R_i \cap Q_1| \leq \frac{7}{8}k$. By inequality \eqref{ineq:set-sizes}, we have that $|R_i \cap P_\ell| \leq |R_i \cap Q_1| \leq \frac{7}{8}k$ for each $\ell \in [k] \setminus \{1, i\}$. Additionally, we have that $|R_i \cap P_1| \leq |R_i \cap Q_1| \leq \frac{7}{8}k$  since $P_1 \subseteq Q_1$. 
    Consequently, 
    \begin{align*}
        &\phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \sum_{\ell \notin \{1, i\}} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) \\
        & \quad = |R_i \cap Q_1| - |R_i \cap P_1| + \sum_{\ell \notin \{1, i\}} \left(|R_i \cap Q_\ell| - |R_i \cap P_\ell|\right) \\
        & \quad = 0. 
    \end{align*}

    \noindent \textbf{Case 2}. Suppose $|R_i \cap Q_1| > \frac{7}{8}k$. Since $|R_i \cap Q_1| > \frac{7}{8}k$, we have that $|R_i \cap Q_\ell| \leq \frac{7}{8}k$ for each $\ell \in [k] \setminus \{1, i\}$. Hence, 
    \[
    \phin{R_i \cap Q_\ell} = \begin{cases} \frac{7}{8}k & \ell = 1, \\ |R_i \cap Q_\ell| & \ell \notin \{1, i\}.\end{cases} 
    \]
    Therefore,
    \begin{align*}
        \sum_{\ell \neq i} \phin{R_i \cap Q_\ell} &= \frac{7}{8}k + \sum_{\ell \notin \{1, i\}} |R_i \cap Q_\ell| \\
        &= \frac{7}{8}k + \sum_{\ell \neq i} |R_i \cap Q_\ell| - |R_i \cap Q_1| \\
        &= \frac{7}{8}k + \sum_{\ell \neq i} |R_i \cap P_\ell| - |R_i \cap Q_1|.
    \end{align*}
    Now we consider $\sum_{\ell \neq i} \phin{R_i \cap P_\ell}$. Let $\ell^* = \argmax_{\ell \neq i} |R_i \cap P_\ell|$. Then, 
    \begin{align*}
        \sum_{\ell \neq i} \phin{R_i \cap P_\ell} &= \phin{R_i \cap P_{\ell^*}} + \sum_{\ell \notin \{\ell^*, i\}} |R_i \cap P_\ell| \quad \text{(since for each $\ell \notin \{\ell^*, i\}$, $|R_i \cap P_\ell| \leq \frac{7}{8}k$)} \\
        &= \phin{R_i \cap P_{\ell^*}} + \sum_{\ell \neq i} |R_i \cap P_\ell| - |R_i \cap P_{\ell^*}|.
    \end{align*}
    Therefore, 
    \[
        \sum_{\ell \neq i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) = \frac{7}{8}k - \phin{R_i \cap P_{\ell^*}} - |R_i \cap Q_1| + |R_i \cap P_{\ell^*}|. 
    \]
    If $|R_i \cap P_{\ell^*}| \leq \frac{7}{8}k$, then 
    \begin{align*}
        \sum_{\ell \neq i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) &= \frac{7}{8}k - |R_i \cap P_{\ell^*}| - |R_i \cap Q_1| + |R_i \cap P_{\ell^*}| \\
        &= \frac{7}{8}k - |R_i \cap Q_1| \\
        &< 0. \quad \text{(since $|R_i \cap Q_1| > \frac{7}{8}k$)}
    \end{align*}
    Otherwise, $|R_i \cap P_{\ell^*}| > \frac{7}{8}k$. Then,
    \begin{align*}
        \sum_{\ell \neq i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) &= \frac{7}{8}k - \frac{7}{8}k - |R_i \cap Q_1| - |R_i \cap P_{\ell^*}| \\
        &= -|R_i \cap Q_1| + |R_i \cap P_{\ell^*}| \\
        &\leq 0,
    \end{align*}
    since $|R_i \cap P_\ell| \leq |R_i \cap Q_1|$ for each $\ell \in [k] \setminus \{1, i\}$ by inequality \eqref{ineq:set-sizes} and $|R_i \cap P_1| \leq |R_i \cap Q_1|$. 
    %Hence, in both cases, $\sum_{\ell = 1}^k \left(g(R_i \cap Q_\ell) - g(R_i \cap P_\ell)\right) \leq 0$. 
\end{proof}

We will use the following claim later to move certain elements to adjust sizes of certain parts in the symmetric partition without increasing the objective value. 
\begin{claim}
\label{claim:move_pair}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ %\knote{such that $R_1 \subseteq P_1$ and $U(P_1, \ldots, P_k)\subseteq P_1$. Let $(i, j) \in R_i \cap P_i$ where $i \neq j$. If $|R_j \cap P_j| \geq |R_i \cap P_i|$, then the symmetric partition $Q_i = P_i \setminus \{(i, j), (j, i)\}, Q_j = P_j \cup \{(i, j), (j, i)\}, Q_\ell = P_\ell$ for all $\ell \notin \{i, j\}$ satisfies $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. } 
    with the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P_1$ and %\knote{Can't we remove this condition and just keep the second condition?}

        \item $U(P_1, \ldots, P_k)\subseteq P_1$. 
    \end{enumerate}
    Let $(i, j) \in R_i \cap P_i$ where $i \neq j$. If $|R_j \cap P_j| \geq |R_i \cap P_i|$, 
    %Consider $(i, j) \in R_i \cap P_i$ where $i \neq j$. If $|R_j \cap P_j| \geq |R_i \cap P_i|$, 
    then the symmetric multiway partition $Q_i := P_i \setminus \{(i, j), (j, i)\}, Q_j := P_j \cup \{(i, j), (j, i)\}, Q_\ell := P_\ell$ for all $\ell \notin \{i, j\}$ satisfies $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
\end{claim}
\begin{proof}
    % \donote{From definition of unhappy vertices.}  
    We observe that $1 \notin \{i, j\}$ since $(j, i) \notin P_j$ implies that $k - 1 \geq |R_j \cap P_j| \geq |R_i \cap P_i|$ and $|R_1 \cap P_1| = k$. Let $a = |R_i \cap P_i|$ and $b = |R_j \cap P_j|$. 
    
    We have
    \begin{align*}
        &\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) \\
        &= \phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j} \quad \text{(since $P_\ell = Q_\ell$ for all $\ell \notin \{i, j\}$)} \\
        &= \phi_t(a - 1) - \phi_t(a) + 1 - 0 \quad \text{(since $P_j \cap U = \emptyset$ and $(i, j) \in P_i$ implies $|R_i \cap P_j| = 0$)} \\
        &= \phi_t(a - 1) - \phi_t(a) + 1.
    \end{align*}

    Additionally, 
    \begin{align*}
        &\phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \sum_{\ell \in [k] - j} \left(\phin{R_j \cap Q_\ell} - \phin{R_j \cap P_\ell}\right) \\
        &= \phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \phin{R_j \cap Q_i} - \phin{R_j \cap P_i} \quad \text{(since $P_\ell = Q_\ell$ for all $\ell \notin \{i, j\}$)} \\
        &= \phi_t(b + 1) - \phi_t(b) + 0 - 1 \quad \text{(since $P_i \cap U = \emptyset$ and $(j, i) \in P_i$ implies $|R_j \cap P_i| = 1$)} \\
        &= \phi_t(b + 1) - \phi_t(b) - 1.
    \end{align*}

    Then, we have 
    \begin{align*}
        &\obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} \\
        &= \sum_{x = 1}^k \left(\phit{R_x \cap Q_x}  - \phit{R_x \cap P_x} + \sum_{\ell \in [k] - x} \left(\phin{R_x \cap Q_\ell} - \phin{R_x \cap P_\ell}\right)\right) \\
        &= \sum_{x \in \{i, j\}} \left(\phit{R_x \cap Q_x}  - \phit{R_x \cap P_x} + \sum_{\ell \in [k] - x} \left(\phin{R_x \cap Q_\ell} - \phin{R_x \cap P_\ell}\right)\right),
    \end{align*}
    since for all $x \notin \{i, j\}$ and $\ell \in [k]$, $R_x \cap Q_\ell = R_x \cap P_\ell$. 
    Thus, 
    \begin{align*}
        \obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} &= \phi_t(a - 1) - \phi_t(a) + 1 + \phi_t(b + 1) - \phi_t(b) - 1 \\
        &= \phi_t(b + 1) - \phi_t(b) - (\phi_t(a) - \phi_t(a - 1)) \\
        &\leq 0 \quad \text{(since $\phi_t$ is concave and $a \leq b$)}. 
    \end{align*}
\end{proof}

For the rest of the transformations, we will use the following notion of \emph{swap} operation. 
\begin{definition}[swap operation]
\label{def:swap}
    For each $i\in \{2, 3, \ldots, k\}$, define $\pi_i:[k] \rightarrow [k]$ as follows:
    \[
        \pi_{i}(\ell) = \begin{cases} \ell & \text{if } \ell \notin \{i-1, i\}, \\ i-1 & \text{if } \ell = i, \\ i & \text{if } \ell = i-1. \end{cases}
    \]
    %Let $V = [k] \times [k]$. 
    For $i \in \{2, 3, \ldots, k\}$ and a symmetric multiway partition $P_1, \ldots, P_k$ of $V$, we define $\swapi{P_1, \ldots, P_k}$ as the symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ defined by 
    \begin{enumerate}
        \item $Q_{i - 1} = \left\{\left(\pi_{i}(x), \pi_{i}(y)\right) \colon (x, y) \in P_i \right\}$, 
        \item $Q_i = \left\{\left(\pi_{i}(x), \pi_{i}(y)\right) \colon (x, y) \in P_{i - 1} \right\}$, and 
        \item $Q_\ell = \left\{\left(\pi_{i}(x), \pi_{i}(y)\right) \colon (x, y) \in P_\ell \right\}$ for each $\ell \in [k]\setminus \{i-1, i\}$.
    \end{enumerate}
    Condensing this definition, we see that $Q_{\pi_i(\ell)} = \left\{ \left(\pi_i(x), \pi_i(y)\right) \colon (x, y) \in P_\ell \right\}$ for every $\ell\in [k]$. 
\end{definition}

\begin{figure}[ht]
\centering
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
    
        \definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
        
        % Define grid size
        \def\gridsize{5}
        \def\spacing{0.9} % Distance between points
    
        % Draw the grid of vertices
        \foreach \x in {1,...,\gridsize} {
            \foreach \y in {1,...,\gridsize} {
                % Draw regular black vertices
                \filldraw[black] (\x*\spacing, \y*\spacing) circle (2pt);
            }
        }
        
        % P1
        \foreach \i in {0,...,4} {
            \foreach \j in {0} {
                \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
            }
        }
    
        \foreach \i in {0} {
            \foreach \j in {1,...,4} {
                \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
            }
        }
    
        % P2
        \foreach \i/\j in {1/1, 1/3, 3/1}{
            \fill[orange, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P3
        \foreach \i/\j in {1/2, 2/1, 2/2, 2/3, 2/4, 3/2, 4/2}{
            \fill[green, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P4
        \foreach \i/\j in {1/4, 3/3, 4/1}{
            \fill[blue, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P5
        \foreach \i/\j in {4/3, 4/4, 3/4}{
            \fill[brightube, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    \end{tikzpicture}
    \captionsetup{singlelinecheck=off}
    \caption*{
        \begin{itemize}
            \item[] $P_1 = R_1 \cup C_1$

            \item[] $P_2 = \{(2, 2), (2, 4), (4, 2)\}$

            \item[] $P_3 = \{(2, 3), (3, 2), (3, 3), (3, 4), (3, 5), (4, 3), (5, 3)\}$

            \item[] $P_4 = \{(2, 5), (4, 4), (5, 2)\}$

            \item[] $P_5 = \{(4, 5), (5, 4), (5, 5)\}$
        \end{itemize}
    }
    \captionsetup{singlelinecheck=on}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
    
        \definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
        
        % Define grid size
        \def\gridsize{5}
        \def\spacing{0.9} % Distance between points
    
        % Draw the grid of vertices
        \foreach \x in {1,...,\gridsize} {
            \foreach \y in {1,...,\gridsize} {
                % Draw regular black vertices
                \filldraw[black] (\x*\spacing, \y*\spacing) circle (2pt);
            }
        }
        
        % Q1
        \foreach \i in {0,...,4} {
            \foreach \j in {0} {
                \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
            }
        }
    
        \foreach \i in {0} {
            \foreach \j in {1,...,4} {
                \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
            }
        }
    
        % Q2
        \foreach \i/\j in {2/1, 1/2, 1/1, 1/3, 1/4, 3/1, 4/1}{
            \fill[green, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q3
        \foreach \i/\j in {2/2, 2/3, 3/2}{
            \fill[orange, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q4
        \foreach \i/\j in {2/4, 3/3, 4/2}{
            \fill[blue, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q5
        \foreach \i/\j in {4/3, 4/4, 3/4}{
            \fill[brightube, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    \end{tikzpicture}
    \captionsetup{singlelinecheck=off}
    \caption*{
        \begin{itemize}
            \item[] $Q_1 = R_1 \cup C_1$

            \item[] $Q_2 = \{(2, 2), (2, 3), (2, 4), (2, 5), (3, 2), (4, 2), (5, 2)\}$

            \item[] $Q_3 = \{(3, 3), (3, 4), (4, 3)\}$

            \item[] $Q_4 = \{(3, 5), (4, 4), (5, 3)\}$

            \item[] $Q_5 = \{(4, 5), (5, 4), (5, 5)\}$
        \end{itemize}
    }
    \captionsetup{singlelinecheck=on}
\end{minipage}
\caption{An example of a swap in which $(Q_1, \ldots, Q_5) = \text{swap}_3(P_1, \ldots, P_5)$. On the left, $P_2$, $P_3$, and $P_4$ correspond to the orange, green, and blue part respectively. On the right, $Q_2$, $Q_3$, and $Q_4$ correspond to the green,  orange, and blue part respectively.}
\end{figure}

We now show that swap operations preserve certain structural properties without increasing the objective value. 
\begin{claim}
\label{claim:swap_properties}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$. Let $Q_1, \ldots, Q_k = \swapi{P_1, \ldots, P_k}$ for some $i \in \{3,\ldots, k\}$. Then,
    \begin{enumerate}
        \item $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$.
        \label{item:is_sym_mult_part}
        
        \item If $U(P_1, \ldots, P_k) \subseteq P_1$, then $U(Q_1, \ldots, Q_k) \subseteq Q_1$. 
        \label{item:swap_unhappy}
    
        \item 
        \label{item:swap_size}
        $\left|R_x \cap Q_\ell\right| = \left|R_{\pi_{i}(x)} \cap P_{\pi_{i}(\ell)}\right|$ for all $x, \ell \in [k]$. 

        \item $\obj{Q_1, \ldots, Q_k} = \obj{P_1, \ldots, P_k}$. 
        \label{item:swap_obj}

        \item If $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ and $\ell \in [k] \setminus \{i-1, i\}$, then $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$.
        \label{item:swap_preserve_empty}

        \item If $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ and $\ell \in [k] \setminus \{i - 1, i\}$, then $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$. 
        \label{item:swap_preserve_subset}

    \end{enumerate}
\end{claim}
\begin{proof}
    First, we show property \ref{item:is_sym_mult_part}. We have $(x, y) \in Q_\ell$ if and only if $(\pi_i(x), \pi_i(y)) \in P_{\pi_i(\ell)}$. Using this fact, we have that $Q_1, \ldots, Q_k$ is a partition of $V$. We now show that $Q_1, \ldots, Q_k$ is symmetric: Suppose for contradiction that $Q_1, \ldots, Q_k$ is not symmetric. Then, there exists $\ell \in [k]$ and $(x, y) \in Q_\ell$ such that $(y, x) \notin Q_\ell$. Then, $(\pi_i(x), \pi_i(y)) \in P_{\pi_i(\ell)}$ and $(\pi_i(y), \pi_i(x)) \notin P_{\pi_i(\ell)}$, but this implies that $P_1, \ldots, P_k$ is not symmetric, which is a contradiction. Hence, $Q_1, \ldots, Q_k$ is symmetric. Finally, $Q_1, \ldots, Q_k$ satisfies $(\ell, \ell) \in Q_\ell$ for each $\ell \in [k]$: To see this, we observe that for each $\ell \in [k] \setminus \{i - 1, i\}$, we have $(\pi_i(\ell), \pi_i(\ell)) = (\ell, \ell) \in P_\ell = P_{\pi_i(\ell)}$, so $(\ell, \ell) \in Q_\ell$. Additionally, because $(i - 1, i - 1) \in P_{i - 1}$, we have $(i, i) = (\pi_i(i - 1), \pi_i(i - 1)) \in Q_{\pi_i(i - 1)} = Q_i$. Similar reasoning shows that $(i - 1, i - 1) \in Q_{i - 1}$. 
    
    Next, we show property \ref{item:swap_size}. We observe that $(x, y) \in Q_\ell$ if and only if $(\pi_i(x), \pi_i(y)) \in P_{\pi_i(\ell)}$. Hence, $|R_x \cap Q_\ell| = \sum_{y = 1}^k \mathbbm{1}\left[(x, y) \in Q_\ell\right] = \sum_{y = 1}^k \mathbbm{1}\left[\left(\pi_i(x), \pi_i(y)\right) \in P_{\pi_i(\ell)}\right] = \left|R_{\pi_i(x)} \cap P_{\pi_i(\ell)}\right|$ since $[k] = \{\pi_i(y)\}_{y \in [k]}$ as $\pi_i$ is a bijection. 

    Now, we show property \ref{item:swap_obj}. Consider $\phit{R_i \cap Q_i} + \sum_{\ell \neq x} \phin{R_x \cap Q_\ell}$. We have
    \begin{align*}
        &\phit{R_i \cap Q_i} + \sum_{\ell \neq i} \phin{R_x \cap Q_\ell} \\
        &= \phit{R_i \cap Q_i} + \phin{R_i \cap Q_{i -1}} + \sum_{\ell \notin \{i-1, i\}} \phin{R_i \cap Q_\ell} \\
        &= \phit{R_{i - 1} \cap P_{i - 1}} + \phin{R_{i - 1} \cap P_i} + \sum_{\ell \notin \{i - 1, i\}} \phin{R_{i - 1} \cap P_\ell} \quad \text{(by property \ref{item:swap_size})} \\
        &= \phit{R_{i - 1} \cap P_{i - 1}} + \sum_{\ell \neq i - 1} \phin{R_{i - 1} \cap P_\ell}.
    \end{align*}
    Similar reasoning shows that 
    \[ 
        \phit{R_{i - 1} \cap Q_{i - 1}} + \sum_{\ell \neq i - 1} \phin{R_{i - 1} \cap Q_\ell} = \phit{R_i \cap P_i} + \sum_{\ell \neq i}\phin{R_i \cap P_\ell}. 
    \]
    Finally, for $x \notin \{i - 1, i\}$, we have
    \begin{align*}
        &\phit{R_x \cap Q_x} + \sum_{\ell \neq x}\phin{R_x \cap Q_\ell} \\
        &= \phit{R_x \cap Q_x} + \phin{R_x \cap Q_{i - 1}} + \phin{R_x \cap Q_i} + \sum_{\ell \notin \{x, i - 1, i\}} \phin{R_x \cap Q_\ell} \\
        &= \phit{R_x \cap P_x} + \phin{R_x \cap P_i} + \phin{R_x \cap P_{i - 1}} + \sum_{\ell \notin \{x, i- 1, i\}} \phin{R_x \cap P_\ell} \quad \text{(by property \ref{item:swap_size})} \\
        &= \phit{R_x \cap P_x} + \sum_{\ell \neq x}\phin{R_x \cap P_\ell}. 
    \end{align*}
    Hence, 
    \begin{align*}
        \obj{Q_1, \ldots, Q_k} &= \sum_{x = 1}^k \left(\phit{R_x \cap Q_x} + \sum_{\ell \neq x} \phin{R_x \cap Q_\ell}\right) \\ 
        &= \sum_{x = 1}^k \left(\phit{R_x \cap P_x} + \sum_{\ell \neq x} \phin{R_x \cap P_\ell}\right) \\
        &= \obj{P_1, \ldots, P_k}. 
    \end{align*}

    Next, we prove property \ref{item:swap_unhappy}. For the sake of contradiction, suppose that property \ref{item:swap_unhappy} does not hold. Then, $U(P_1, \ldots, P_k) \subseteq P_1$ and there exists $(x, y) \in U(Q_1, \ldots, Q_k)$ such that $(x, y) \notin Q_1$. Then, $(x, y) \in Q_\ell$ for some $\ell \notin \{1, x, y\}$. Consequently, $\left(\pi_i(x), \pi_i(y)\right) \in P_{\pi_i(\ell)}$. If $\left(\pi_i(x), \pi_i(y)\right)$ is not unhappy under $P_1, \ldots, P_k$, then $\pi_i(\ell) = \pi_i(x)$ or $\pi_i(\ell) = \pi_i(y)$, which would imply that $x = \ell$ or $y = \ell$, a contradiction. Hence, $\left(\pi_i(x), \pi_i(y)\right)$ is unhappy under $P_1 \ldots, P_k$, so $\left(\pi_i(x), \pi_i(y)\right) \in P_1$. Then, $(x, y) \in Q_{\pi_i(1)} = Q_1$, which contradicts the assumption that $(x, y) \notin Q_1$. Thus, all unhappy vertices under $Q_1, \ldots, Q_k$ are in $Q_1$. 

    Next, we prove property \ref{item:swap_preserve_empty}. We consider two cases based on the value of $\ell$.
    \begin{enumerate}
        \item Suppose $\ell \in [i - 2]$. Suppose for contradiction that $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ and $\overleftarrow{R}_\ell \cap Q_\ell \neq \emptyset$. Then there exists $y \in [\ell - 1]$ such that $(\ell, y) \in Q_\ell$. Therefore, $(\ell, y) = (\pi_i(\ell), \pi_i(y)) \in P_{\pi_i(\ell)} = P_\ell$, which contradicts $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$. 
        
        \item Suppose $\ell \in \{i + 1, \ldots, k\}$. Suppose for contradiction that $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ and $\overleftarrow{R}_\ell \cap Q_\ell \neq \emptyset$. Then there exists $y \in [\ell - 1]$ such that $(\ell, y) \in \overleftarrow{R}_\ell \cap Q_\ell$. Then, $(\ell, \pi_i(y)) = (\pi_i(\ell), \pi_i(y)) \in P_{\pi_i(\ell)} = P_\ell$. We observe that $\pi_i(y) = \begin{cases} i & y = i - 1 \\ i - 1 & y = i \\ y & y \notin\{i - 1, i\}\end{cases}$, and in all cases, $\pi_i(y) < \ell$. Hence, $(\ell, \pi_i(y)) \in \overleftarrow{R}_\ell \cap P_\ell$, which contradicts $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$.
    \end{enumerate}

    Finally, we prove property \ref{item:swap_preserve_subset}. Again, we consider two cases based on the value of $\ell$. \begin{enumerate}
        \item Suppose $\ell \in [i - 2]$. Suppose for contradiction that $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ and $\overrightarrow{R}_\ell \not\subseteq Q_1 \cup Q_\ell$. Then, there exists $y \in \{\ell + 1, \ldots, k\}$ and $\ell' \in [k] \setminus \{1, \ell\}$ such that $(\ell, y) \in Q_{\ell'}$. Then, $(\ell, \pi_i(y)) = (\pi_i(\ell), \pi_i(y)) \in P_{\pi_i(\ell')}$. We observe that $\pi_i(y) = \begin{cases} i - 1 & y = i \\ i & y = i - 1 \\ y & y \notin \{i - 1, i\}\end{cases}$, and $\pi_i(\ell') \in [k] \setminus \{1, \ell\}$. Hence, $(\ell, \pi_i(y)) \in \overrightarrow{R}_\ell \cap P_{\pi_i(\ell')}$ is a witnesses the fact that $\overrightarrow{R}_\ell \not\subseteq P_1 \cup P_\ell$, which is a contradiction. 
        
        \item Suppose $\ell \in \{i + 1, \ldots, k\}$. Suppose for contradiction that $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ and $\overrightarrow{R}_\ell \not\subseteq Q_1 \cup Q_\ell$. Then there exists $y \in \{\ell + 1, \ldots, k\}$ and $\ell' \in [k] \setminus \{1, \ell\}$ such that $(\ell, y) \in Q_{\ell'}$. Then, $(\ell, y) = (\pi_i(\ell), \pi_i(y)) \in P_{\pi_i(\ell')}$ where $\pi_i(\ell') \in [k] \setminus \{1, \ell\}$. Then, $\overrightarrow{R}_\ell \not\subseteq P_1 \cup P_\ell$, which is a contradiction.
    \end{enumerate}
\end{proof}

\iffalse
\begin{claim}
    Let $V = [k] \times [k]$. Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ such that all unhappy vertices under $P_1, \ldots, P_k$ are in $P_1$. Let $Q_1, \ldots, Q_k = \swapi{P_1, \ldots, P_k}$. Then, all unhappy vertices under $Q_1, \ldots, Q_k$ are in $Q_1$. 
\end{claim}
\fi

Next, we show that swap operation can be used to enforce additional structure. 
\begin{claim}
\label{claim:swap_preserves_structure}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ and let $i\in \{3, \ldots, k\}$. 
    %\rnote{changed to $i \in \{3, \ldots, k\}$ since swaps only make sense if $i \leq k$}. 
    %Suppose that for some $i - 1 \geq 2$, 
    %$R_{i - 1}, R_i, \ldots, R_k$ satisfy 
    Suppose that the following properties hold for each $\ell \geq i - 1$:
    \begin{enumerate}
        \item $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ with the possible exception that $(i, i - 1) \in \overleftarrow{R}_i \cap P_i$;

        \item $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ with the possible exception that $(i - 1, i) \in P_i$;

        \item $\{(i - 1, i), (i, i - 1)\} \subseteq P_i$ or $\{(i - 1, i), (i, i - 1)\} \subseteq P_1$.
    \end{enumerate}
    Let $(Q_1, \ldots, Q_k) = \swapi{P_1, \ldots, P_k}$. Then, we have that  $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ and $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$
    for each $\ell \geq i - 1$. 
\end{claim}
\begin{proof}
    % \donote{From definition of swap operation.}  
    First, we show that for each $\ell \in \{i - 1, \ldots, k\}$, we have $\overleftarrow{R}_\ell \cap Q_\ell= \emptyset$. By Claim \ref{claim:swap_properties} property \ref{item:swap_preserve_empty}, this statement is true for each $\ell \in \{i + 1, \ldots, k\}$. Hence, suppose for contradiction there exists $j \in \{i - 1, i\}$ such that $\overleftarrow{R}_j \cap Q_j \neq \emptyset$. We case on the value $j$:
    \begin{enumerate}
        \item 
        If $j = i - 1$, then there exists $y \in [i - 2]$ such that $(i - 1, y) \in \overleftarrow{R}_{i - 1} \cap Q_{i - 1}$. Then $(i, \pi_i(y)) = (\pi_i(i - 1), \pi_i(y)) \in P_{\pi_i(i - 1)} = P_i$. This contradicts the fact that $\overleftarrow{R}_i \cap P_i \subseteq \{(i, i - 1)\}$. 

        \item 
        If $j = i$, then there exists $y \in [i - 1]$ such that $(i, y) \in \overleftarrow{R}_i \cap Q_i$. Since $(i - 1, i) \in P_i$ or $(i - i, i) \in P_1$, we have $(i, i - 1) = (\pi_i(i - 1), \pi_i(i)) \in Q_{\pi_i(i)} = Q_{i - 1}$ or $(i, i - 1) \in Q_{\pi_i(1)} = Q_1$. Hence, $y \neq i - 1$, so $y \in [i - 2]$. But then $(i - 1, y) = (\pi_i(i), \pi_i(y)) \in P_{\pi_i(i)} = P_{i - 1}$, which contradicts $\overleftarrow{R}_{i - 1} \cap P_{i - 1} = \emptyset$. 
    \end{enumerate}
    %Hence, we have that $\overleftarrow{R}_j \cap Q_j \neq \emptyset$ for each $j\in \{i-1, \ldots, k\}$. 
    %Overall, the assumption that there exists $j \in \{i - 1, \ldots, k\}$ such that $\overleftarrow{R}_j \cap Q_j \neq \emptyset$ is false. 

    Now, we show that for each $\ell \in \{i - 1, \ldots, k\}$, we have $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$. By Claim \ref{claim:swap_properties} property \ref{item:swap_preserve_subset}, this statement is true for each $\ell \in \{i + 1, \ldots, k\}$. Hence, suppose for contradiction there exists $j \in \{i - 1, i\}$ such that $\overrightarrow{R}_j \not\subseteq Q_1 \cup Q_j$. Again, we case on the value of $j$:
    \begin{enumerate}
        \item 
        If $j = i - 1$, then there exists $y \in \{i, \ldots, k\}$ and $\ell \in [k] \setminus \{1, i - 1\}$ such that $(i - 1, y) \in Q_\ell$. Since $(i, i - 1) \in P_i$ or $(i, i - 1) \in P_1$, we have $(i - 1, i) = (\pi_i(i), \pi_i(i - 1)) \in Q_{\pi_i(i - 1)} = Q_{i - 1}$ or $(i - 1, i) \in Q_{\pi_i(1)} = Q_1$. Therefore, $y \neq i$ and $y \in \{i + 1, \ldots, k\}$. Then, we have $(i, y) = (\pi_i(i - 1), \pi_i(y)) \in P_{\pi_i(\ell)}$ where $\pi_i(\ell) \in [k] \setminus \{1, i\}$. Since $y > i$, $\overrightarrow{R}_i \not\subseteq P_1 \cup P_i$, which is a contradiction. 

        \item 
        If $j = i$, then there exists $y \in \{i + 1, \ldots, k\}$ and $\ell \in [k] \setminus \{1, i\}$ such that $(i, y) \in Q_\ell$. Then, $(i - 1, y) = (\pi_i(i), \pi_i(y)) \in P_{\pi_i(\ell)}$ where $\pi_i(\ell) \in [k] \setminus \{1, i - 1\}$. But then since $y \geq i + 1 \geq i - 1$, we have a contradiction of $\overrightarrow{R}_{i - 1} \subseteq P_1 \cup P_{i - 1}$ with the possible exception that $(i - 1, i) \in P_i$. 
    \end{enumerate}
    %Hence, we have that for each $j \in \{i - 1, \ldots, k\}$, we have $\overrightarrow{R}_j \subseteq Q_1 \cup Q_j$.
\end{proof}

\begin{figure}[ht]
\centering
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
    
        \definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
        
        % Define grid size
        \def\gridsize{6}
        \def\spacing{0.9} % Distance between points
    
        % Draw the grid of vertices
        \foreach \x in {1,...,\gridsize} {
            \foreach \y in {1,...,\gridsize} {
                % Draw regular black vertices
                \filldraw[black] (\x*\spacing, \y*\spacing) circle (2pt);
            }
        }
        
        % P1
        \foreach \i/\j in {0/0, 0/1, 0/2, 1/0, 1/3, 1/4, 1/5, 2/0, 2/5, 3/1, 3/4, 4/1, 4/3, 5/1, 5/2} {
            \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P2
        \foreach \i/\j in {0/3, 0/4, 0/5, 1/1, 1/2, 2/1, 3/0, 4/0, 5/0}{
            \fill[orange, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P3
        \foreach \i/\j in {2/2, 2/4, 4/2}{
            \fill[green, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P4
        \foreach \i/\j in {2/3, 3/2, 3/3, 3/5, 5/3}{
            \fill[blue, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P5
        \foreach \i/\j in {4/4, 4/5, 5/4}{
            \fill[brightube, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % P6
        \foreach \i/\j in {5/5}{
            \fill[gray, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    \end{tikzpicture}
    \caption*{Visualization of $P_1, \ldots, P_6$.}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
    
        \definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
        
        % Define grid size
        \def\gridsize{6}
        \def\spacing{0.9} % Distance between points
    
        % Draw the grid of vertices
        \foreach \x in {1,...,\gridsize} {
            \foreach \y in {1,...,\gridsize} {
                % Draw regular black vertices
                \filldraw[black] (\x*\spacing, \y*\spacing) circle (2pt);
            }
        }
        
        % Q1
        \foreach \i/\j in {0/0, 0/1, 0/3, 1/0, 1/2, 1/4, 1/5, 3/0, 3/5, 2/1, 2/4, 4/1, 4/2, 5/1, 5/3} {
            \fill[red, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q2
        \foreach \i/\j in {0/2, 0/4, 0/5, 1/1, 1/3, 3/1, 2/0, 4/0, 5/0}{
            \fill[orange, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q4
        \foreach \i/\j in {3/3, 3/4, 4/3}{
            \fill[green, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q3
        \foreach \i/\j in {3/2, 2/3, 2/2, 2/5, 5/2}{
            \fill[blue, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q5
        \foreach \i/\j in {4/4, 4/5, 5/4}{
            \fill[brightube, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    
        % Q6
        \foreach \i/\j in {5/5}{
            \fill[gray, opacity = 0.4] (0.5*\spacing + \i*\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing) rectangle (0.5*\spacing + \i*\spacing +\spacing, \gridsize*\spacing - 0.5*\spacing - \j*\spacing + \spacing);
        }
    \end{tikzpicture}
    \caption*{Visualization of $Q_1, \ldots, Q_6$.}
\end{minipage}
\caption{An example of applying Claim \ref{claim:swap_preserves_structure}. On the left is $P_1, \ldots, P_6$. On the right is $(Q_1, \ldots, Q_6) = \text{swap}_4(P_1, \ldots, P_6)$. On the left, $P_3$ and $P_4$ correspond to the green and blue part respectively. On the right, $Q_3$ and $Q_4$ correspond to the blue and green part respectively.}
\end{figure}

Our next claim will help in inductively achieving the required structure. We include an additional conclusion in the claim which will not be used beyond this claim, namely property 7. The purpose of this property is that it serves as a stronger induction hypothesis to prove the claim. 

\begin{claim}\label{claim:induction-size}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ and let $i \in \{3, \ldots, k + 1\}$. Suppose $P_1, \ldots, P_k$ additionally satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P_1$, 
        
        \item $U(P_1, \ldots, P_k) \subseteq P_1$, 

        \item $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ for each $\ell \in \{i - 1, i, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ for each $\ell \in \{i - 1, i, \ldots, k\}$, and 

        \item $\left|R_i \cap P_i\right| \geq \left|R_{i + 1} \cap P_{i + 1}\right| \geq \ldots \geq \left|R_k \cap P_k\right|$. 
    \end{enumerate}
    Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ that additionally satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq Q_1$, 
        
        \item $U(Q_1, \ldots, Q_k)\subseteq Q_1$, 

        \item $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ for each $\ell \in \{i - 1, i, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$ for each $\ell \in \{i - 1, i, \ldots, k\}$, 

        \item $\left|R_{i - 1} \cap Q_{i - 1}\right| \geq \left|R_i \cap Q_i\right| \geq \ldots \geq \left|R_k \cap Q_k\right|$, 

        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$, and

        \item $Q_1, \ldots, Q_k$ is obtained from $P_1, \ldots, P_k$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{i \ldots, k\}$. 
        %\knote{Why do we need to state this property in the lemma statement? Where is it used?} \knote{Or is this statement needed as a stronger inductive hypothesis? } \rnote{Yes. This statement serves as an inductive hypothesis}
    \end{enumerate}
\end{claim}
\begin{proof}
    % \knote{Relies on Claims 2.8, 2.9, and 2.10.}
    If $i = k + 1$, then setting $Q_\ell := P_\ell$ for each $\ell \in [k]$ gives a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ satisfying the required properties. We will henceforth assume that $i\le k$. Now, suppose for contradiction that the claim is false. Let $\mathcal{C}$ be the set of pairs $\left((P_1, \ldots, P_k), i\right)$, where $P_1, \ldots, P_k$ is a symmetric multiway partition of $V$ and $i \in \{3, \ldots, k + 1\}$, that serve as counterexamples to the claim. Let $t = \max\left\{i \colon \left((P_1, \ldots, P_k), i\right) \in \mathcal{C} \right\}$. Since the claim holds for $i = k + 1$, we have that $t \in \{3, \ldots, k\}$. Let 
    \[
        \left(P_1^{(0)}, \ldots, P_k^{(0)}\right) = \argmax_{(P_1, \ldots, P_k) \colon \left((P_1, \ldots, P_k), t\right) \in \mathcal{C}} |R_t \cap P_t|.
    \]
    In other words, among symmetric multiway partitions $P_1, \ldots, P_k$ that serve as a counterexample to the claim when paired with $t$, $\left|R_t \cap P_t^{(0)}\right|$ maximizes $|R_t \cap P_t|$. 

    Since $P_1^{(0)}, \ldots, P_k^{(0)}$ is a counterexample when paired with $t$, we must have 
    \begin{align}
        \left|R_{t - 1} \cap P_{t - 1}^{(0)} \right| < \left|R_t \cap P_t^{(0)} \right|. \label{ineq:row-intersection-sizes}   
    \end{align} 
    If not, then letting $Q_\ell := P_\ell^{(0)}$ for each $\ell \in [k]$ would satisfy the properties required of $Q_1, \ldots, Q_k$ in the claim. In the rest of this proof, we will perform a series of transformations to $P_1^{(0)}, \ldots, P_k^{(0)}$ to arrive at a partition $Q_1, \ldots, Q_k$ satisfying the conclusions of the claim. This contradicts the existence of a counterexample to the claim.
    
    If $\{(t - 1, t), (t, t - 1)\} \subseteq P_{t - 1}^{(0)}$, then we define $P_1^{(1)}, \ldots, P_k^{(1)}$ as $P_{t - 1}^{(1)} := P_{t - 1}^{(0)} \setminus \{(t - 1, t), (t, t - 1)\}$, $P_t^{(1)} := P_t^{(0)} \cup \{(t - 1, t), (t, t - 1)\}$, and $P_\ell^{(1)} := P_\ell^{(0)}$ for each $\ell \in [k] \setminus \{t - 1, t\}$. Otherwise, we let $P_\ell^{(1)} := P_\ell^{(0)}$ for each $\ell \in [k]$. By \eqref{ineq:row-intersection-sizes} and Claim \ref{claim:move_pair}, we have that $\obj{P_1^{(1)}, \ldots, P_k^{(1)}} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}}$. 

    Next, let $\left(P_1^{(2)}, \ldots, P_k^{(2)}\right) = \text{swap}_t\left(P_1^{(1)}, \ldots, P_k^{(1)}\right)$. The symmetric multiway partition $P_1^{(2)}, \ldots, P_k^{(2)}$ of $V$ satisfies the following properties:
    \begin{enumerate}
        \item 
        We have $R_1 \subseteq P_1^{(2)}$ since $R_1 \subseteq P_1^{(1)}$ and by Claim \ref{claim:swap_properties} property \ref{item:swap_preserve_subset}. 

        \item 
        We have $U\left(P_1^{(2)}, \ldots, P_k^{(2)}\right) \subseteq P_1^{(2)}$ since $U\left(P_1^{(1)}, \ldots, P_k^{(1)}\right) \subseteq P_1^{(1)}$ and by Claim \ref{claim:swap_properties} property \ref{item:swap_unhappy}. 

        \item 
        For each $\ell \in \{t - 1, t, \ldots, k\}$, we have $\overleftarrow{R}_\ell \cap P_\ell^{(2)} = \emptyset$. This is because $P_1^{(1)}, \ldots, P_k^{(1)}$ and $i=t$ satisfy the hypotheses of Claim \ref{claim:swap_preserves_structure}. 

        \item 
        For each $\ell \in \{t - 1, t \ldots, k\}$, we have $\overrightarrow{R}_\ell \subseteq P_1^{(2)} \cup P_\ell^{(2)}$. Again, this is because $P_1^{(1)}, \ldots, P_k^{(1)}$ and $i=t$ satisfy the hypotheses of Claim \ref{claim:swap_preserves_structure}.

        \item 
        We have that $\left|R_{t + 1} \cap P_{t + 1}^{(2)}\right| \geq \left|R_{t + 2} \cap P_{t + 2}^{(2)}\right| \geq \ldots \geq \left|R_k \cap P_k^{(2)}\right|$: By Claim \ref{claim:swap_properties} property \ref{item:swap_size}, we have $\left|R_{\ell} \cap P_{\ell}^{(2)}\right| = \left|R_{\ell} \cap P_{\ell}^{(1)}\right|$ for each $\ell \in \{t + 1, \ldots, k\}$. Additionally, we have $\left|R_{\ell} \cap P_{\ell}^{(1)}\right| = \left|R_{\ell} \cap P_{\ell}^{(0)}\right|$ for each $\ell \in \{t + 1, \ldots, k\}$. Then the claimed property follows from the fact that $\left|R_{t + 1} \cap P_{t + 1}^{(0)} \right| \geq \left|R_{t + 2} \cap P_{t + 2}^{(0)}\right| \geq \ldots \geq \left|R_k \cap P_k^{(0)}\right|$ since $P_1^{(0)}, \ldots, P_k^{(0)}$ paired with $t$ is a counterexample to the claim. %Claim \ref{claim:induction-size}.

        \item 
        $\obj{P_1^{(2)}, \ldots, P_k^{(2)}} = \obj{P_1^{(1)}, \ldots, P_k^{(1)}} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}}$: This is because of Claim \ref{claim:swap_properties} property \ref{item:swap_obj}.
    \end{enumerate}
    Since $t + 1 > t$, we have that $\left(\left(P_1^{(2)}, \ldots, P_k^{(2)}\right), t + 1\right) \notin \mathcal{C}$. Therefore, there exists a symmetric multiway partition $P^{(3)}_1, \ldots, P^{(3)}_k$ of $V$ that satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P^{(3)}_1$, 
        
        \item $U(P^{(3)}_1, \ldots, P^{(3)}_k)\subseteq P^{(3)}_1$, 

        \item $\overleftarrow{R}_\ell \cap P^{(3)}_\ell = \emptyset$ for each $\ell \in \{t, t + 1, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq P^{(3)}_1 \cup P^{(3)}_\ell$ for each $\ell \in \{t, t + 1, \ldots, k\}$, 

        \item $\left|R_{t} \cap P^{(3)}_{t}\right| \geq \left|R_{t + 1} \cap P^{(3)}_{t + 1}\right| \geq \ldots \geq \left|R_k \cap P^{(3)}_k\right|$,

        \item $\obj{P^{(3)}_1, \ldots, P^{(3)}_k} \leq \obj{P_1^{(2)}, \ldots, P_k^{(2)}} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}}$, and

        \item $P^{(3)}_1, \ldots, P^{(3)}_k$ can be obtained from $P_1^{(2)}, \ldots, P_k^{(2)}$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$.
    \end{enumerate}

    Now, we show that $\overleftarrow{R}_{t - 1} \cap P^{(3)}_{t - 1} = \emptyset$:  We recall that $\overleftarrow{R}_{t - 1} \cap P_{t - 1}^{(2)} = \emptyset$. Additionally, $P^{(3)}_1, \ldots, P^{(3)}_k$ is obtained from $P_1^{(2)}, \ldots, P_k^{(2)}$ using only $\text{swap}_j$ operations and operations that change the part containing $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$. Hence, we apply Claim \ref{claim:swap_properties} property \ref{item:swap_preserve_empty} in addition to the fact that modifying the assignment for $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$ does not affect the assignment for elements in $R_{t - 1}$ to conclude that $\overleftarrow{R}_{t - 1} \cap P^{(3)}_{t - 1} = \emptyset$. 

    Next, using similar reasoning, we show that $\overrightarrow{R}_{t - 1} \subseteq P^{(3)}_1 \cup P^{(3)}_{t - 1}$: We recall that $\overrightarrow{R}_{t - 1} \subseteq P_1^{(2)} \cup P_{t - 1}^{(2)}$. Additionally, $P^{(3)}_1, \ldots, P^{(3)}_k$ is obtained from $P_1^{(2)}, \ldots, P_k^{(2)}$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$. Hence, we apply Claim \ref{claim:swap_properties} property \ref{item:swap_preserve_subset} in addition to the fact that modifying the assignment for $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$ does not affect the assignment for vertices in $R_{t - 1}$ to see that $\overrightarrow{R}_{t - 1} \subseteq P^{(3)}_1 \cup P^{(3)}_{t - 1}$. 

    Above, we have established that $P^{(3)}_1, \ldots, P^{(3)}_k$ and $t$ satisfy the hypotheses of Claim \ref{claim:induction-size}. Now, we demonstrate that $\left(\left(P^{(3)}_1, \ldots, P^{(3)}_k\right), t\right) \notin \mathcal{C}$. We have
    \begin{align}
        \left|R_t \cap P_t^{(0)} \right| &\leq \left|R_t \cap P_t^{(1)} \right| \quad \text{(since $P_t^{(0)} \subseteq P_t^{(1)}$)} \notag\\ 
        &= \left|R_{t - 1} \cap P_{t - 1}^{(2)} \right| \quad \text{(by Claim \ref{claim:swap_properties} property \ref{item:swap_size} applied to $\text{swap}_t$)} \notag \\
        &= \left|R_{t - 1} \cap P^{(3)}_{t - 1} \right|, \label{ineq:R_t-intersection-size}
    \end{align}
    where the last equality follows from repeated use of Claim \ref{claim:swap_properties} property \ref{item:swap_size} for $\text{swap}_j$ where $j \in \{t + 1, \ldots, k\}$ and the fact that changing the assignment for $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t + 1, \ldots, k\}$ does not affect the assignment for vertices in $R_{t - 1}$. Suppose for contradiction $\left(\left(P^{(3)}_1, \ldots, P^{(3)}_k\right), t\right) \in \mathcal{C}$. Then, $\left|R_{t - 1} \cap P^{(3)}_{t - 1}\right| < \left|R_t \cap P^{(3)}_t\right|$---otherwise, setting $Q_{\ell}:=P_{\ell}^{(3)}$ for each $\ell\in [k]$ would satisfy the properties required of $Q_1, \ldots, Q_k$ in the claim thereby implying that $\left(\left(P^{(3)}_1, \ldots, P^{(3)}_k\right), t\right) \not\in \mathcal{C}$. However, by \eqref{ineq:R_t-intersection-size}, we have that $\left|R_t \cap P_t^{(0)} \right| < \left|R_t \cap P^{(3)}_t\right|$, which contradicts the fact that
    \[
        \left|R_t \cap P_t^{(0)}\right| = \max_{(P_1, \ldots, P_k) \colon \left((P_1, \ldots, P_k), t\right) \in \mathcal{C}} |R_t \cap P_t|. 
    \]
    Hence, $\left(\left(P^{(3)}_1, \ldots, P^{(3)}_k\right), t\right) \notin \mathcal{C}$. 
    
    Furthermore, we observe that $P^{(3)}_1, \ldots, P^{(3)}_k$ was obtained from $P_1^{(0)}, \ldots, P_k^{(0)}$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t, \ldots, k\}$. 

    Finally, since $\left(\left(P^{(3)}_1, \ldots, P^{(3)}_k\right), t\right) \notin \mathcal{C}$ and $P^{(3)}_1, \ldots, P^{(3)}_k$ and $t$ satisfy the hypotheses of Claim \ref{claim:induction-size}, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that 
    \begin{enumerate}
        \item $R_1 \subseteq Q_1$, 
        
        \item $U(Q_1, \ldots, Q_k)\subseteq Q_1$, 

        \item $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ for each $\ell \in \{t - 1, t, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$ for each $\ell \in \{t - 1, t, \ldots, k\}$, 

        \item $\left|R_{t - 1} \cap Q_{t - 1}\right| \geq \left|R_t \cap Q_t\right| \geq \ldots \geq \left|R_k \cap Q_k\right|$, 

        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1^{(3)}, \ldots, P_k^{(3)}}$, and

        \item $Q_1, \ldots, Q_k$ is obtained from $P_1^{(3)}, \ldots, P_k^{(3)}$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t, \ldots, k\}$.
    \end{enumerate}
    Since, $\obj{P_1^{(3)}, \ldots, P_k^{(3)}} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}}$, we have $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}}$. Additionally, $P^{(3)}_1, \ldots, P^{(3)}_k$ was obtained from $P_1^{(0)}, \ldots, P_k^{(0)}$ using only $\text{swap}_j$ operations and operations that modify the assignment of $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t, \ldots, k\}$. Therefore, $Q_1, \ldots, Q_k$ was obtained from $P_1^{(0)}, \ldots, P_k^{(0)}$ using only $\text{swap}_j$ operations and operations that change the part containing $\{(j, j - 1), (j - 1, j)\}$ where $j \in \{t, \ldots, k\}$. Hence, $Q_1, \ldots, Q_k$ satisfies the properties required by the claim. 
    %for Claim \ref{claim:induction-size}. 
    However, this shows that $P_1^{(0)}, \ldots, P_k^{(0)}$ paired with $t$ is not a counterexample to the claim. 
    %Claim \ref{claim:induction-size}, which contradicts $\left(\left(P_1^{(0)}, \ldots, P_k^{(0)}\right), t\right) \in \mathcal{C}$. Therefore, the original assumption that the Claim \ref{claim:induction-size} is false does not hold. 
\end{proof}

Our next claim will be applied immediately after the previous claim and will help in inductively achieving the required structure. 
\begin{claim}\label{claim:induction-containment}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ and let $i \in \{3, \ldots, k + 1\}$. Suppose $P_1, \ldots, P_k$ additionally satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P_1$, 
        
        \item $U(P_1, \ldots, P_k) \subseteq P_1$, 

        \item $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ for each $\ell \in \{i - 1, i, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ for each $\ell \in \{i - 1, i, \ldots, k\}$, and 

        \item $\left|R_{i - 1} \cap P_{i - 1}\right| \geq \left|R_i \cap P_i\right| \geq \ldots \geq \left|R_k \cap P_k\right|$. 
    \end{enumerate}
    Then there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ that additionally satisfies the following properties: \begin{enumerate}
        \item $R_1 \subseteq Q_1$;
        
        \item $U(Q_1, \ldots, Q_k) \subseteq Q_1$, 

        \item $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ for each $\ell \in \{i - 2, i-1, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$ for each $\ell \in \{i - 2, i-1, \ldots, k\}$, 

        \item $\left|R_{i - 1} \cap Q_{i - 1}\right| \geq \left|R_i \cap Q_i\right| \geq \ldots \geq \left|R_k \cap Q_k\right|$, and 

        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$.
    \end{enumerate}
\end{claim}
\begin{proof}
    % \knote{Relies on Claims 2.8 and 2.9?}
    If $i=3$, then the claim holds by setting $Q_\ell = P_\ell$ for each $\ell \in [k]$. We will henceforth assume that $i\ge 4$. 
    Let $j = \argmin_{\ell = 1}^{i - 2} |R_\ell \cap P_\ell|$. We observe that $j \geq 2$ since $R_1 \subseteq P_1$ implies $|R_1 \cap P_1| > |R_\ell \cap P_\ell|$ for all $\ell \in [k] - 1$. Let 
    \[ 
        (P_1', \ldots, P_k') = \text{swap}_{i - 2}\left(\text{swap}_{i - 3}\left(\ldots \text{swap}_{j + 1}\left(P_1, \ldots, P_k) \ldots \right)\right)\right). 
    \]
    Consider the bijection $\pi \colon [k] \rightarrow [k]$ defined as follows:
    \[
        \pi(t) = \begin{cases} t & t \leq j - 1 \text{ or } t \geq i - 1, \\
                    t - 1 & j + 1 \leq t \leq i - 2, \\
                    i - 2 & t = j.
                    \end{cases}
    \]
    We observe that $\pi = \pi_{i - 2} \circ \pi_{i - 3} \circ \ldots \circ \pi_{j + 1}$.
    By applying Claim \ref{claim:swap_properties} repeatedly, we observe that $P_1', \ldots, P_k'$ has the following properties:
    \begin{enumerate}
        \item $P_1', \ldots, P_k'$ is a symmetric multiway partition of $V$.

        \item $U(P_1', \ldots, P_k') \subseteq P_1'$.

        \item $\left|R_x \cap P_\ell'\right| = \left|R_{\pi^{-1}(x)} \cap P_{\pi^{-1}(\ell)}\right|$ for all $x, \ell\in [k]$.

        \item $\obj{P_1', \ldots, P_k'} \leq \obj{P_1, \ldots, P_k}$.

        \item $\overleftarrow{R}_\ell \cap P_\ell' = \emptyset$ for each $\ell \in \{i - 1, \ldots, k\}$. 

        \item $\overrightarrow{R}_\ell \subseteq P_1' \cup P_\ell'$ for each $\ell \in \{i - 1, \ldots, k\}$. 
    \end{enumerate} 
    We observe that $|R_1 \cap P_1'| = \left|R_{\pi^{-1}(1)} \cap P_{\pi^{-1}(1)}\right| = |R_1 \cap P_1| = k$, so $R_1 \subseteq P_1'$. Additionally, for each $\ell \in \{i - 1, \ldots, k\}$, we have $|R_\ell \cap P_\ell'| = \left|R_{\pi^{-1}(\ell)} \cap P_{\pi^{-1}(\ell)}\right| = |R_\ell \cap P_\ell|$. Hence, we have $|R_{i - 1} \cap P_{i - 1}'| \geq |R_i \cap P_i'| \geq \ldots \geq |R_k \cap P_k'|$. 

    We now show the following:  
    \begin{align}
        i - 2 = \argmin_{\ell = 1}^{i - 2} |R_\ell \cap P_\ell'|. \label{eq:i-2-smallest}
    \end{align}
        Since $\pi$ permutes the elements in $[i - 2]$, we have 
    \[  
        \left\{|R_\ell \cap P_\ell'| \colon \ell \in [i - 2]\right\} = \left\{\left|R_{\pi^{-1}(\ell)} \cap P_{\pi^{-1}(\ell)}\right| \colon \ell \in [i - 2]\right\} = \left\{|R_\ell \cap P_\ell| \colon \ell \in [i - 2]\right\}. 
    \]
    By the definition of $j$, we have $|R_j \cap P_j| = \min\left\{|R_\ell \cap P_\ell| \colon \ell \in [i - 2]\right\}$. Hence, 
    \begin{align*}
        \left|R_{i - 2} \cap P_{i - 2}'\right| &= |R_j \cap P_j| \\
        &= \min\left\{|R_\ell \cap P_\ell| \colon \ell \in [i - 2]\right\} \\
        &= \min\left\{|R_\ell \cap P_\ell'| \colon \ell \in [i - 2]\right\}, 
    \end{align*}
    demonstrating that $i - 2 = \argmin_{\ell = 1}^{i - 2} |R_\ell \cap P_\ell'|$. 

    Now, we obtain $Q_1, \ldots, Q_k$ using the following iterative procedure: For each $\ell \in [i - 3]$, if $(i - 2, \ell) \in P_{i - 2}'$, then 
    %\knote{define $Q_1, \ldots, Q_k$ as $Q_{i - 2} := P_{i - 2}' \setminus \{(i - 2, \ell), (\ell, i - 2)\}$, $Q_\ell := P_\ell' \cup \{(i - 2, \ell), (\ell, i - 2)\}$ and $Q_t:=P_t'$ for all $t \notin \{i - 2, \ell\}$. Otherwise, define $Q_t:=P_t'$ for all $t\in [k]$. Then, $Q_1, \ldots, Q_k$ is a symmetric multiway partition. We will show that $Q_1, \ldots, Q_k$ satisfies the properties required in the claim statement:}
    redefine $P_1', \ldots, P_k'$ such that $P_{i - 2}' := P_{i - 2}' \setminus \{(i - 2, \ell), (\ell, i - 2)\}$, $P_\ell' := P_\ell' \cup \{(i - 2, \ell), (\ell, i - 2)\}$ and $P_t'$ is unchanged for all $t \notin \{i - 2, \ell\}$. Let $Q_1, \ldots, Q_k$ be the parts obtained after the procedure is complete. Then, $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$. We will show that $Q_1, \ldots, Q_k$ satisfies the properties mentioned in the claim statement:
    \begin{enumerate}
        \item 
        As established above, $R_1 \subseteq P_1'$. Since no vertices are removed from $P_1'$ during the procedure, we have $R_1 \subseteq Q_1$. 

        \item 
        Since $U(P_1', \ldots, P_k') \subseteq P_1'$ and no vertices in $U(P_1', \ldots, P_k')$ change parts during the procedure, we have $U(Q_1, \ldots, Q_k) \subseteq Q_1$.

        \item 
        Since $\overleftarrow{R}_\ell \cap P_\ell' = \emptyset$ for each $\ell \in \{i - 1, \ldots, k\}$ and the procedure only changes parts for vertices $(x, y)$ in which $x, y \in [i - 2]$, we have $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ for each $\ell \in \{i - 1, \ldots, k\}$. Further, the procedure ensures that $\overleftarrow{R}_{i - 2} \cap Q_{i - 2} = \emptyset$. 

        \item 
        Since $\overrightarrow{R}_\ell \subseteq P_1' \cup P_\ell'$ for each $\ell \in \{i - 1, \ldots, k\}$ and the procedure only changes parts for vertices $(x, y)$ in which $x, y \in [i - 2]$, we have $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$ for each $\ell \in \{i - 1, \ldots, k\}$. Now, suppose for contradiction that $\overrightarrow{R}_{i - 2} \not\subseteq Q_1 \cup Q_{i - 2}$. Then, there exists $j \in \{i - 1, \ldots, k\}$ such that $(i - 2, j) \in Q_j$. However, $(j, i - 2) \in Q_j$ since $Q_1, \ldots, Q_k$ is symmetric, which contradicts $\overleftarrow{R}_j \cap Q_j = \emptyset$. 

        \item 
        As established above, we have $|R_{i - 1} \cap P_{i - 1}'| \geq |R_i \cap P_i'| \geq \ldots \geq |R_k \cap P_k'|$. Since the procedure only changes parts for vertices $(x, y)$ in which $x, y \in [i - 2]$, we have $R_\ell \cap P_\ell' = R_\ell \cap Q_\ell$ for each $\ell \in \{i - 1, \ldots, k\}$. Hence, $|R_{i - 1} \cap Q_{i - 1}| \geq |R_i \cap Q_i| \geq \ldots \geq |R_k \cap Q_k|$.

        \item We have that $\obj{P_1', \ldots, P_k'} \leq \obj{P_1, \ldots, P_k}$. Moreover, we have that $|R_{\ell}\cap P_{\ell}| \ge |R_{i-2}\cap P_{i-2}'|$ for every $\ell\in [i-3]$ by \eqref{eq:i-2-smallest} before the procedure and this inequality is preserved throughout the procedure. Hence, by Claim \ref{claim:move_pair}, we have that $\obj{P_1', \ldots, P_k'}$ does not increase during the procedure. Consequently, $\obj{Q_1 \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
        %\knote{Claim \ref{claim:move_pair} requires the hypothesis $|R_j\cap P_j|\ge |R_i\cap P_i|$ for the objective to be non-increasing. Applying it here requires $|R_{\ell}\cap P_{\ell}'|\ge |R_{i-2}\cap P_{i-2}'|$ as the hypothesis. Why does this hypothesis hold?}
    \end{enumerate}
\end{proof}

The next claim follows by applying Claim \ref{claim:induction-size} followed by Claim \ref{claim:induction-containment}. 
\begin{claim}\label{claim:induction}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ and let $i \in \{3, \ldots, k + 1\}$. Suppose $P_1, \ldots, P_k$ additionally satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P_1$, 
        
        \item $U(P_1, \ldots, P_k)\subseteq P_1$, 

        \item $\overleftarrow{R}_\ell \cap P_\ell = \emptyset$ for each $\ell \in \{i - 1, i, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq P_1 \cup P_\ell$ for each $\ell \in \{i - 1, i, \ldots, k\}$, and 

        \item $\left|R_i \cap P_i\right| \geq \left|R_{i + 1} \cap P_{i + 1}\right| \geq \ldots \geq \left|R_k \cap P_k\right|$. 
    \end{enumerate}
    Then there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ that additionally satisfies the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq Q_1$, 
        
        \item $U(Q_1, \ldots, Q_k) \subseteq Q_1$, 

        \item $\overleftarrow{R}_\ell \cap Q_\ell = \emptyset$ for each $\ell \in \{i - 2, i-1, \ldots, k\}$, 

        \item $\overrightarrow{R}_\ell \subseteq Q_1 \cup Q_\ell$ for each $\ell \in \{i - 2, i-1, \ldots, k\}$, 

        \item $\left|R_{i - 1} \cap Q_{i - 1}\right| \geq \left|R_i \cap Q_i\right| \geq \ldots \geq \left|R_k \cap Q_k\right|$, and 

        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$.
    \end{enumerate}
\end{claim}
%\begin{proof}
%    \knote{Relies on Claims 2.12, 2.13.}
%\end{proof}

We have the following corollary from Claim \ref{claim:induction} by induction. 
\begin{corollary}
\label{cor:partial_structure}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ such that $R_1 \subseteq P_1$ and $U(P_1, \ldots, P_k)\subseteq P_1$. Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that the following properties hold:
    \begin{enumerate}
        \item $R_1 \subseteq Q_1$, 

        \item $\overrightarrow{R}_i \subseteq Q_1 \cup Q_i$ for each $i \in \{2, \ldots, k\}$, 

        \item $\left|R_1 \cap Q_1\right| \geq \left|R_2 \cap Q_2\right| \geq \ldots \geq \left|R_k \cap Q_k\right|$, and 

        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
    \end{enumerate}
\end{corollary}
%\begin{proof}
    %\knote{Relies on Claim 2.11.}
%\end{proof}

The next claim will help in inductively achieving the required structure. It helps achieve a certain structure for parts with large size without increasing the objective value. 
\begin{claim}
\label{claim:move_to_j}
Let $j\in [k]$ and $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ with the following properties:
\begin{enumerate}
    %\item $R_1 \subseteq P_1$, 
    \item $\overrightarrow{R}_i\subseteq P_i$ for each $i\in [j-1]$, 
    \label{item:suffix_contained_geq_1}
    \item $\overrightarrow{R}_i \subseteq P_1\cup P_i$ for each $i \in \{j, \ldots, k\}$, and 
    \label{item:suffix_contained_geq_2}
    \item $|R_j \cap P_j| \geq \frac{k}{2} + 2$. 
    \end{enumerate}
Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that the following properties hold:
    \begin{enumerate}
        %\item $R_1\subseteq Q_1$, 
        \item $\overrightarrow{R}_i\subseteq Q_i$ for each $i\in [j]$, 
        \item $\overrightarrow{R}_i \subseteq Q_1\cup Q_i$ for each $i \in \{j+1, \ldots, k\}$, and 
        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$
    \end{enumerate}
\end{claim}
\begin{proof}
% \knote{There is an issue with $Q_i$s not being symmetric since we describe movements of only rows and not columns. This issue persists for the rest of the section. We will edit it at the end with a  symmetrizing macro or some such alternative.}. 
    We define $\overrightarrow{C}_{t}:=\{(i,t): i\in \{t+1, t+2, \ldots, k\}\}$ for each $t\in [k]$. 
    We set $Q_1 := P_1 \setminus (\overrightarrow{R}_j \cup \overrightarrow{C}_j)$, $Q_j := P_j \cup (\overrightarrow{R}_j\cup \overrightarrow{C}_j)$, and $Q_\ell := P_\ell$ for all $\ell \in [k] \setminus \{1, j\}$. Then, $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$ and the first two properties follow by definition. We now bound the objective value of $Q_1, \ldots, Q_k$. 

    We assume $j \neq 1$ since if $j = 1$, we have $Q_\ell = P_\ell$ for each $\ell \in [k]$ and the bound on the objective value follows immediately. We have 
    \begin{align*}
        &\obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} \\
        &\quad \quad \quad \quad = \sum_{i = 1}^k \left(\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right)\right) \\
        &\quad \quad \quad \quad = \sum_{i = j}^k \left(\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right)\right),
    \end{align*}
    since for each $i \in [j - 1]$ and $\ell \in [k]$, $R_i \cap Q_\ell = R_i \cap P_\ell$. 

    We let $a = |\overrightarrow{R}_j \cap P_1|$, $b = |\overrightarrow{R}_j \cap P_j|$, $c = |\overleftarrow{R}_j \cap P_1|$, and $d = |\overleftarrow{R}_j \cap P_j|$. By assumption, we have $b + d + 1 \geq \frac{k}{2} + 2$.
    Then, 
    \begin{align*}
        &\phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \sum_{\ell \in [k] - j} \left(\phin{R_j \cap Q_\ell} - \phin{R_j \cap P_\ell}\right) \\
        &= \phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \phin{R_j \cap Q_1} - \phin{R_j \cap P_1} \quad \text{(since $Q_\ell = P_\ell$ for all $\ell \in [k] \setminus \{1, j\}$)} \\
        &= \phi_t(a + b + d + 1) - \phi_t(b + d + 1) + \phi_n(c) - \phi_n(a + c) \\
        &= \frac{7}{8}k - \frac{7}{8}k + \phi_n(c) - \phi_n(a + c) \\
        &= -a \quad \text{(since $|R_j \cap P_j| \geq \frac{k}{2} + 2$, we have $a + c = |R_j \cap P_1| \leq \frac{k}{2} - 2$)}. 
    \end{align*}
    
    Now fix $i \in \{j + 1, \ldots, k\}$. We have
    \begin{align*}
        &\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) \\
        &= \phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j} \\
        &= \mathbbm{1}\left[(i, j) \in P_1\right]\left(\phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j}\right),
    \end{align*}
    since if $(i, j) \in P_j$, $R_i \cap Q_\ell = R_i \cap P_\ell$ for each $\ell \in [k]$.  
    Therefore,
    \begin{align*}
        &\sum_{i \in \{j + 1, \ldots, k\}} \left(\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) \\
        &= \sum_{i \in \{j + 1, \ldots, k\}} \mathbbm{1}\left[(i, j) \in P_1\right]\left(\phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j}\right) \\
        &= \sum_{i > j \colon (j, i) \in P_1} \left(\phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j}\right) \\
        &= \sum_{i > j \colon (j, i) \in P_1} \left(\phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + 1 - 0\right)\\
        & \quad \quad \quad \quad \quad \quad \text{(by properties \ref{item:suffix_contained_geq_1} and \ref{item:suffix_contained_geq_2} and since $(i, j) \in P_1$, $R_i \cap P_j = \emptyset$)} \\
        &\leq \sum_{i > j \colon (j, i) \in P_1} 1 \quad \text{(since $\phi_n$ is monotonic and $R_i \cap Q_1 \subseteq R_i \cap P_1$)} \\
        &= a.
    \end{align*}
    Hence, $\obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} \leq -a + a = 0$. 
\end{proof}

Our next claim builds on the previous claim and will help in inductively achieving the required structure. It helps achieve a certain structure for parts with small size without increasing the objective value. 
\begin{claim}
\label{claim:move_to_1}
Let $i^*, j\in [k]$ with $i^*<j$ and $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ with the following properties:
\begin{enumerate}
    %\item $R_1 \subseteq P_1$, 
    \item $\overrightarrow{R}_i\subseteq P_i$ for each $i\in [i^*]$, 
    \label{item:suffix_contained_leq_1}
    \item $\overrightarrow{R}_i\subseteq P_1$ for each $i\in \{i^* + 1, \ldots, j-1\}$, 
    \label{item:suffix_contained_leq_2}
    \item $\overrightarrow{R}_i \subseteq P_1\cup P_i$ for each $i \in \{j, \ldots, k\}$, and 
    \item $|R_j \cap P_j| \leq \frac{k}{2} + 1$. 
    \end{enumerate}
Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that the following properties hold:
    \begin{enumerate}
        %\item $R_1\subseteq Q_1$, 
        \item $\overrightarrow{R}_i\subseteq Q_i$ for each $i\in [i^*]$, 
        \item $\overrightarrow{R}_i\subseteq Q_1$ for each $i\in \{i^* + 1, \ldots, j-1, j\}$, 
        \item $\overrightarrow{R}_i \subseteq Q_1\cup Q_i$ for each $i \in \{j+1, \ldots, k\}$, and 
        \item $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$
    \end{enumerate}
\end{claim}
\begin{proof}
We define $\overrightarrow{C}_{t}:=\{(i,t): i\in \{t+1, t+2, \ldots, k\}$ for each $t\in [k]$. 
We set $Q_1 := P_1 \cup (\overrightarrow{R}_j \cup \overrightarrow{C}_j)$, $Q_j := P_j \setminus (\overrightarrow{R}_j\cup \overrightarrow{C}_j)$, and $Q_\ell := P_\ell$ for all $\ell \in [k] \setminus \{1, j\}$. Then, $Q_1, \ldots, Q_k$ is a symmetric multiway partition of $V$ and the first three properties follow by definition. We now bound the objective value of $Q_1, \ldots, Q_k$. 

    We begin by observing that $j \neq 1$ since $R_1 \subseteq P_1$ implies that $|R_1 \cap P_1| \geq \frac{k}{2} + 2$. We have  
    \begin{align*}
        &\obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} \\
        &\quad \quad \quad \quad = \sum_{i = 1}^k \left(\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right)\right) \\
        &\quad \quad \quad \quad = \sum_{i = j}^k \left(\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right)\right)
    \end{align*}
    since for each $i \in [j - 1]$ and $\ell \in [k]$, $R_i \cap Q_\ell = R_i \cap P_\ell$. 

    We let $a = |\overrightarrow{R}_j \cap P_1|$, $b = |\overrightarrow{R}_j \cap P_j|$, $c = |\overleftarrow{R}_j \cap P_1|$, and $d = |\overleftarrow{R}_j \cap P_j|$. By assumption, we have $b + d + 1 \leq \frac{k}{2} + 1$.
    Then,  
    \begin{align*}
        &\phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \sum_{\ell \in [k] - j} \left(\phin{R_j \cap Q_\ell} - \phin{R_j \cap P_\ell}\right) \\
        &= \phit{R_j \cap Q_j} - \phit{R_j \cap P_j} + \phin{R_j \cap Q_1} - \phin{R_j \cap P_1} \quad \text{(since $Q_\ell = P_\ell$ for all $\ell \in [k] \setminus \{1, j\}$)} \\
        &= \phi_t(d + 1) - \phi_t(b + d + 1) + \phi_n(a + b + c) - \phi_n(a + c) \\
        &\leq -b + b \quad \text{(since $b + d + 1 \leq \frac{k}{2} + 1$)} \\
        &= 0.
    \end{align*}

    Now, consider $i \in \{j + 1, \ldots, k\}$. If $(j, i) \in P_1$, then $R_i \cap Q_\ell = R_i \cap P_\ell$ for each $\ell \in [k]$, so $\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) = 0$. Hence, we assume $(j, i) \in P_j$. Then, 
    \begin{align*}
        &\phit{R_i \cap Q_i} - \phit{R_i \cap P_i} + \sum_{\ell \in [k] - i} \left(\phin{R_i \cap Q_\ell} - \phin{R_i \cap P_\ell}\right) \\
        &= \phin{R_i \cap Q_1} - \phin{R_i \cap P_1} + \phin{R_i \cap Q_j} - \phin{R_i \cap P_j} \\
        &\leq 1 + \phi_n(0) - \phi_n(1) \quad \text{(by properties \ref{item:suffix_contained_leq_1} and \ref{item:suffix_contained_leq_2}, $R_i \cap P_j = \{(i, j)\}$)} \\
        &= 1 - 1 \\
        &= 0.
    \end{align*}

    Hence, $\obj{Q_1, \ldots, Q_k} - \obj{P_1, \ldots, P_k} \leq 0$. 
\end{proof}


We have the following corollary from Claims \ref{claim:move_to_j} and \ref{claim:move_to_1}. 
\begin{corollary}
\label{cor:final_structure}
    %Let $V = [k] \times [k]$. 
    Let $P_1, \ldots, P_k$ be a symmetric multiway partition of $V$ with the following properties:
    \begin{enumerate}
        \item $R_1 \subseteq P_1$.

        \item $\overrightarrow{R}_i \subseteq P_1 \cup P_i$ for each $i \in \{2, \ldots, k\}$.

        \item $|R_1 \cap P_1| \geq |R_2 \cap P_2| \geq \ldots \geq |R_k \cap P_k|$.
    \end{enumerate}
    Then, there exists a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ with the following properties:
    \begin{enumerate}
        \item 
        There exists $i^* \in [k]$ such that $\overrightarrow{R}_i \subseteq Q_i$ for each $i \in [i^*]$ and $\overrightarrow{R}_i \subseteq Q_1$ for each $i \in \{i^* + 1, \ldots, k\}$. 

        \item 
        $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
    \end{enumerate}
\end{corollary}
\begin{proof}
    Since $R_1 \subseteq P_1$, we have that $k = |R_1 \cap P_1| \geq |R_2 \cap P_2| \geq \ldots \geq |R_k \cap P_k|\ge 1$. Since $k\ge 4$, there exists $i^* \in [k]$ such that $|R_i \cap P_i| \geq \frac{k}{2} + 2$ for each $i \in [i^*]$ and $|R_i \cap P_i| \leq \frac{k}{2} + 1$ for each $i \in \{i^* + 1, \ldots, k\}$. 
    Applying Claim \ref{claim:move_to_j} inductively for each $j\in [i^*]$ and then applying Claim \ref{claim:move_to_1} inductively for each $j\in \{i^*+1, \ldots, k\}$, we obtain the desired partition. 
    %We define the symmetric multiway partition $Q_1, \ldots, Q_k$ such that for each $i \in [i^*]$, $\overrightarrow{R}_i \subseteq Q_i$ and for each $i \in \{i^* + 1, \ldots, k\}$, $\overrightarrow{R}_i \subseteq Q_1$. By Claim \ref{claim:move_to_j} and Claim \ref{claim:move_to_1}, $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
\end{proof}

We now restate and prove Lemma \ref{lem:sym_part_structure}. 
\lemSymPartStructure*
\begin{proof}
    % \donote{}
    Let us define $P_1^{(0)}, \ldots, P_k^{(0)}$ such that $P_\ell^{(0)} = P_\ell$ for each $\ell \in [k]$. We arrive at the required symmetric multiway partition by a series of transformations as described below.
    \begin{enumerate}
        \item 
        Apply Claim \ref{claim:move-first-row} to the symmetric multiway partition $P_1^{(0)}, \ldots, P_k^{(0)}$ of $V$ and obtain a symmetric multiway partition $P_1^{(1)}, \ldots, P_k^{(1)}$ of $V$. We have that 
        \[\obj{P_1^{(1)}, \ldots, P_k^{(1)}} \leq \obj{P_1^{(0)}, \ldots, P_k^{(0)}} + k = \obj{P_1, \ldots, P_k} + k.
        \]

        \item The symmetric multiway partition $P_1^{(1)}, \ldots, P_k^{(1)}$ of $V$ satisfies the hypothesis of Claim \ref{claim:move-unhappy}. 
        Apply Claim \ref{claim:move-unhappy} 
        to the symmetric multiway partition $P_1^{(1)}, \ldots, P_k^{(1)}$ of $V$ and obtain a symmetric multiway partition $P_1^{(2)}, \ldots, P_k^{(2)}$ of $V$ such that (1) $R_1 \subseteq P_1^{(2)}$ and (2) $U\left(P_1^{(2)}, \ldots, P_k^{(2)}\right) \subseteq P_1^{(2)}$. We also have that 
        \[\obj{P_1^{(2)}, \ldots, P_k^{(2)}} \leq \obj{P_1^{(1)}, \ldots, P_k^{(1)}} \leq \obj{P_1, \ldots, P_k} + k.\]

        \item The symmetric multiway partition $P_1^{(2)}, \ldots, P_k^{(2)}$ of $V$ satisfies the hypothesis of Corollary \ref{cor:partial_structure}. 
        Apply Corollary \ref{cor:partial_structure} 
        to the symmetric multiway partition $P_1^{(2)}, \ldots, P_k^{(2)}$ of $V$ and obtain a symmetric multiway partition $P_1^{(3)}, \ldots, P_k^{(3)}$ of $V$ such that 
        \begin{enumerate}[label=(\roman*)]
            \item $R_1 \subseteq P_1^{(3)}$, 

            \item $\overrightarrow{R}_i \subseteq P_1^{(3)} \cup P_i^{(3)}$ for each $i \in \{2, \ldots, k\}$, and 

            \item $\left|R_1 \cap P_1^{(3)}\right| \geq \left|R_2 \cap P_2^{(3)}\right| \geq \ldots \geq \left|R_k \cap P_k^{(3)}\right|$. 
        \end{enumerate}
        We also have that 
        \[\obj{P_1^{(3)}, \ldots, P_k^{(3)}} \leq \obj{P_1^{(2)}, \ldots, P_k^{(2)}} \leq \obj{P_1, \ldots, P_k} + k. \]

        \item The symmetric multiway partition $P_1^{(3)}, \ldots, P_k^{(3)}$ of $V$ satisfies the hypothesis of Corollary \ref{cor:final_structure}. 
        Apply Corollary \ref{cor:final_structure} 
        to the symmetric multiway partition $P_1^{(3)}, \ldots, P_k^{(3)}$ of $V$ and obtain a symmetric multiway partition $Q_1, \ldots, Q_k$ of $V$ such that 
        %obtain a symmetric multiway partition $Q_1, \ldots, Q_k$ such that 
        there exists $i^* \in [k]$ such that $\overrightarrow{R}_i \subseteq Q_i$ for each $i \in [i^*]$ and $\overrightarrow{R}_i \subseteq Q_1$ for each $i \in \{i^* + 1, \ldots, k\}$. We also have that 
        \[\obj{Q_1, \ldots, Q_k} \leq \obj{P_1^{(3)}, \ldots, P_k^{(3)}} \leq \obj{P_1, \ldots, P_k} + k. \]
    \end{enumerate}
    %Since $\obj{Q_1, \ldots, Q_k} = \frac{1}{2} \sum_{i = 1}^k f(Q_i)$ and $\obj{P_1, \ldots, P_k} = \frac{1}{2} \sum_{i = 1}^k f(P_i)$, we see that $Q_1, \ldots, Q_k$ satisfies the properties required for Lemma \ref{lem:sym_part_structure}.
\end{proof}

% We consider the following instance of \monosubmp. Let $V = [k] \times [k]$. We define $R_i = \{(i, j) \colon j \in [k]\}$ and $C_j = \{(i, j) \colon i \in [k]\}$. For each $i \in [k]$, we let terminal $t_i = (i, i)$, and we define $T = \{t_i \colon i \in [k]\}$. Now, we define the function $f$ as follows. 

% Let $\phi_n \colon \mathbb{R} \rightarrow \mathbb{R}_{\geq 0}$ be defined such that $\phi_n(a) = \min\left\{a, \frac{7}{8}k\right\}$, and let $\phi_t \colon \mathbb{R} \rightarrow \mathbb{R}_{\geq 0}$ be defined such that $\phi_t(a) = \min\left\{\frac{3}{8}ka, \frac{3}{8}k + a - 1, \frac{7}{8}k \right\}$. Let $g \colon 2^V \rightarrow \mathbb{R}_{\geq 0}$ be defined as follows:
% \[
%     g(S) = \begin{cases} \phi_t(|S|) & \text{if } T \cap S \neq \emptyset, \\
%     \phi_n(|S|) & \text{otherwise.} \end{cases}
% \]
% Then we define $f(S) = \sum_{i = 1}^k \left(g(S \cap R_i) + g(S \cap C_i) \right)$. As in \cite{EVW}, we say a solution to this instance of \monosubmp is symmetric if for all $i, j \in [k]$, vertices $(i, j)$ and $(j, i)$ are assigned to the same part in the solution. 

% We will use the following definitions to bound the symmetry gap of this instance. First, we let $\widehat{R}_i = \{(i, j) \colon i < j \leq k \}$ and $\overline{R}_i = \{(i, j) \colon 1 \leq j < i\}$. Given a solution to the above instance of \monosubmp, we will index the parts of the solution from $1$ to $i$, and the $i$th part will contain $t_i$. (E.g. if $[P_1, P_2, \ldots, P_k]$ is a solution, then $t_1 \in P_1$, $t_2 \in P_2$, etc.) In a solution $[P_1, \ldots, P_k]$, a vertex $(i, j)$ is unhappy if $(i, j) \in P_\ell$ where $\ell \notin \{i, j\}$. Finally, for a symmetric solution $[P_1, \ldots, P_k]$, we define $\obj{P_1, \ldots, P_k} = \frac{1}{2} \sum_{\ell = 1}^k f(P_\ell)$. Observe that $\obj{P_1, \ldots, P_k} = \sum_{\ell = 1}^k \sum_{i = 1}^k g\left(P_\ell \cap R_i\right)$ since the symmetry of $[P_1, \ldots, P_k]$ ensures $|P_\ell \cap R_i| = |P_\ell \cap C_i|$.  

% \begin{lemma}
%     Given a symmetric solution $[P_1, \ldots, P_k]$ with $R_1 \subseteq P_1$, let $U = \{(i, j) \colon (i, j) \text{ is unhappy}\}$. 
%     Define $[Q_1, \ldots, Q_k]$ such that $Q_1 = P_1 \cup U$ and for each $\ell \geq 2$, $Q_\ell = P_\ell \setminus U$.
%     Then $\obj{Q_1, \ldots, Q_k} \leq \obj{P_1, \ldots, P_k}$. 
% \end{lemma}
% \begin{proof}
%     Fix $i \in \{2, \ldots, k\}$. Then we have
%     \begin{align*}
%         \sum_{\ell = 1}^k g(Q_\ell \cap R_i) - g(P_\ell \cap R_i) & = \phi_t\left(|Q_i \cap R_i|\right) - \phi_t\left(|P_i \cap R_i|\right) + \sum_{\ell \neq i} \left(\phi_n\left(|Q_\ell \cap R_i|\right) - \phi_n\left(|P_\ell \cap R_i|\right) \right) \\
%         &= \sum_{\ell \neq i} \left(\phi_n\left(|Q_\ell \cap R_i|\right) - \phi_n\left(|P_\ell \cap R_i|\right) \right) \quad \quad \text{(since $P_i \cap R_i \cap U = \emptyset$)} \\ 
%         &= \phi_n\left(|Q_1 \cap R_i|\right) - \phi_n\left(|P_1 \cap R_i|\right) + \sum_{\ell \notin \{1, i\}} \left(\phi_n\left(|Q_\ell \cap R_i|\right) - \phi_n\left(|P_\ell \cap R_i|\right)\right).
%     \end{align*}

%     We consider two cases based on $|Q_1 \cap R_i|$. 

%     \noindent \textbf{Case 1.} Suppose $|Q_1 \cap R_i| \leq \frac{7}{8}k$. We observe that 
%     \[
%         \sum_{\ell \neq i} \left(|Q_\ell \cap R_i| - |P_\ell \cap R_i|\right) = \sum_{\ell = 1}^k \left(|Q_\ell \cap R_i| - |P_\ell \cap R_i|\right) = 0.
%     \]
%     Then for each $\ell \in [k] \setminus \{1, i\}$, 
%     \[
%         |P_\ell \cap R_i| - |Q_\ell \cap R_i| \leq \sum_{\ell' \in \{1, i\}} \left(|P_\ell \cap R_i| - |Q_\ell \cap R_i|\right) = |Q_1 \cap R_i| - |P_1 \cap R_i|.
%     \]
%     Hence, for each $\ell \in [k] \setminus \{1, i\}$,
%     \begin{align*}
%         |P_\ell \cap R_i| &\leq |Q_1 \cap R_i| - |P_1 \cap R_i| + |Q_\ell \cap R_i| \\
%         &\leq |Q_1 \cap R_i| - |P_1 \cap R_i| + 1 \quad \quad \text{(since $Q_\ell \cap R_i \subseteq \{(i, \ell)\}$)} \\
%         &\leq |Q_1 \cap R_i| - 1 + 1 \quad \quad \text{(since $R_1 \subseteq P_1$, $(1, i) \in P_1$, so $(i, 1) \in P_1$)} \\
%         &\leq \frac{7}{8}k.
%     \end{align*}
    
% \end{proof}





==> sym-gap-to-query-lower-bound-1.tex <==
\subsubsection{Lower Bound from Symmetry Gap}
\knote{State the relevant lemmas from EVW and write a proof of the lower bound result.}

\begin{definition} 
\label{def:instance}
    Let $\phi_n, \phi_t \colon [k] \rightarrow \mathbb{R}$ be given functions. We define 
    \begin{enumerate}
        \item $V = [k] \times [k]$, $R_i = \{(i, j) \colon j \in [k]\}$ and $C_j = \{(i, j) \colon i \in [k]\}$. 
        \item $g \colon 2^V \rightarrow \mathbb{R}$ is defined such that 
        \[
            g(S) = \begin{cases} \phi_t(|S|) & \text{if } S \cap \{(i, i) \colon i \in [k]\} \neq \emptyset, \\
                                \phi_n(|S|) & \text{otherwise}; \end{cases}
        \]
        \item $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ is defined such that 
        \[
            f_{\phi_n, \phi_t}(S) = \sum_{i = 1}^k \left(g(S \cap R_i) + g(S \cap C_i)\right). 
        \] 
    \end{enumerate}
\end{definition}

\begin{definition}
\label{def:multilinear}
    Given $V$ and $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ as defined in Definition \ref{def:instance}, we define the multilinear extension of $f_{\phi_n, \phi_t}$ to be $F_{\phi_n, \phi_t} \colon [0, 1]^V \rightarrow \mathbb{R}$ such that 
    \[
        F_{\phi_n, \phi_t}(\vx) = \sum_{S \subseteq V} f_{\phi_n, \phi_t}(S) \prod_{v \in S} x_v \prod_{v \in V \setminus S} (1 - x_v). 
    \]
    We define the multilinear relaxation to be the following:
    \begin{align*}
        \text{minimize: } \sum_{\ell = 1}^k F_{\phi_n, \phi_t}\left(\vx_\ell\right) & \\
        \text{subject to: } \sum_{\ell = 1}^k x((i, j), \ell) = 1 & \quad \forall (i, j) \in V \\
        x((\ell, \ell), \ell) = 1 & \quad \forall \ell \in [k] \\
        x((i, j), \ell) \geq 0 & \quad \forall (i, j) \in V, \ell \in [k], 
    \end{align*}
    where $F_{\phi_n, \phi_t}$ is the multilinear extension of $f_{\phi_n, \phi_t}$ and $\vx_\ell = \left(x((i, j), \ell)\right)_{(i, j) \in V}$. We will say a vector $\vx = \left(x((i, j), \ell) \right)_{(i, j) \in V, \ell \in [k]} \in [0, 1]^{V \times [k]}$ is a solution to the multilinear relaxation if it satisfies the constraints of the multilinear relaxation. 
\end{definition}

\begin{definition}
    Let $V$ be defined as in \ref{def:instance}. 
    A partition of $V$ with parts $V_1, \ldots, V_k \subseteq V$ is symmetric if for all $(i, j) \in V$ and $\ell \in [k]$, $(i, j) \in V_\ell$ implies that $(j, i) \in V_\ell$. Generalizing, we say that a solution to the multilinear relaxation $\vx \in [0, 1]^{V \times [k]}$ is symmetric if for all $(i, j) \in V$ and $\ell \in [k]$, $x((i, j), \ell) = x((j, i), \ell)$. 
\end{definition}

% For properly chosen $\phi_n$ and $\phi_t$, $f_{\phi_n, \phi_t}$ is a non-negative monotone submodular function such that 
% \[
%     \min \left\{\sum_{i = 1}^k f_{\phi_n, \phi_t}(V_i) \colon V_1, \ldots, V_k \text{ is a partition of } V \text{ such that for each } i \in [k], (i, i) \in V_i \right\}
% \]
% is an instance of \monosubmp. For such $f_{\phi_n, \phi_t}$, we define the notion of a symmetry gap. 

\begin{definition}
\label{def:OPT_def}
    Let $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ be defined as in Definition \ref{def:instance}, we define the following two quantities:
    \[
    OPT = \min \left\{\sum_{i = 1}^k f_{\phi_n, \phi_t}(V_i) \colon V_1, \ldots, V_k \text{ is a partition of } V \text{ such that for each } i \in [k], (i, i) \in V_i \right\},
    \]
    and 
    \[
    \overline{OPT} = \min \left\{\sum_{i = 1}^k f_{\phi_n, \phi_t}(V_i) \colon V_1, \ldots, V_k \text{ is a symmetric partition of } V \text{ such that for each } i \in [k], (i, i) \in V_i \right\}.
    \]
    We define the symmetry gap of $f_{\phi_n, \phi_t}$, denoted $\text{Sym-Gap}(f_{\phi_n, \phi_t})$, to be $\overline{OPT} / OPT$. 
\end{definition}

\begin{lemma}
\label{lem:OPT_equality}
    Let $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ be defined as in Definition \ref{def:instance} and let $F_{\phi_n, \phi_t} \colon [0, 1]^V \rightarrow \mathbb{R}$ be the multilinear extension of $f_{\phi_n, \phi_t}$. Let $OPT$ and $\overline{OPT}$ be defined as in Definition \ref{def:OPT_def}. Then, 
    \begin{enumerate}
        \item $OPT = \min\left\{\sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\vx_\ell): \left(\vx_\ell \right)_{\ell \in [k]} \text{ is a solution to the multilinear relaxation} \right\}$  and 
        \item $\overline{OPT} = \min\left\{\sum_{\ell = 1}^k F_{\phi_n, \phi_t}\left(\overline{\vx}_\ell\right): \left(\overline{\vx}_\ell \right)_{\ell \in [k]} \text{ is a symmetric solution to the multilinear relaxation}\right\}$. 
    \end{enumerate}
\end{lemma}
\begin{proof}
    Let $OPT_{relax} = \min\{\sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\vx_\ell): \left(\vx_\ell \right)_{\ell \in [k]} \text{ is a solution to the multilinear relaxation} \}$. We show that $OPT = OPT_{relax}$. Let $V_1, \ldots, V_k$ be a partition of $V$ such that for each $i \in [k]$, $(i, i) \in V_i$ and $\sum_{i = 1}^k f_{\phi_n, \phi_t}(V_i) = OPT$, so $OPT_{relax} \leq OPT$. Defining $x((i, j), \ell) = \begin{cases} 1 & (i, j) \in V_\ell \\ 0 & (i, j) \notin V_\ell \end{cases}$, we see that $\left(x((i, j), \ell)\right)_{(i, j) \in V, \ell \in [k]}$ is a solution to the multilinear relaxation that obtains value $\sum_{\ell = 1}^k F_{\phi_n, \phi_t}\left(\left(x((i, j), \ell) \right)_{(i, j) \in V}\right) = OPT$. Now, let $\vx^*$ denote a solution to the multilinear relaxation realizing $OPT_{relax}$. We obtain a partition $V^*_1, \ldots, V^*_k$ by assigning each vertex $(i, j)$ independently such that the probability $(i, j)$ is assigned to $V^*_\ell$ is $x^*((i, j), \ell)$. We observe that $V^*_1, \ldots, V^*_k$ is a partition of $V$ such that for each $i \in [k]$, $(i, i) \in V^*_i$. Then, $\E \left[ f_{\phi_n, \phi_t}(V^*_\ell) \right] = \sum_{S \subseteq V} f_{\phi_n, \phi_t}(S) \prod_{(i, j) \in S} x^*((i, j), \ell) \prod_{(i, j) \in V \setminus S} (1 - x^*((i, j), \ell)) = F_{\phi_n, \phi_t}(\vx^*_\ell)$. Hence, $\E \left[ \sum_{\ell = 1}^k f_{\phi_n, \phi_t}(V^*_\ell) \right] = \sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\vx^*_\ell) = OPT_{relax}$. This implies that there exists a partition $V_1, \ldots, V_k$ satisfying $(i, i) \in V_i$ for each $i \in [k]$ such that $\sum_{\ell = 1}^k f_{\phi_n, \phi_t}(V_\ell) \leq OPT_{relax}$, so $OPT = OPT_{relax}$. 

    We define $\overline{OPT}_{relax} = \min\left\{\sum_{\ell = 1}^k F_{\phi_n, \phi_t}\left(\overline{\vx}_\ell\right): \left(\overline{\vx}_\ell \right)_{\ell \in [k]} \text{ is a symmetric solution to the multilinear relaxation}\right\}$. Now, we show that $\overline{OPT} = \overline{OPT}_{relax}$. Using identical reasoning to the previous paragraph, we see that $\overline{OPT}_{relax} \leq \overline{OPT}$. Let $\overline{\vx}$ be a symmetric solution to the multilinear realxation that realizes $\overline{OPT}_{relax}$. We obtain a partition $V^*_1, \ldots, V^*_k$ of $V$ in the same manner as the previous paragraph. We also obtain a partition $\overline{V}_1, \ldots, \overline{V}_k$ by independently assigning each set $\{(i, j), (j, i)\}$ such that the probability $\{(i, j), (j, i)\} \subseteq \overline{V}_\ell$ is $\overline{x}((i, j), \ell) = \overline{x}((j, i), \ell)$. Observe that $V^*_1, \ldots, V^*_k$ is not necessarily a symmetric partition of $V$, but $\overline{V}_1, \ldots, \overline{V}_k$ is a symmetric partition of $V$. By the reasoning of the above paragraph, we have $\E \left[\sum_{\ell = 1}^k f_{\phi_n, \phi_t}(V^*_\ell)\right] = \overline{OPT}_{relax}$. 

    Now, fix $i, \ell \in [k]$. We have 
    \begin{align*}
        \E \left[ g\left(\overline{V}_\ell \cap R_i\right) \right] &= \sum_{S \subseteq R_i} g(S) \Pr \left[ \overline{V}_\ell \cap R_i = S\right] \\
        &= \sum_{S \subseteq R_i} g(S) \prod_{(i, j) \in S} \bar{x}((i, j), \ell) \prod_{(i, j) \in R_i \setminus S} (1 - \bar{x}((i, j), \ell)) \quad \quad \text{(each $(i, j) \in R_i$ is assigned independently)} \\
        &= \sum_{S \subseteq R_i} g(S) \Pr \left[ V^*_\ell \cap R_i = S\right] \\
        &= \E \left[ g\left(V^*_\ell \cap R_i\right) \right]. 
    \end{align*}
    Similar reasoning shows that $\E \left[ g\left(\overline{V}_\ell \cap C_i\right) \right] = \E \left[ g(V^*_\ell \cap C_i) \right]$. 
    Hence, we have 
    \begin{align*}
        \E \left[ \sum_{\ell = 1}^k f_{\phi_n, \phi_t}\left(\overline{V}_\ell\right) \right] &= \sum_{\ell = 1}^k \sum_{i = 1}^k \left(\E \left[ g\left(\overline{V}_\ell \cap R_i\right)\right] + \E \left[ g\left(\overline{V}_\ell \cap C_i\right) \right]\right)\\ 
        &= \sum_{\ell = 1}^k \sum_{i = 1}^k \left(\E \left[ g(V^*_\ell \cap R_i) \right] + \E \left[ g(V^*_\ell \cap R_i) \right]\right) \\
        &= \E \left[ \sum_{\ell = 1}^k f_{\phi_n, \phi_t}(V^*_\ell) \right] \\
        &= \overline{OPT}_{relax}. 
    \end{align*}
    This demonstrates that there exists an symmetric partition $V_1, \ldots, V_k$ of $V$ satisfying $(i, i) \in V_i$ for each $i \in [k]$ such that $\overline{OPT} \leq \sum_{\ell = 1}^k f_{\phi_n, \phi_t}(V_\ell) \leq \overline{OPT}_{relax}$. 
\end{proof}

Now, we will appeal to several lemmas from \cite{EVW} to prove our result on the inapproximability of \monosubmp. 

\knote{Cite Vondrak's journal paper instead of EVW.}

\begin{lemma}[Lemma 3.2 from \cite{EVW}] 
\label{lem:EVW_continuous}
    Consider a function $f \colon 2^V \rightarrow \mathbb{R}$ that is invariant under a group of permutations $\mathcal{G}$ on the ground set $V$. Let $F$ be the multilinear extension of $f$, $\overline{\vx} = \E_{\sigma \in \mathcal{G}} \left[\sigma(\vx)\right]$, and fix an arbitrary $\epsilon > 0$. Then, there exists $\delta > 0$ and functions $\hat{F}, \hat{G} \colon [0, 1]^V \rightarrow \mathbb{R}_+$ (which are also symmetric with respect to $\mathcal{G}$) \knote{What does symmetric with respect to $\mathcal{G}$ mean?} \rnote{I think this means that $\hat{F}$ and $\hat{G}$ are invariant under $\mathcal{G}$}, satisfying:
    \begin{enumerate}
        \item For all $\vx \in [0, 1]^V$, $\hat{G}(\vx) = \hat{F}(\overline{\vx})$.

        \item For all $\vx \in [0, 1]^V$, $|\hat{F}(\vx) - F(\vx)| \leq \epsilon$. 

        \item Whenever $\|\vx - \overline{\vx}\|^2 \leq \delta$, $\hat{F}(\vx) = \hat{G}(\vx)$ and the value depends only on $\overline{\vx}$. 

        \item The first partial derivatives of $\hat{F}$ and $\hat{G}$ are absolutely continuous.

        \item If $f$ is monotone, then $\frac{\partial \hat{F}}{\partial x_i} \geq 0$ and $\frac{\partial \hat{G}}{\partial x_i} \geq 0$ everywhere. \label{label:monotone}

        \item If $f$ is submodular, then $\frac{\partial^2 \hat{F}}{\partial x_i \partial x_j} \leq 0$ and $\frac{\partial^2 \hat{G}}{\partial x_i \partial x_j} \leq 0$ almost everywhere. \label{submodular}
    \end{enumerate}
\end{lemma}

\begin{lemma}[Lemma 3.3 from \cite{EVW}]
\label{lem:EVW_discrete}
    Let $H \colon [0, 1]^V \rightarrow \mathbb{R}$ be a function with absolutely continuous first partial derivatives. Let $N = [n]$, $n \geq 1$, and define $h \colon N \times V \rightarrow \mathbb{R}$ so that $h(S) = H(\vx)$ where $x_i = \frac{1}{n}|S \cap (N \times \{i\})|$. Then
    \begin{enumerate}
        \item If $\frac{\partial H}{\partial x_i} \geq 0$ everywhere for each $i$, then $h$ is monotone. 

        \item If $\frac{\partial^2 H}{\partial x_i \partial x_j} \leq 0$ almost everywhere for all $i, j$, then $h$ is submodular.
    \end{enumerate}
\end{lemma}

% Using $f \colon 2^V \rightarrow \mathbb{R_+}$ defined in Section \ref{subsect:sym_gap}, we define $\hat{F}$ and $\hat{G}$ from $f$ as in Lemma \ref{lem:EVW_continuous} (the value of $\epsilon$ will be chosen later). We consider two permutations of $V$, the identity and transpose, denoted $id \colon V \rightarrow V$ and $tr \colon V \rightarrow V$, respectively. For each $(i, j) \in V$, $id(i, j) = (i, j)$ and $tr(i, j) = (j, i)$. We extend $id$ and $tr$ to $[0, 1]^V$ in the natural fashion: for $\vx \in [0, 1]^V$, $id(\vx) = \vx$ and $tr(\vx) = \vx^T$ where $x^T(i, j) = x(j, i)$ for each $(i, j) \in V$. The group of permutations $\mathcal{G}$ that we use to define $\hat{F}$ and $\hat{G}$ is $\mathcal{G} = \{id, tr\}$. Hence, $\overline{\vx}$ is defined such that $\overline{x}(i, j) = \frac{1}{2} x(i, j) + \frac{1}{2} x(j, i)$ for each $(i, j) \in V$. 

% Next, for $n \geq 1$, which we will choose later, let $N = [n]$ and $X = N \times V$. For each $r \in N$, choose a permutation $\sigma^{(r)} \in \{id, tr\}$, each with probability $\frac{1}{2}$. Now, for $S \subseteq X$, we define the vector $\xi(S) \in [0, 1]^V$ such that 
% \[
%     \xi(S)_{(i, j)} = \frac{1}{n}\left|\left\{r \in N \colon \left(r, \sigma^{(r)}(i, j)\right) \in S\right\}\right|. 
% \]
% Finally, we define $\hat{f}, \hat{g} \colon X \rightarrow \mathbb{R}_+$ such that $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. By applying Lemmas \ref{lem:EVW_continuous} and \ref{lem:EVW_discrete}, we see that $\hat{f}$ and $\hat{g}$ are monotone submodular functions. As described in \cite{Vondrak}, for the purposes of proving the monotonicity and the submodularity of $\hat{f}$ and $\hat{g}$, it suffices to assume that $\sigma^{(r)} = id$ for all $r \in N$. We now consider the following instances of \monosubmp:
% \begin{align*}
%     &\min\left\{\sum_{\ell = 1}^k \hat{f}(S_\ell) \colon [S_1, \ldots, S_k] \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}, \\
%     &\min\left\{\sum_{\ell = 1}^k \hat{g}(S_\ell) \colon [S_1, \ldots, S_k] \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}. 
% \end{align*}
% For each $\ell \in [k]$, we can contract $N \times (\ell, \ell)$ into a single vertex such that we specify exactly one terminal per part $S_\ell \in [S_1, \ldots, S_k]$. 

% To prove our hardness result, we will need the following lemma from \cite{EVW}.

\begin{lemma}[Lemma 3.4 from \cite{EVW}]
\label{lem:EVW_distinguish}
    Let $\hat{F}$, $\hat{G}$ be two functions provided by Lemma \ref{lem:EVW_continuous}. For a parameter $n \in \mathbb{Z}_+$ and $N = [n]$, define two discrete functions $\hat{f}, \hat{g} \colon 2^{N \times V} \rightarrow \mathbb{R}_+$ as follows: Let $\sigma^{(r)}$ be chosen uniformly at random in $\mathcal{G}$ for each $r \in N$. For every set $S \subseteq N \times V$, we define a vector $\xi(S) \in [0, 1]^V$ by 
    \[
        \xi(S)_{(i, j)} = \frac{1}{n} |\{r \in N \colon (r, \sigma^{(r)}(i, j) \in S\}|. 
    \]
    Let us define: $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. Then deciding whether a function given by a value oracle is $\hat{f}$ or $\hat{g}$ (even using a randomized algorithm with a constant probability of success) requires an exponential number of queries in $n$. 
\end{lemma}

\begin{theorem}
    Let $V$ and $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ be defined as in Definition \ref{def:instance} such that $f_{\phi_n, \phi_t}$ is non-negative monotone submodular. We define $OPT$ and $\overline{OPT}$ as in Definition \ref{def:OPT_def}. Then for all $\gamma > 0$ and sufficiently large $n \in \mathbb{Z_+}$, there exists a non-negative monotone submodular function $\hat{f} \colon 2^{[n] \times V} \rightarrow \mathbb{R_+}$ and a set of terminals $\{t_1, \ldots, t_k\}$ such that all approximation algorithms for \monosubmp require an exponential number of oracle queries in $n$ to achieve an $\left(\frac{\overline{OPT}}{OPT} - \gamma\right)$-approximation for the following instance of \monosubmp 
    \[
        \min\left\{\sum_{\ell = 1}^k \hat{f}(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } [n] \times V \text{ such that } t_\ell \in X_\ell \text{ for each } \ell \in [k]\right\}. 
    \]
\end{theorem}
\begin{proof}
    First, we define $\hat{F}$ and $\hat{G}$ from $f_{\phi_n, \phi_t}$ as in Lemma \ref{lem:EVW_continuous} (the value of $\epsilon$ will be chosen later). We consider two permutations of $V$, the identity and transpose, denoted $id \colon V \rightarrow V$ and $tr \colon V \rightarrow V$, respectively. For each $(i, j) \in V$, $id(i, j) = (i, j)$ and $tr(i, j) = (j, i)$. We extend $id$ and $tr$ to $[0, 1]^V$ in the natural fashion: for $\vx \in [0, 1]^V$, $id(\vx) = \vx$ and $tr(\vx) = \vx^T$ where $x^T(i, j) = x(j, i)$ for each $(i, j) \in V$. The group of permutations $\mathcal{G}$ that we use to define $\hat{F}$ and $\hat{G}$ is $\mathcal{G} = \{id, tr\}$. Hence, $\overline{\vx}$ is defined such that $\overline{x}(i, j) = \frac{1}{2} x(i, j) + \frac{1}{2} x(j, i)$ for each $(i, j) \in V$. 

    Next, for $n \geq 1$, which we will choose later, let $N = [n]$ and $X = N \times V$. For each $r \in N$, choose a permutation $\sigma^{(r)} \in \{id, tr\}$, each with probability $\frac{1}{2}$. Now, for $S \subseteq X$, we define the vector $\xi(S) \in [0, 1]^V$ such that 
    \[
        \xi(S)_{(i, j)} = \frac{1}{n}\left|\left\{r \in N \colon \left(r, \sigma^{(r)}(i, j)\right) \in S\right\}\right|. 
    \]

    Now, we define $\hat{f}, \hat{g} \colon X \rightarrow \mathbb{R}_+$ such that $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. By applying Lemmas \ref{lem:EVW_continuous} and \ref{lem:EVW_discrete}, we see that $\hat{f}$ and $\hat{g}$ are monotone submodular functions. As described in \cite{Vondrak}, for the purposes of proving the monotonicity and the submodularity of $\hat{f}$ and $\hat{g}$, it suffices to assume that $\sigma^{(r)} = id$ for all $r \in N$.

    Fix $\epsilon > 0$. We demonstrate that for all partitions $X_1, \ldots, X_k$ of $X = N \times V$ such that $(r, (\ell, \ell)) \in X_\ell$ for each $r \in N$ and $\ell \in [k]$, $\sum_{\ell = 1}^k \hat{g}(X_\ell) \geq \overline{OPT} - \epsilon k$. By Lemma \ref{lem:EVW_continuous}, we have 
    \begin{align*}
        \sum_{\ell = 1}^k \hat{g}(X_\ell) &= \sum_{\ell = 1}^k \hat{G}(\xi(X_\ell)) \\
        &= \sum_{\ell = 1}^k \hat{F}(\overline{\xi(X_\ell)}) \\
        &\geq \sum_{\ell = 1}^k (F_{\phi_n, \phi_t}(\overline{\xi(X_\ell)}) - \epsilon) \\
        &= \sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\overline{\xi(X_\ell)}) - \epsilon k. 
    \end{align*}
    We observe that $\left(\overline{\xi(X_\ell)}\right)_{\ell = 1}^k$ is a feasible symmetric solution to the multilinear relaxation. Hence, $\sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\overline{\xi(X_\ell)}) \geq \overline{OPT}$, using the result of Lemma \ref{lem:OPT_equality}. Thus, $\sum_{\ell = 1}^k \hat{g}(X_\ell) \geq \overline{OPT} - \epsilon k$. 

    Now, we demonstrate that for sufficiently large $n$ there exists a partition $X_1, \ldots, X_k$ of $X = N \times V$ satisfying $(r, (\ell, \ell)) \in X_\ell$ for each $r \in N$ and $\ell \in [k]$ such that $\sum_{\ell = 1}^k \hat{f}(X_\ell) \leq OPT + \epsilon (k + 1)$. First, let $\vx^*$ be a solution to the multilinear relaxation defined in Definition \ref{def:multilinear} with value $OPT$. Because the objective of the multilinear relaxation is continuous, we may choose $n$ large enough such that there exists a feasible solution to the multilinear relaxation $\tilde{\vx}$ such that the entries of $\tilde{\vx}$ are all rational number with $n$ in the denominator and $\sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\tilde{\vx}_\ell) \leq \sum_{\ell = 1}^k F_{\phi_n, \phi_t}(\vx^*_\ell) + \epsilon$. $\tilde{\vx} = \left(\xi(X_\ell)\right)_{\ell = 1}^k$ for the partition $X_1, \ldots, X_k$ defined as follows. Fix $i, j \in [k]$. Then for $1 \leq r \leq nx((i, j), 1)$, let $(r, \sigma^{(r)}(i, j))$ be assigned to $X_1$, for $nx((i, j), 1) + 1 \leq r \leq nx((i, j), 1) + nx((i, j), 2)$ let $(r, \sigma^{(r)}(i, j))$ be assigned to $X_2$, etc. Therefore, 
    \begin{align*}
        \sum_{\ell = 1}^k \hat{f}(X_\ell) &= \sum_{\ell = 1}^k \hat{F}(\tilde{\vx}_\ell)\\
        &\leq \sum_{\ell = 1}^k \left(F(\tilde{\vx}_\ell) + \epsilon\right) \\
        &= \sum_{\ell = 1}^k F(\tilde{\vx}_\ell) + \epsilon k \\
        &\leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon(k + 1) \\
        &= OPT + \epsilon(k + 1). 
    \end{align*}

    Now fix $\gamma > 0$. We choose $\epsilon > 0$ such that $\frac{\overline{OPT} - \epsilon k}{OPT + \epsilon(k + 1)} > \frac{\overline{OPT}}{OPT} - \gamma$. Then fix $n \in \mathbb{Z}_+$ large enough such that there exists a feasible solution $\tilde{\vx}$ to the multilinear relaxation such that the entries of $\tilde{\vx}$ are all rational number with $n$ in the denominator and $\sum_{\ell = 1}^k F(\tilde{\vx}_\ell) \leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon$, where $\vx^*$ is the optimal solution to the multilinear relaxation. Then, we consider the following instance of \monosubmp:
    \[
        \min\left\{\sum_{\ell = 1}^k \hat{f}(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}. 
    \]
    For each $\ell \in [k]$, we can contract $N \times (\ell, \ell)$ into a single vertex $t_\ell$ such that we specify exactly one terminal per part $X_\ell \in \{X_1, \ldots, X_k\}$. Suppose for contradiction there exists an approximation algorithm for \monosubmp that achieves an $\left(\frac{\overline{OPT}}{OPT} - \gamma\right)$-approximation algorithm for the above instance of \monosubmp using fewer than exponentially-many oracle queries in $n$. 
    
    Given an oracle for an unknown function $h \in \{\hat{f}, \hat{g}\}$, we apply this algorithm to the following instance of \monosubmp:
    \[
        \min\left\{\sum_{\ell = 1}^k h(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}. 
    \]
    Let the value returned by the algorithm be $\beta$. If $\beta < \overline{OPT} - \epsilon k$, then we declare that $h = \hat{f}$. Otherwise, $\beta \geq \overline{OPT} - \epsilon k$ and we declare that $h = \hat{g}$. 
    
    We show that the identity of $h$ is correctly determined. If in reality $h = \hat{f}$, then $\beta \leq (OPT + \epsilon(k + 1)) \left( \frac{\overline{OPT}}{OPT} - \gamma \right) < (OPT + \epsilon(k + 1)) \left( \frac{\overline{OPT} - \epsilon k}{OPT + \epsilon(k + 1)}  \right) = \overline{OPT} - \epsilon k$. If in reality $h = \hat{g}$, then $\beta \geq \overline{OPT} - \epsilon k$. We correctly determine the identity of $h$ using fewer than an exponential number of oracle queries in $n$. However, this contradicts Lemma \ref{lem:EVW_distinguish}. We conclude that all algorithms achieving a $\left(\frac{\overline{OPT}}{OPT} - \gamma\right)$-approximation to the above instance of \monosubmp require exponentially many oracle queries in $|X|$.
\end{proof}

==> sym-gap-to-query-lower-bound-2.tex <==
\subsubsection{Lower Bound from Symmetry Gap}
\label{subsec:sym_gap_to_query-complexity}

%Let $V=[k]\times [k]$ and $f: 2^V\rightarrow \R$ be a set function defined over the set $V$. For a set $A\subseteq V$, we denote $A^T:=\{(j,i): (i,j)\in A\}$. 
In this section, we %define the notion of symmetry gap and 
prove that the approximation factor of an algorithm that makes polynomial number of function evaluation queries should be at least the symmetry gap, i.e., prove Theorem \ref{thm:sym-gap-to-oracle-lower-bound}. Our proof approach is similar to the proof approaches in \cite{Vondrak, EVW}, but we have to work out the details since we are interested in \monosubmp which was not the focus of those two works. 
%which does not follow immediately from the results in \cite{Vondrak, EVW}. 
%We encourage first-time readers to skip this section. 
We begin by showing that \opt and \symopt can be obtained as optimum solutions to the multilinear relaxation. We define the multilinear extension and the multilinear relaxation of the multiway partitioning problem. 

\begin{definition}
Let $V=[k]\times [k]$ and $f: 2^V\rightarrow \R$ be a set function. 
%Let $U$ be a ground set and $h:2^U\rightarrow \R$ be a set function. 
    \begin{enumerate}
    \item The \emph{multilinear extension} of $f$ is the function $F \colon [0, 1]^V \rightarrow \mathbb{R}$ defined by
        \[
        F(\vx) = \sum_{S \subseteq V} f(S) \left(\prod_{v \in S} x_v \prod_{v \in V \setminus S} (1 - x_v)\right). 
        \]
    \iffalse
        \item The \emph{multilinear extension} of $h$ is the function $H \colon [0, 1]^V \rightarrow \mathbb{R}$ defined by
        \[
        H(\vx) = \sum_{S \subseteq V} h(S) \prod_{v \in S} x_v \prod_{v \in V \setminus S} (1 - x_v). 
        \]
        \fi
    \iffalse
    \item The \emph{multilinear relaxation} of the multiway partitioning problem over $V$ for a pairwise disjoint collection of terminal sets $T_1, \ldots, T_k\subseteq U$ is 
    \begin{align*}
        \text{min} \sum_{\ell = 1}^k H\left(\vx_\ell\right) & \\
        \text{subject to } \sum_{\ell = 1}^k x(u, \ell) = 1 & \quad \forall u \in U \\
        x(u, \ell) = 1 & \quad \forall u\in T_{\ell},\ \ell \in [k] \\
        x(u, \ell) \geq 0 & \quad \forall u \in U, \ell \in [k], 
    \end{align*}
    where $\vx_\ell = \left(x(u, \ell)\right)_{u \in U}$. We will say that a vector $\vx = \left(x(u, \ell) \right)_{u \in U, \ell \in [k]} \in [0, 1]^{U \times [k]}$ is a solution to the multilinear relaxation if it satisfies the constraints of the multilinear relaxation.
    \fi
    %\iffalse
    \item The \emph{multilinear relaxation} of the multiway partitioning problem over $V$ wrt $f$ for the set $\{(\ell,\ell): \ell\in [k]\}$ of terminals is 
    \begin{align*}
        \text{min} \sum_{\ell = 1}^k F\left(\vx_\ell\right) & \\
        \text{subject to } \sum_{\ell = 1}^k x((i, j), \ell) = 1 & \quad \forall (i, j) \in V \\
        x((\ell, \ell), \ell) = 1 & \quad \forall \ell \in [k] \\
        x((i, j), \ell) \geq 0 & \quad \forall (i, j) \in V, \ell \in [k], 
    \end{align*}
    where $\vx_\ell = \left(x((i, j), \ell)\right)_{(i, j) \in V}$. We will say that a vector $\vx = \left(x((i, j), \ell) \right)_{(i, j) \in V, \ell \in [k]} \in [0, 1]^{V \times [k]}$ is a solution to the multilinear relaxation if it satisfies the constraints of the multilinear relaxation.
    %\fi
    \end{enumerate}
\end{definition}

The following lemma shows that both \opt and \symopt can be expressed as optimum solutions to the multilinear relaxation and a symmetry constrained multilinear relaxation respectively. 
\begin{lemma}
\label{lem:OPT_equality}
    %Let $f_{\phi_n, \phi_t} \colon 2^V \rightarrow \mathbb{R}$ be defined as in Definition \ref{def:instance} and let $F_{\phi_n, \phi_t} \colon [0, 1]^V \rightarrow \mathbb{R}$ be the multilinear extension of $f_{\phi_n, \phi_t}$. Let $OPT$ and $\overline{OPT}$ be defined as in Definition \ref{def:OPT_def}. Then, 
    Let $V=[k]\times [k]$ and let $f:2^V\rightarrow \R$ be a row-column-type set function defined over the set $V$. 
    We have the following: 
    \begin{enumerate}
        \item $\opt(f) = \min\left\{\sum_{\ell = 1}^k F(\vx_\ell): \left(\vx_\ell \right)_{\ell \in [k]} \text{ is a feasible solution to the multilinear relaxation} \right\}$  and 
        \item %$\symopt(f) = \min\left\{\sum_{\ell = 1}^k F\left(\overline{\vx}_\ell\right): \left(\overline{\vx}_\ell \right)_{\ell \in [k]} \text{ is a symmetric feasible solution to the multilinear relaxation}\right\}$.
        $\symopt(f) = \min\left\{\sum_{\ell = 1}^k F\left(\vy_\ell\right): \left(\vy_\ell \right)_{\ell \in [k]} \text{ is a symmetric feasible solution to the multilinear relaxation}\right\}$.
    \end{enumerate}    
\end{lemma}
\begin{proof}
%\donote{Proof needs to be edited to adhere to the lemma statement.}  
For simplicity, we denote $\opt = \opt(f)$ and $\symopt = \symopt(f)$. 
\begin{enumerate}
    \item Let $\mlopt = \min\{\sum_{\ell = 1}^k F(\vx_\ell): \left(\vx_\ell \right)_{\ell \in [k]} \text{ is a feasble solution to the multilinear relaxation} \}$. We show that $\opt = \mlopt$. Let $V_1, \ldots, V_k$ be a partition of $V$ such that $(i, i) \in V_i$ for each $i \in [k]$ and $\sum_{i = 1}^k f(V_i) = OPT$. For every $i, j, \ell\in [k]$, we define 
    \[
    x((i, j), \ell) = \begin{cases} 1 & \text{ if } (i, j) \in V_\ell, \\ 0 & \text{ if } (i, j) \notin V_\ell. \end{cases}
    \]
    Then, $\left(x((i, j), \ell)\right)_{(i, j) \in V, \ell \in [k]}$ is a feasible solution to the multilinear relaxation and its objective value is $\sum_{\ell = 1}^k F\left(\left(x((i, j), \ell) \right)_{(i, j) \in V}\right) = \opt$. Consequently, $\mlopt\le \opt$. Next, let $\vx^*$ be an optimum solution to the multilinear relaxation. 
    We obtain a partition $V^*_1, \ldots, V^*_k$ of $V$ by assigning each element $(i,j)\in V$ to one of the parts as follows: consider an element $(i, j)\in V$; 
    we define $z_0:=0$ and $z_{\ell}:=\sum_{m=1}^{\ell}x^*((i,j),m)$ for every $\ell\in [k]$, pick $\theta\in [0,1]$ uniformly at random, and assign $(i,j)$ to $V_{\ell}$ such that $z_{\ell-1}\le \theta < z_{\ell}$. We note that each element $(i,j)$ is assigned to a part $V^*_{\ell}$ independently with probability $x((i,j), \ell)$. 
    %we assign it to $V^*_{\ell}$ independently such that the probability $(i, j)$ is assigned to $V^*_\ell$ is $x^*((i, j), \ell)$ \knote{Need to explain better}. 
    We observe that $V^*_1, \ldots, V^*_k$ is a partition of $V$ with $(i, i) \in V^*_i$ for every $i\in [k]$. Moreover, $\E \left[ f(V^*_\ell) \right] = \sum_{S \subseteq V} f(S) \prod_{(i, j) \in S} x^*((i, j), \ell) \prod_{(i, j) \in V \setminus S} (1 - x^*((i, j), \ell)) = F(\vx^*_\ell)$. Hence, $\E \left[ \sum_{\ell = 1}^k f(V^*_\ell) \right] = \sum_{\ell = 1}^k F(\vx^*_\ell) = \mlopt$. This implies that there exists a partition $V_1, \ldots, V_k$ with $(i, i) \in V_i$ for each $i \in [k]$ such that $\sum_{\ell = 1}^k f(V_\ell) \leq \mlopt$, so $OPT \le \mlopt$. 

    \item Let $\mlsymopt = \min\left\{\sum_{\ell = 1}^k F\left(\overline{\vx}_\ell\right): \left(\overline{\vx}_\ell \right)_{\ell \in [k]} \text{ is a symmetric solution to the multilinear relaxation}\right\}$. We show that $\symopt = \mlsymopt$. Using identical reasoning to the previous paragraph, we have that $\mlsymopt \leq \symopt$. Let $\vy$ be an optimum symmetric solution to the multilinear relaxation. We obtain a partition $V^*_1, \ldots, V^*_k$ of $V$ in the same manner as the previous paragraph from $\vy$. 
    By the reasoning of the above paragraph, we have $\E \left[\sum_{\ell = 1}^k f(V^*_\ell)\right] = \mlsymopt$. 
    We recall that $\vy$ is a symmetric feasible solution to the multilinear relaxation but the the partition $V^*_1, \ldots, V^*_k$ need not be symmetric. 
    In addition to the partition $V^*_1, \ldots, V^*_k$, we obtain a symmetric partition $\overline{V}_1, \ldots, \overline{V}_k$ of $V$ by assigning each pair $\{(i,j), (j,i)\}\subseteq V$ to one of the parts as follows: for $i,j\in [k]$ consider the pair of elements $\{(i,j), (j,i)\}\in V$; 
     we define $z_0:=0$ and $z_{\ell}:=\sum_{m=1}^{\ell}y((i,j),m)$ for every $\ell\in [k]$, pick $\theta\in [0,1]$ uniformly at random, and assign the pair of elements $\{(i,j), (j,i)\}$ to $V_{\ell}$ such that $z_{\ell-1}\le \theta < z_{\ell}$. We note that each element pair $\{(i,j), (j,i)\}$ is assigned to a part $\overline{V}_{\ell}$ independently with probability $y((i,j), \ell)$. 
    %by independently assigning each set $\{(i, j), (j, i)\}$ such that the probability $\{(i, j), (j, i)\} \subseteq \overline{V}_\ell$ is $\overline{x}((i, j), \ell) = \overline{x}((j, i), \ell)$. We observe that $V^*_1, \ldots, V^*_k$ is not necessarily a symmetric partition of $V$, but $\overline{V}_1, \ldots, \overline{V}_k$ is a symmetric partition of $V$. 
    We observe that $\overline{V}_1, \ldots, \overline{V}_k$ is a partition of $V$ with  $\overline{V}_i$ being symmetric and $(i, i)\in \overline{V}_i$ for every $i\in [k]$. We now show that $\E\left[f(\overline{V}_{\ell})\right]\le \E \left[ f(V^*_\ell)\right]$ for every $\ell\in [k]$. 
    
    %By the reasoning of the above paragraph, we have $\E \left[\sum_{\ell = 1}^k f(V^*_\ell)\right] = \mlsymopt$. 
    \begin{claim}\label{claim:symmetric-rounding-atmost-rounding}
        For every $\ell\in [k]$, we have that 
        \[\E\left[f(\overline{V}_{\ell})\right]\le \E \left[f(V^*_\ell)\right].\]
    \end{claim}
    \begin{proof}
    %\knote{Proof depends on row-column definition of $f$. Can we get rid of the dependence on this row-column definition and just rely on the fact that $f$ is transpose-invariant and $y_\ell$ is symmetric?}
    Let $\ell\in [k]$. 
    We recall that $V=[k]\times [k]$ and $f:2^V\rightarrow \R_{\ge 0}$ is a row-column-type function. %\knote{Define row-column type function.}. 
    Hence, there exists a function $g:2^{V}\rightarrow \R_{\ge 0}$ such that $f(A)=\sum_{i=1}^k (g(A\cap R_i) + g(A\cap C_i))$ for every $A\subseteq V$, where $R_i:=\{(i, j): j\in [k]\}$ and $C_i:=\{(j,i): j\in [k]\}$ for every $i\in [k]$. Hence, for every $i\in [k]$, we have that 
    \begin{align*}
        \E \left[ g\left(\overline{V}_\ell \cap R_i\right) \right] &= \sum_{S \subseteq R_i} g(S) \Pr \left[ \overline{V}_\ell \cap R_i = S\right] \\
        &= \sum_{S \subseteq R_i} g(S) \prod_{(i, j) \in S} y((i, j), \ell) \prod_{(i, j) \in R_i \setminus S} (1 - y((i, j), \ell)) \\%\quad \quad \text{(since each $(i, j) \in R_i$ is assigned independently)} \\
        &= \sum_{S \subseteq R_i} g(S) \Pr \left[ V^*_\ell \cap R_i = S\right] \\
        &= \E \left[ g\left(V^*_\ell \cap R_i\right) \right]. 
    \end{align*}
    Similar reasoning shows that $\E \left[ g\left(\overline{V}_\ell \cap C_i\right) \right] = \E \left[ g(V^*_\ell \cap C_i) \right]$ for every $i\in [k]$. 
    Hence, we have that 
    \begin{align*}
        \E \left[ f\left(\overline{V}_\ell\right) \right] &= \sum_{i = 1}^k \left(\E \left[ g\left(\overline{V}_\ell \cap R_i\right)\right] + \E \left[ g\left(\overline{V}_\ell \cap C_i\right) \right]\right)\\ 
        &= \sum_{i = 1}^k \left(\E \left[ g(V^*_\ell \cap R_i) \right] + \E \left[ g(V^*_\ell \cap C_i) \right]\right) \\
        &= \E \left[ f(V^*_\ell) \right].
    \end{align*}
    \end{proof}
    Claim \ref{claim:symmetric-rounding-atmost-rounding} implies that there exists a partition $\overline{V}_1, \ldots, \overline{V}_k$ of $V$ with  $\overline{V}_i$ being symmetric and $(i, i)\in \overline{V}_i$ for every $i\in [k]$ such that $\sum_{i=1}^{\ell}f(\overline{V}_{\ell})\le \E \left[\sum_{\ell = 1}^k f(V^*_\ell)\right] = \mlsymopt$ and hence, $\symopt\le \mlsymopt$. 
\end{enumerate}
\end{proof}

We will use the following three lemmas from \cite{Vondrak} to prove Theorem \ref{thm:sym-gap-to-oracle-lower-bound}. 

%\knote{Cite Vondrak's journal paper instead of EVW.}

\begin{lemma}[Lemma 3.1 from \cite{Vondrak}]
\label{lem:EVW_discrete}
    Let $H \colon [0, 1]^V \rightarrow \mathbb{R}$ be a function with absolutely continuous first partial derivatives. For an integer $n \geq 1$, let $N = [n]$ and define $h \colon 2^{N \times V} \rightarrow \mathbb{R}$ as $h(S) = H(\vx)$ where $x_i = \frac{1}{n}|S \cap (N \times \{i\})|$. Then, we have the following: 
    \begin{enumerate}
        \item If $\frac{\partial H}{\partial x_i} \geq 0$ everywhere for each $i$, then $h$ is monotone. 

        \item If $\frac{\partial^2 H}{\partial x_i \partial x_j} \leq 0$ almost everywhere for all $i, j$, then $h$ is submodular.
    \end{enumerate}
\end{lemma}

We will need the notion of transpose-invariant functions to state the next lemma. 
\begin{definition}
Let $V=[k]\times [k]$. A set function $f:2^V\rightarrow \R$ is \emph{transpose-invariant} if $f(A)=f(A^T)$ for every $A\subseteq V$. Generalizing, we say that a function $F:[0,1]^V\rightarrow R$ is \emph{transpose-invariant} if $F(\vx)=F(\vx^T)$ for every $\vx \in [0,1]^{[k]\times [k]}$, where $\vx^T$ is the transpose of the matrix $\vx$. 
\end{definition}
We note that a row-column-type set function is transpose-invariant by definition. 

\begin{lemma}[Lemma 3.2 from \cite{Vondrak}] 
\label{lem:EVW_continuous}
    Let $V=[k]\times [k]$, $f: 2^V\rightarrow \R_{\ge 0}$ be a transpose-invariant function over the set $V$, and $\eps>0$. 
    For $\vx\in [0,1]^{V}$, denote $\overline{\vx}=(\vx+\vx^T)/2$. 
    Then, there exists $\delta>0$ and functions $\hat{F}, \hat{G} \colon [0, 1]^V \rightarrow \mathbb{R}_{\ge 0}$ satisfying the following: 
    %Consider a function $f \colon 2^V \rightarrow \mathbb{R}$ that is invariant under a group of permutations $\mathcal{G}$ on the ground set $V$. Let $F$ be the multilinear extension of $f$, $\overline{\vx} = \E_{\sigma \in \mathcal{G}} \left[\sigma(\vx)\right]$, and fix an arbitrary $\epsilon > 0$. Then, there exists $\delta > 0$ and functions $\hat{F}, \hat{G} \colon [0, 1]^V \rightarrow \mathbb{R}_+$ (which are also symmetric with respect to $\mathcal{G}$) \knote{What does symmetric with respect to $\mathcal{G}$ mean?} \rnote{I think this means that $\hat{F}$ and $\hat{G}$ are invariant under $\mathcal{G}$}, satisfying:
    \begin{enumerate}[label=(\roman*)]
        \item Both $\hat{F}$ and $\hat{G}$ are transpose-invariant. %\knote{where is this conclusion used?}
        \item For all $\vx \in [0, 1]^V$, $\hat{G}(\vx) = \hat{F}(\overline{\vx})$.

        \item For all $\vx \in [0, 1]^V$, $|\hat{F}(\vx) - F(\vx)| \leq \epsilon$. 

        \item If $\|\vx - \overline{\vx}\|^2 \leq \delta$, then $\hat{F}(\vx) = \hat{G}(\vx)$ and the value of $\hat{F}(x)$ depends only on $\overline{\vx}$. 

        \item The first partial derivatives of $\hat{F}$ and $\hat{G}$ are absolutely continuous.

        \item If $f$ is monotone, then $\frac{\partial \hat{F}}{\partial x_i} \geq 0$ and $\frac{\partial \hat{G}}{\partial x_i} \geq 0$ everywhere. \label{label:monotone}

        \item If $f$ is submodular, then $\frac{\partial^2 \hat{F}}{\partial x_i \partial x_j} \leq 0$ and $\frac{\partial^2 \hat{G}}{\partial x_i \partial x_j} \leq 0$ almost everywhere. \label{submodular}
    \end{enumerate}
\end{lemma}



% Using $f \colon 2^V \rightarrow \mathbb{R_+}$ defined in Section \ref{subsect:sym_gap}, we define $\hat{F}$ and $\hat{G}$ from $f$ as in Lemma \ref{lem:EVW_continuous} (the value of $\epsilon$ will be chosen later). We consider two permutations of $V$, the identity and transpose, denoted $id \colon V \rightarrow V$ and $tr \colon V \rightarrow V$, respectively. For each $(i, j) \in V$, $id(i, j) = (i, j)$ and $tr(i, j) = (j, i)$. We extend $id$ and $tr$ to $[0, 1]^V$ in the natural fashion: for $\vx \in [0, 1]^V$, $id(\vx) = \vx$ and $tr(\vx) = \vx^T$ where $x^T(i, j) = x(j, i)$ for each $(i, j) \in V$. The group of permutations $\mathcal{G}$ that we use to define $\hat{F}$ and $\hat{G}$ is $\mathcal{G} = \{id, tr\}$. Hence, $\overline{\vx}$ is defined such that $\overline{x}(i, j) = \frac{1}{2} x(i, j) + \frac{1}{2} x(j, i)$ for each $(i, j) \in V$. 

% Next, for $n \geq 1$, which we will choose later, let $N = [n]$ and $X = N \times V$. For each $r \in N$, choose a permutation $\sigma^{(r)} \in \{id, tr\}$, each with probability $\frac{1}{2}$. Now, for $S \subseteq X$, we define the vector $\xi(S) \in [0, 1]^V$ such that 
% \[
%     \xi(S)_{(i, j)} = \frac{1}{n}\left|\left\{r \in N \colon \left(r, \sigma^{(r)}(i, j)\right) \in S\right\}\right|. 
% \]
% Finally, we define $\hat{f}, \hat{g} \colon X \rightarrow \mathbb{R}_+$ such that $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. By applying Lemmas \ref{lem:EVW_continuous} and \ref{lem:EVW_discrete}, we see that $\hat{f}$ and $\hat{g}$ are monotone submodular functions. As described in \cite{Vondrak}, for the purposes of proving the monotonicity and the submodularity of $\hat{f}$ and $\hat{g}$, it suffices to assume that $\sigma^{(r)} = id$ for all $r \in N$. We now consider the following instances of \monosubmp:
% \begin{align*}
%     &\min\left\{\sum_{\ell = 1}^k \hat{f}(S_\ell) \colon [S_1, \ldots, S_k] \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}, \\
%     &\min\left\{\sum_{\ell = 1}^k \hat{g}(S_\ell) \colon [S_1, \ldots, S_k] \text{ is a partition of } X \; \& \; \forall r \in N; \forall \ell \in [k]; (r, (\ell, \ell)) \in S_\ell\right\}. 
% \end{align*}
% For each $\ell \in [k]$, we can contract $N \times (\ell, \ell)$ into a single vertex such that we specify exactly one terminal per part $S_\ell \in [S_1, \ldots, S_k]$. 

% To prove our hardness result, we will need the following lemma from \cite{EVW}.

\begin{lemma}[Lemma 3.3 from \cite{Vondrak}]
\label{lem:EVW_distinguish} 
Let $V=[k]\times [k]$, $f: 2^V\rightarrow \R_{\ge 0}$ be a transpose-invariant function over the set $V$, and $\eps>0$. 
    Let $\hat{F}$, $\hat{G}$ be the two functions satisfying the conclusions of Lemma \ref{lem:EVW_continuous}. For an integer $n \ge 1$ and $N = [n]$, define two discrete functions $\hat{f}, \hat{g} \colon 2^{N \times V} \rightarrow \mathbb{R}_+$ as follows: 
    Let $\sigma_r\in \{0, 1\}$ be chosen uniformly at random for each $r\in N$. 
    %Let $\sigma^{(r)}$ be chosen uniformly at random in $\mathcal{G}$ for each $r \in N$. 
    For every set $S \subseteq N \times V$, we define a vector $\xi(S) \in [0, 1]^V$ by 
    \begin{align*}
    %:= \{r: \sigma^r = 0\}
    \xi(S)_{(i, j)} = \frac{1}{n} \left|\left\{r \in N \colon (r, (i, j)) \in S\text{ and } \sigma_r = 0\right\}\cup 
    \left\{r \in N \colon (r, (j, i)) \in S\text{ and } \sigma_r = 1\right\}
    \right|. 
        %\xi(S)_{(i, j)} = \frac{1}{n} |\{r \in N \colon (r, \sigma^{(r)}(i, j) \in S\}|. 
    \end{align*}
    and define $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. Then, deciding whether a function given by a value oracle is $\hat{f}$ or $\hat{g}$ (even using a randomized algorithm with a constant probability of success) requires $2^{\Omega(n)}$ function evaluation queries. 
\end{lemma}

We now prove Theorem \ref{thm:sym-gap-to-oracle-lower-bound}. In Theorem \ref{thm:sym-gap-to-oracle-lower-bound-terminal-sets} below, we prove that symmetry gap gives an inapproximability bound for a slight variant of \monosubmp where the terminals correspond to disjoint sets rather than singleton elements. 
We note that Theorem \ref{thm:sym-gap-to-oracle-lower-bound} follows from Theorem \ref{thm:sym-gap-to-oracle-lower-bound-terminal-sets}  (i.e., for the version of \monosubmp where the terminals are singleton elements) by a standard contraction  of terminal sets into a single terminal and appropriately modifying the associated submodular function. 
%\symGapToLowerBound*
\begin{theorem}\label{thm:sym-gap-to-oracle-lower-bound-terminal-sets}
    Let $V=[k]\times [k]$ and $f\colon 2^V \rightarrow \mathbb{R}_{\ge 0}$ be a row-column-type non-negative monotone submodular function over the set $V$. Then, for all $\gamma > 0$ and sufficiently large $n \in \mathbb{Z_+}$, there exists a non-negative monotone submodular function $\hat{f} \colon 2^{[n] \times V} \rightarrow \mathbb{R_+}$ and a collection of pairwise disjoint terminal sets $T_1, \ldots, T_k \subseteq  [n]\times V$ such that every algorithm that achieves an approximation factor of $\symgap(f)-\gamma$
    %require an exponential number of oracle queries in $n$ to achieve an $\left(\frac{\overline{OPT}}{OPT} - \gamma\right)$-approximation 
    for the following instance of \monosubmp requires $2^{\Omega(n)}$ function evaluation queries: 
    \[
        \min\left\{\sum_{i = 1}^k \hat{f}(V_i) \colon V_1, \ldots, V_k \text{ is a partition of } [n] \times V \text{ with } T_i \subseteq V_i \ \forall\ i \in [k]\right\}.  
    \]
\end{theorem}
\begin{proof}


    Let $\gamma > 0$. We choose $\epsilon > 0$ such that $\frac{\symopt - \epsilon k}{\opt + \epsilon(k + 1)} > \frac{\symopt}{\opt} - \gamma$. 
    Consider the multilinear relaxation of multiway partitioning wrt the function $f: 2^V\rightarrow \R$ for the terminals $t_{\ell}=(\ell,\ell)$ for every $\ell\in [k]$. We  fix $n \in \mathbb{Z}_+$ large enough such that there exists a feasible solution $\tilde{\vx}$ to the multilinear relaxation such that the entries of $\tilde{\vx}$ are all rational numbers with $n$ in the denominator and $\sum_{\ell = 1}^k F(\tilde{\vx}_\ell) \leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon$, where $\vx^*$ is an optimal solution to the multilinear relaxation (we note that such a solution $\tilde{x}$ exists since the objective of the multilinear relaxation is continuous). 
    For the chosen value of $\epsilon$, we use Lemma \ref{lem:EVW_continuous} to obtain $\hat{F}:[0,1]^V\rightarrow \R_+$ and $\hat{G}:[0,1]^V\rightarrow \R_+$ satisfying the conclusions of the lemma. For the chosen value of $n$, we let $N=[n]$ and $X=N\times V$. For each $r \in N$, we choose $\sigma_r \in \{0,1\}$ uniformly at random. Now, for $S \subseteq X$, we define the vector $\xi(S) \in [0, 1]^V$ such that 
    \[
        \xi(S)_{(i, j)} = \frac{1}{n} \left|\left\{r \in N \colon (r, (i, j)) \in S\text{ and } \sigma_r = 0\right\}\cup 
    \left\{r \in N \colon (r, (j, i)) \in S\text{ and } \sigma_r = 1\right\}
    \right|. 
    \]
    Next, we define $\hat{f}, \hat{g} \colon X \rightarrow \mathbb{R}_+$ as $\hat{f}(S) = \hat{F}(\xi(S))$ and $\hat{g}(S) = \hat{G}(\xi(S))$. By Lemma \ref{lem:EVW_continuous}(v)--(vii) and Lemma \ref{lem:EVW_discrete}, the functions $\hat{f}$ and $\hat{g}$ are monotone submodular. 
    %As described in \cite{Vondrak}, for the purposes of proving the monotonicity and the submodularity of $\hat{f}$ and $\hat{g}$, it suffices to assume that $\sigma^{(r)} = id$ for all $r \in N$ \knote{Why is this mentioned? Why doesn't it follow directly from the lemmas?}.
    %Fix $\epsilon > 0$ \knote{Is this the same $\eps$ that appears in the previous paragraph?}. 
    For each $\ell\in [k]$, let $T_{\ell}:=\{(r, (\ell, \ell): r\in N\}$. 
    We consider the following two instances of \monosubmp:
    \begin{align*}
        \min&\left\{\sum_{\ell = 1}^k \hat{f}(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } X \text{ with } T_{\ell}\subseteq X_{\ell}\ \forall\ \ell\in[k]\right\} \text{ and}  \\
        \min&\left\{\sum_{\ell = 1}^k \hat{g}(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } X \text{ with } T_{\ell}\subseteq X_{\ell}\ \forall\ \ell\in[k]\right\}. 
    \end{align*}
    %For each $\ell \in [k]$, we can contract $N \times (\ell, \ell)$ into a single vertex $t_\ell$ such that we specify exactly one terminal per part $X_\ell \in \{X_1, \ldots, X_k\}$ \knote{What is contraction?}. 
    Suppose for contradiction, there exists an approximation algorithm $\mathcal{A}$ for \monosubmp that achieves an approximation factor of $\left(\symgap(f)- \gamma\right)$ for both instances of \monosubmp using $2^{o(n)}$ function evaluation queries. We will use such an algorithm to design a procedure that decides whether a function given by a value oracle is $\hat{f}$ or $\hat{g}$ using $2^{o(n)}$ function evaluation queries, thereby contradicting Lemma \ref{lem:EVW_distinguish}. 
    
    We now describe our procedure to distinguish between $\hat{f}$ and $\hat{g}$ using algorithm $\mathcal{A}$. Given an oracle for an unknown function $h \in \{\hat{f}, \hat{g}\}$, the procedure applies algorithm $\mathcal{A}$ to the following instance of \monosubmp:
    \[
        \min\left\{\sum_{\ell = 1}^k h(X_\ell) \colon X_1, \ldots, X_k \text{ is a partition of } X \text{ with } T_{\ell}\subseteq S_\ell\ \ \forall\ \ell \in [k] \right\}. 
    \]
    Let the value returned by the algorithm be $\beta$. If $\beta < \symopt - \epsilon k$, then the procedure declares that $h = \hat{f}$. Otherwise, %$\beta \geq \symopt - \epsilon k$ and 
    the procedure declares that $h = \hat{g}$. 
    
    We now show correctness of our procedure. It suffices to show that $h=\hat{f}$ if and only if $\beta<\symopt - \eps k$. 
    Suppose $h\neq \hat{f}$, i.e., $h=\hat{g}$. Then, by Claim \ref{claim:hat-g-opt-is-larger-than-sym-opt} shown below, $\beta \geq \symopt - \epsilon k$. 
    Next, suppose that $h = \hat{f}$. Then, by Claim \ref{claim:hat-f-opt-is-smaller-than-sym-opt} shown below, $\beta \leq (OPT + \epsilon(k + 1)) \left( \symgap(f) - \gamma\right) < (OPT + \epsilon(k + 1)) \left( \frac{\symopt - \epsilon k}{\opt + \epsilon(k + 1)}  \right) = \symopt - \epsilon k$. 
    %We correctly determine the identity of $h$ using fewer than an exponential number of oracle queries in $n$. 
    %However, this contradicts Lemma \ref{lem:EVW_distinguish}. We conclude that all algorithms achieving a $\left(\frac{\overline{OPT}}{OPT} - \gamma\right)$-approximation to the above instance of \monosubmp require exponentially many oracle queries in $|X|$.
\end{proof}

\begin{claim}\label{claim:hat-g-opt-is-larger-than-sym-opt}
        For every partition $X_1, \ldots, X_k$ of $X = N \times V$ with $T_{\ell} \subseteq X_{\ell}$ for every $\ell \in [k]$, we have that 
        \[
        \sum_{\ell = 1}^k \hat{g}(X_\ell) \geq \symopt - \epsilon k. 
        \]
    \end{claim}
    %We demonstrate that for all partitions $X_1, \ldots, X_k$ of $X = N \times V$ such that $(r, (\ell, \ell)) \in X_\ell$ for each $r \in N$ and $\ell \in [k]$, $\sum_{\ell = 1}^k \hat{g}(X_\ell) \geq \symopt - \epsilon k$. 
    \begin{proof}
    Let $X_1, \ldots, X_k$ be a partition of $X$ with $T_{\ell} \subseteq X_{\ell}$ for every $\ell \in [k]$.  We have that 
    \begin{align*}
        \sum_{\ell = 1}^k \hat{g}(X_\ell) &= \sum_{\ell = 1}^k \hat{G}(\xi(X_\ell)) \quad \quad \text{(by definition of $\hat{g}$)}\\
        &= \sum_{\ell = 1}^k \hat{F}(\overline{\xi(X_\ell)}) \quad \quad \text{(by Lemma \ref{lem:EVW_continuous}(ii))}\\
        &\geq \sum_{\ell = 1}^k (F(\overline{\xi(X_\ell)}) - \epsilon) \quad \quad \text{(by Lemma \ref{lem:EVW_continuous}(iii))}\\
        &= \sum_{\ell = 1}^k F(\overline{\xi(X_\ell)}) - \epsilon k\\
        &\ge \symopt-\epsilon k. \quad \quad \text{(by Lemma \ref{lem:OPT_equality})} 
    \end{align*}
    The last inequality is by Lemma \ref{lem:OPT_equality} since  $\left(\overline{\xi(X_\ell)}\right)_{\ell = 1}^k$ is a feasible symmetric solution to the multilinear relaxation of multiway partitioning wrt the function $f:2^V\rightarrow \R$ for the terminals $t_{\ell}=(\ell,\ell)$ for every $\ell\in [k]$. 
    \end{proof}

    \begin{claim}\label{claim:hat-f-opt-is-smaller-than-sym-opt}
        There exists a partition $X_1, \ldots, X_k$ of $X = N \times V$ with $T_{\ell}\subseteq X_{\ell}$ for every $\ell \in [k]$ such that 
        \[
        \sum_{\ell = 1}^k \hat{f}(X_\ell) \leq \opt + \epsilon (k + 1). 
        \]
    \end{claim}
    \begin{proof}
    %Now, we demonstrate that for sufficiently large $n$ there exists a partition $X_1, \ldots, X_k$ of $X = N \times V$ satisfying $(r, (\ell, \ell)) \in X_\ell$ for each $r \in N$ and $\ell \in [k]$ such that $\sum_{\ell = 1}^k \hat{f}(X_\ell) \leq \opt + \epsilon (k + 1)$. 
    %Let $\vx^*$ be an optimum solution to the multilinear relaxation with value $\opt$. %defined in Definition \ref{def:multilinear} 
    %Since the objective of the multilinear relaxation is continuous, we may choose $n$ large enough such that 
    We recall that there exists a feasible solution $\tilde{\vx}$ and an optimum solution $\vx^*$ to the multilinear relaxation of multiway partitioning wrt the function $f: 2^V\rightarrow \R$ for the terminals $t_{\ell}=(\ell,\ell)$ for every $\ell\in [k]$ with the following property: the entries of $\tilde{\vx}$ are all rational numbers with $n$ in the denominator and $\sum_{\ell = 1}^k F(\tilde{\vx}_\ell) \leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon$. 
    We will round such a fractional solution $(\tilde{\vx}_{\ell})_{\ell\in [k]}$ to a partition $X_1, \ldots, X_k$ of $X=N\times V$ with $T_{\ell}\subseteq X_{\ell}$ for every $\ell\in [k]$ as follows: 
    %$\tilde{\vx} = \left(\xi(X_\ell)\right)_{\ell = 1}^k$ for the partition $X_1, \ldots, X_k$ defined as follows. Fix $i, j \in [k]$. Then for $1 \leq r \leq nx((i, j), 1)$, let $(r, \sigma^{(r)}(i, j))$ be assigned to $X_1$, for $nx((i, j), 1) + 1 \leq r \leq nx((i, j), 1) + nx((i, j), 2)$ let $(r, \sigma^{(r)}(i, j))$ be assigned to $X_2$, etc. 
    %We define a partition $X_1, \ldots, X_k$ by rounding $\tilde{\vx}$ as follows: 
    we define 
    \begin{align*}
        X_1^0&:=\{(r, (i,j)): r\in N, i, j\in [k], \sigma_r=0, r\in [nx((i,j), 1)]\}\},\\
        X_1^1&:=\{(r, (j,i)): r\in N, i, j\in [k], \sigma_r=1, r\in [nx((i,j), 1)]\}\}, 
    \end{align*}
    and for each $\ell\in \{2, \ldots, k\}$, 
    \begin{align*}
        X_{\ell}^0&:= \left\{(r, (i,j)): r\in N, i, j\in [k], \sigma_r=0, r\in [nx((i,j), {\ell-1})+1, nx((i,j), \ell-1)+nx((i,j), \ell)]\right\}\\
        X_{\ell}^1&:= \left\{(r, (j,i)): r\in N, i, j\in [k], \sigma_r=1, r\in [nx((i,j), {\ell-1})+1, nx((i,j), \ell-1)+nx((i,j), \ell)]\right\}, 
    \end{align*}
    and set
    $X_{\ell}:=X_{\ell}^0\cup X_{\ell}^1$ for every $\ell\in [k]$. We note that $X_1, \ldots, X_{\ell}$ is a partition of $X=N\times V$ with $T_{\ell}\subseteq X_{\ell}$ for every $\ell\in [k]$. Finally, we bound the cost of the solution as follows: 
    \begin{align*}
        \sum_{\ell = 1}^k \hat{f}(X_\ell) &= \sum_{\ell = 1}^k \hat{F}(\tilde{\vx}_\ell) \quad \quad \text{(by definition of $\hat{f}$ and $X_1, \ldots, X_k$)}\\
        &\leq \sum_{\ell = 1}^k \left(F(\tilde{\vx}_\ell) + \epsilon\right) \quad \quad \text{(by Lemma \ref{lem:EVW_continuous}(iii))}\\
        &= \sum_{\ell = 1}^k F(\tilde{\vx}_\ell) + \epsilon k \\
        &\leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon(k + 1) \quad \quad \left(\text{since $\sum_{\ell = 1}^k F(\tilde{\vx}_\ell) \leq \sum_{\ell = 1}^k F(\vx^*_\ell) + \epsilon$}\right)\\
        &= \opt + \epsilon(k + 1). 
    \end{align*}
    The last inequality is by Lemma \ref{lem:OPT_equality} since  $\left(x^*_\ell\right)_{\ell = 1}^k$ is an optimum solution to the multilinear relaxation of multiway partitioning wrt the function $f:2^V\rightarrow \R$ for the terminals $t_{\ell}=(\ell,\ell)$ for every $\ell\in [k]$. 
    \end{proof}
